A Primer on the Signature Method in Machine Learning

We provide an introduction to the signature method, focusing on its theoretical properties and machine learning applications. Our presentation is divided into two parts. In the first part, we present the definition and fundamental properties of the signature of a path. The signature is a sequence of numbers associated with a path that captures many of its important analytic and geometric properties. As a sequence of numbers, the signature serves as a compact description (dimension reduction) of a path. In presenting its theoretical properties, we assume only familiarity with classical real analysis and integration, and supplement theory with straightforward examples. We also mention several advanced topics, including the role of the signature in rough path theory. In the second part, we present practical applications of the signature to the area of machine learning. The signature method is a non-parametric way of transforming data into a set of features that can be used in machine learning tasks. In this method, data are converted into multi-dimensional paths, by means of embedding algorithms, of which the signature is then computed. We describe this pipeline in detail, making a link with the properties of the signature presented in the first part. We furthermore review some of the developments of the signature method in machine learning and, as an illustrative example, present a detailed application of the method to handwritten digit classification.

==> latexmkrc <==
$makeindex  = 'makeindex -s svind.ist %O -o %D %S';

$ENV{'TEXINPUTS'}='./style//:' . $ENV{'TEXINPUTS'}; 
$ENV{'BSTINPUTS'}='./style//:' . $ENV{'BSTINPUTS'}; 

###############################
# Post processing of pdf file #
###############################

# assume the jobname is 'output' for Overleaf v2
my $ORIG_PDF_AGE = -M "output.pdf"; # get age of existing pdf if present

END {
    my $NEW_PDF_AGE = -M "output.pdf";
    return if !defined($NEW_PDF_AGE); # bail out if no pdf file
    return if defined($ORIG_PDF_AGE) && $NEW_PDF_AGE == $ORIG_PDF_AGE; # bail out if pdf was not updated
    my $QPDF = "/usr/bin/qpdf";
    return if ! -x $QPDF; # check that qpdf exists
    my $status = system($QPDF, "--linearize", "output.pdf", "output.pdf.opt");
    my $exitcode = ($status >> 8);
    print "qpdf exit code=$exitcode\n";
    # qpdf returns 0 for success, 3 for warnings (output pdf still created)
    return if !($exitcode == 0 || $exitcode == 3);
    print "Renaming optimised file to output.pdf\n";
    rename("output.pdf.opt", "output.pdf");
}

##############
# Glossaries #
##############
add_cus_dep( 'glo', 'gls', 0, 'glo2gls' );
add_cus_dep( 'acn', 'acr', 0, 'glo2gls');  # from Overleaf v1
sub glo2gls {
	system("makeglossaries $_[0]");
}

#############
# makeindex #
#############
@ist = glob("*.ist");
if (scalar(@ist) > 0) {
        $makeindex = "makeindex -s $ist[0] %O -o %D %S";
}

################
# nomenclature #
################
add_cus_dep("nlo", "nls", 0, "nlo2nls");
sub nlo2nls {
	system("makeindex $_[0].nlo -s nomencl.ist -o $_[0].nls -t $_[0].nlg");
}

#########
# Knitr #
#########
my $root_file = $ARGV[-1];

add_cus_dep( 'Rtex', 'tex', 0, 'rtex_to_tex');
sub rtex_to_tex {
    do_knitr("$_[0].Rtex");
}

sub do_knitr {
    my $dirname = dirname $_[0];
    my $basename = basename $_[0];
    system("Rscript -e \"library('knitr'); setwd('$dirname'); knit('$basename')\"");
}

my $rtex_file = $root_file =~ s/\.tex$/.Rtex/r;
unless (-e $root_file) {
	if (-e $rtex_file) {
		do_knitr($rtex_file);
	}
}

##########
# feynmf #
##########
push(@file_not_found, '^feynmf: Files .* and (.*) not found:$');
add_cus_dep("mf", "tfm", 0, "mf_to_tfm");
sub mf_to_tfm { system("mf '\\mode:=laserjet; input $_[0]'"); }

push(@file_not_found, '^feynmf: Label file (.*) not found:$');
add_cus_dep("mf", "t1", 0, "mf_to_label1");
sub mf_to_label1 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t1"); }
add_cus_dep("mf", "t2", 0, "mf_to_label2");
sub mf_to_label2 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t2"); }
add_cus_dep("mf", "t3", 0, "mf_to_label3");
sub mf_to_label3 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t3"); }
add_cus_dep("mf", "t4", 0, "mf_to_label4");
sub mf_to_label4 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t4"); }
add_cus_dep("mf", "t5", 0, "mf_to_label5");
sub mf_to_label5 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t5"); }
add_cus_dep("mf", "t6", 0, "mf_to_label6");
sub mf_to_label6 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t6"); }
add_cus_dep("mf", "t7", 0, "mf_to_label7");
sub mf_to_label7 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t7"); }
add_cus_dep("mf", "t8", 0, "mf_to_label8");
sub mf_to_label8 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t8"); }
add_cus_dep("mf", "t9", 0, "mf_to_label9");
sub mf_to_label9 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t9"); }

##########
# feynmp #
##########
push(@file_not_found, '^dvipdf: Could not find figure file (.*); continuing.$');
add_cus_dep("mp", "1", 0, "mp_to_eps");
sub mp_to_eps {
    system("mpost $_[0]");
    return 0;
}

#############
# asymptote #
#############
sub asy {return system("asy --offscreen '$_[0]'");}
add_cus_dep("asy","eps",0,"asy");
add_cus_dep("asy","pdf",0,"asy");
add_cus_dep("asy","tex",0,"asy");

#############
# metapost  #  # from Overleaf v1
#############
add_cus_dep('mp', '1', 0, 'mpost');
sub mpost {
  my $file = $_[0];
  my ($name, $path) = fileparse($file);
  pushd($path);
  my $return = system "mpost $name";
  popd();
  return $return;
}

##########
# chktex #
##########
unlink 'output.chktex' if -f 'output.chktex';
if (defined $ENV{'CHKTEX_OPTIONS'}) {
    use File::Basename;
    use Cwd;

    # identify the main file
    my $target = $ARGV[-1];
    my $file = basename($target);

    if ($file =~ /\.tex$/) {
	# change directory for a limited scope
	my $orig_dir = cwd();
	my $subdir = dirname($target);
	chdir($subdir);
	# run chktex on main file
	$status = system(
    "/usr/bin/run-chktex.sh",
    $orig_dir,
    $file
  );
	# go back to original directory
	chdir($orig_dir);

	# in VALIDATE mode we always exit after running chktex
	# otherwise we exit if EXIT_ON_ERROR is set

	if ($ENV{'CHKTEX_EXIT_ON_ERROR'} || $ENV{'CHKTEX_VALIDATE'}) {
	    # chktex doesn't let us access the error info via exit status
	    # so look through the output
	    open(my $fh, "<", "output.chktex");
	    my $errors = 0;
	    {
		local $/ = "\n";
		while(<$fh>) {
		    if (/^\S+:\d+:\d+: Error:/) {
			$errors++;
			print;
		    }
		}
	    }
	    close($fh);
	    exit(1) if $errors > 0;
	    exit(0) if $ENV{'CHKTEX_VALIDATE'};
	}
    }
}


==> references.tex <==
%%%%%%%%%%%%%%%%%%%%%%%% referenc.tex %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sample references
% %
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer-Verlag %%%%%%%%%%%%%%%%%%%%%%%%%%
%
% BibTeX users please use
% \bibliographystyle{plain}
% \bibliography{Refs}
%
\begin{thebibliography}{10}

\bibitem{Agrachev_Sachkov_04}
Andrei~A. Agrachev and Yuri~L. Sachkov.
\newblock {\em Control theory from the geometric viewpoint}, volume~87 of {\em
  Encyclopaedia of Mathematical Sciences}.
\newblock Springer-Verlag, Berlin, 2004.
\newblock Control Theory and Optimization, II.

\bibitem{misc_pen-based_recognition_of_handwritten_digits_81}
E.~Alpaydin and F.~Alimoglu.
\newblock {Pen-Based Recognition of Handwritten Digits}.
\newblock UCI Machine Learning Repository, 1998.
\newblock {DOI}: \url{10.24432/C5MG6K}.

\bibitem{Applebaum09}
David Applebaum.
\newblock {\em L\'{e}vy processes and stochastic calculus}, volume 116 of {\em
  Cambridge Studies in Advanced Mathematics}.
\newblock Cambridge University Press, Cambridge, second edition, 2009.

\bibitem{perez2020signatures}
Imanol~Perez Arribas.
\newblock {\em Signatures in machine learning and finance}.
\newblock PhD thesis, University of Oxford, 2020.

\bibitem{Billingsley12}
Patrick Billingsley.
\newblock {\em Probability and measure}.
\newblock Wiley Series in Probability and Statistics. John Wiley \& Sons, Inc.,
  Hoboken, NJ, 2012.
\newblock Anniversary edition [of MR1324786], With a foreword by Steve Lalley
  and a brief biography of Billingsley by Steve Koppes.

\bibitem{BDMN21}
Horatio Boedihardjo, Joscha Diehl, Marc Mezzarobba, and Hao Ni.
\newblock The expected signature of {B}rownian motion stopped on the boundary
  of a circle has finite radius of convergence.
\newblock {\em Bull. Lond. Math. Soc.}, 53(1):285--299, 2021.

\bibitem{Boedihardjo14}
Horatio Boedihardjo, Xi~Geng, Terry Lyons, and Danyu Yang.
\newblock The signature of a rough path: uniqueness.
\newblock {\em Adv. Math.}, 293:720--737, 2016.

\bibitem{BoedihardjoNi14}
Horatio Boedihardjo, Hao Ni, and Zhongmin Qian.
\newblock Uniqueness of signature for simple curves.
\newblock {\em J. Funct. Anal.}, 267(6):1778--1806, 2014.

\bibitem{Brockett_15}
Roger~W. Brockett.
\newblock {\em Finite dimensional linear systems}, volume~74 of {\em Classics
  in Applied Mathematics}.
\newblock Society for Industrial and Applied Mathematics (SIAM), Philadelphia,
  PA, 2015.
\newblock Reprint of the 1970 original.

\bibitem{CassOgrodnik17}
Thomas Cass and Marcel Ogrodnik.
\newblock Tail estimates for {M}arkovian rough paths.
\newblock {\em Ann. Probab.}, 45(4):2477--2504, 2017.

\bibitem{ChechkinPavlyukevich14}
Alexei Chechkin and Ilya Pavlyukevich.
\newblock Marcus versus {S}tratonovich for systems with jump noise.
\newblock {\em J. Phys. A}, 47(34):342001, 15, 2014.

\bibitem{Chen57}
Kuo-Tsai Chen.
\newblock Integration of paths, geometric invariants and a generalized
  {B}aker-{H}ausdorff formula.
\newblock {\em Ann. of Math. (2)}, 65:163--178, 1957.

\bibitem{Chen58}
Kuo-Tsai Chen.
\newblock Integration of paths---a faithful representation of paths by
  non-commutative formal power series.
\newblock {\em Trans. Amer. Math. Soc.}, 89:395--407, 1958.

\bibitem{Chevyrev18}
Ilya Chevyrev.
\newblock Random walks and {L}\'{e}vy processes as rough paths.
\newblock {\em Probab. Theory Related Fields}, 170(3-4):891--932, 2018.

\bibitem{CF19}
Ilya Chevyrev and Peter~K. Friz.
\newblock Canonical {RDE}s and general semimartingales as rough paths.
\newblock {\em Ann. Probab.}, 47(1):420--463, 2019.

\bibitem{CFKM20}
Ilya Chevyrev, Peter~K. Friz, Alexey Korepanov, and Ian Melbourne.
\newblock Superdiffusive limits for deterministic fast-slow dynamical systems.
\newblock {\em Probab. Theory Related Fields}, 178(3-4):735--770, 2020.

\bibitem{CGW21}
Ilya {Chevyrev}, Andris {Gerasimovics}, and Hendrik {Weber}.
\newblock {Feature Engineering with Regularity Structures}.
\newblock {\em arXiv e-prints}, arXiv:2108.05879, August 2021.

\bibitem{CL16}
Ilya Chevyrev and Terry Lyons.
\newblock Characteristic functions of measures on geometric rough paths.
\newblock {\em Ann. Probab.}, 44(6):4049--4082, 2016.

\bibitem{CNO20}
Ilya {Chevyrev}, Vidit {Nanda}, and Harald {Oberhauser}.
\newblock Persistence paths and signature features in topological data
  analysis.
\newblock {\em IEEE Transactions on Pattern Analysis and Machine Intelligence},
  42(1):192--202, 2020.

\bibitem{CO18}
Ilya Chevyrev and Harald Oberhauser.
\newblock Signature moments to characterize laws of stochastic processes.
\newblock {\em Journal of Machine Learning Research}, 23(176):1--42, 2022.

\bibitem{ContTankov04}
Rama Cont and Peter Tankov.
\newblock {\em Financial modelling with jump processes}.
\newblock Chapman \& Hall/CRC Financial Mathematics Series. Chapman \&
  Hall/CRC, Boca Raton, FL, 2004.

\bibitem{2022arXiv221014247D}
Joscha {Diehl} and Leonard {Schmitz}.
\newblock {Two-parameter sums signatures and corresponding quasisymmetric
  functions}.
\newblock {\em arXiv e-prints}, October 2022.

\bibitem{gyurko2014extracting}
Jonathann Field, Lajos~Gergely Gyurk{\'o}, Mark Kontkowski, and Terry Lyons.
\newblock Extracting information from the signature of a financial data stream.
\newblock arXiv:1307.7244, July 2014.
\newblock Preprint.

\bibitem{FrizHairer14}
Peter~K. Friz and Martin Hairer.
\newblock {\em A course on rough paths}.
\newblock Universitext. Springer, Cham, 2014.
\newblock With an introduction to regularity structures.

\bibitem{FS17}
Peter~K. Friz and Atul Shekhar.
\newblock General rough integration, {L}\'{e}vy rough paths and a
  {L}\'{e}vy-{K}intchine-type formula.
\newblock {\em Ann. Probab.}, 45(4):2707--2765, 2017.

\bibitem{FrizVictoir10}
Peter~K. Friz and Nicolas~B. Victoir.
\newblock {\em Multidimensional stochastic processes as rough paths}, volume
  120 of {\em Cambridge Studies in Advanced Mathematics}.
\newblock Cambridge University Press, Cambridge, 2010.

\bibitem{FZ17}
Peter~K. Friz and Huilin Zhang.
\newblock Differential equations driven by rough paths with jumps.
\newblock {\em J. Differential Equations}, 264(10):6226--6301, 2018.

\bibitem{geddes2015comparative}
John~R Geddes, Alexandra Gardiner, Jennifer Rendell, Merryn Voysey, Elizabeth
  Tunbridge, Christopher Hinds, Ly-Mee Yu, Jane Hainsworth, Mary-Jane
  Attenburrow, Judit Simon, et~al.
\newblock Comparative evaluation of quetiapine plus lamotrigine combination
  versus quetiapine monotherapy (and folic acid versus placebo) in bipolar
  depression (cequel): a 2$\times$ 2 factorial randomised trial.
\newblock {\em The Lancet Psychiatry}, 2015.

\bibitem{Geng15}
Xi~Geng.
\newblock Reconstruction for the signature of a rough path.
\newblock {\em Proc. Lond. Math. Soc. (3)}, 114(3):495--526, 2017.

\bibitem{GLNO22}
Chad {Giusti}, Darrick {Lee}, Vidit {Nanda}, and Harald {Oberhauser}.
\newblock {A Topological Approach to Mapping Space Signatures}.
\newblock {\em arXiv e-prints}, page arXiv:2202.00491, February 2022.

\bibitem{graham2013sparse}
Benjamin Graham.
\newblock Sparse arrays of signatures for online character recognition.
\newblock arXiv:1308.0371, December 2013.
\newblock Preprint.

\bibitem{Gubinelli10}
Massimiliano Gubinelli.
\newblock Ramification of rough paths.
\newblock {\em J. Differential Equations}, 248(4):693--721, 2010.

\bibitem{Hairer14}
Martin Hairer.
\newblock A theory of regularity structures.
\newblock {\em Invent. Math.}, 198(2):269--504, 2014.

\bibitem{Hambly10}
Ben Hambly and Terry Lyons.
\newblock Uniqueness for the signature of a path of bounded variation and the
  reduced path group.
\newblock {\em Ann. of Math. (2)}, 171(1):109--167, 2010.

\bibitem{kalsi2020optimal}
Jasdeep Kalsi, Terry Lyons, and Imanol~Perez Arribas.
\newblock Optimal execution with rough path signatures.
\newblock {\em SIAM Journal on Financial Mathematics}, 11(2):470--493, 2020.

\bibitem{kidger2019deep}
Patrick Kidger, Patric Bonnier, Imanol Perez~Arribas, Cristopher Salvi, and
  Terry Lyons.
\newblock Deep signature transforms.
\newblock {\em Advances in Neural Information Processing Systems}, 32, 2019.

\bibitem{kidger2020signatory}
Patrick Kidger and Terry Lyons.
\newblock Signatory: differentiable computations of the signature and
  logsignature transforms, on both cpu and gpu.
\newblock {\em arXiv preprint arXiv:2001.00706}, 2020.

\bibitem{signatory}
Patrick Kidger and Terry Lyons.
\newblock {\em {signatory}}, 2021.

\bibitem{kidger2020neural}
Patrick Kidger, James Morrill, James Foster, and Terry Lyons.
\newblock Neural controlled differential equations for irregular time series.
\newblock {\em Advances in Neural Information Processing Systems},
  33:6696--6707, 2020.

\bibitem{KO19}
Franz~J. Kir\'{a}ly and Harald Oberhauser.
\newblock Kernels for sequentially ordered data.
\newblock {\em J. Mach. Learn. Res.}, 20:Paper No. 31, 45, 2019.

\bibitem{Carleman_cond_98}
B.~Korenblum, A.~Mascuilli, and J.~Panariello.
\newblock A generalization of {C}arleman's uniqueness theorem and a discrete
  {P}hragm\'{e}n-{L}indel\"{o}f theorem.
\newblock {\em Proc. Amer. Math. Soc.}, 126(7):2025--2032, 1998.

\bibitem{kormilitzin2016application}
AB~Kormilitzin, KEA Saunders, PJ~Harrison, JR~Geddes, and TJ~Lyons.
\newblock Application of the signature method to pattern recognition in the
  cequel clinical trial.
\newblock {\em arXiv preprint arXiv:1606.02074}, 2016.

\bibitem{kormilitzin2017detecting}
Andrey Kormilitzin, Kate~EA Saunders, Paul~J Harrison, John~R Geddes, and Terry
  Lyons.
\newblock Detecting early signs of depressive and manic episodes in patients
  with bipolar disorder using the signature-based model.
\newblock {\em arXiv preprint arXiv:1708.01206}, 2017.

\bibitem{kormilitzin2020efficient}
Andrey Kormilitzin, Nemanja Vaci, Qiang Liu, Hao Ni, Goran Nenadic, and Alejo
  Nevado-Holgado.
\newblock An efficient representation of chronological events in medical texts.
\newblock {\em arXiv preprint arXiv:2010.08433}, 2020.

\bibitem{KPP95}
Thomas~G. Kurtz, \'{E}tienne Pardoux, and Philip Protter.
\newblock Stratonovich stochastic differential equations driven by general
  semimartingales.
\newblock {\em Ann. Inst. H. Poincar\'{e} Probab. Statist.}, 31(2):351--377,
  1995.

\bibitem{levin2015learning}
Daniel Levin, Terry Lyons, and Hao Ni.
\newblock Learning from the past, predicting the statistics for the future,
  learning an evolving system.
\newblock arXiv:1309.0260, September 2015.
\newblock Preprint.

\bibitem{LiNi22}
Siran Li and Hao Ni.
\newblock Expected signature of stopped {B}rownian motion on {$d$}-dimensional
  {$C^{2,\alpha}$}-domains has finite radius of convergence everywhere: {$2\leq
  d\leq8$}.
\newblock {\em J. Funct. Anal.}, 282(12):Paper No. 109447, 45, 2022.

\bibitem{Liao22}
Shujian Liao.
\newblock {\em Log signatures in machine learning}.
\newblock PhD thesis, University College London, 2022.

\bibitem{2019arXiv190808286L}
Shujian {Liao}, Terry {Lyons}, Weixin {Yang}, and Hao {Ni}.
\newblock {Learning stochastic differential equations using RNN with log
  signature features}.
\newblock {\em arXiv e-prints}, August 2019.

\bibitem{lyons2020non}
Terry Lyons, Sina Nejad, and Imanol Perez~Arribas.
\newblock Non-parametric pricing and hedging of exotic derivatives.
\newblock {\em Applied Mathematical Finance}, 27(6):457--494, 2020.

\bibitem{Lyons1998}
Terry~J. Lyons.
\newblock Differential equations driven by rough signals.
\newblock {\em Rev. Mat. Iberoamericana}, 14(2):215--310, 1998.

\bibitem{Lyons07}
Terry~J Lyons, Michael Caruana, and Thierry L{\'e}vy.
\newblock {\em Differential equations driven by rough paths}.
\newblock Springer, 2007.

\bibitem{lyons2005sound}
Terry~J Lyons and Nadia Sidorova.
\newblock Sound compression: a rough path approach.
\newblock In {\em Proceedings of the 4th international symposium on Information
  and communication technologies}, pages 223--228. Trinity College Dublin,
  2005.

\bibitem{LyonsXu15I}
Terry~J. Lyons and Weijun Xu.
\newblock Hyperbolic development and inversion of signature.
\newblock {\em J. Funct. Anal.}, 272(7):2933--2955, 2017.

\bibitem{LyonsXu15II}
Terry~J. Lyons and Weijun Xu.
\newblock Inverting the signature of a path.
\newblock {\em J. Eur. Math. Soc. (JEMS)}, 20(7):1655--1687, 2018.

\bibitem{Marcus78}
Steven~I. Marcus.
\newblock Modeling and analysis of stochastic differential equations driven by
  point processes.
\newblock {\em IEEE Trans. Inform. Theory}, 24(2):164--172, 1978.

\bibitem{Marcus80}
Steven~I. Marcus.
\newblock Modeling and approximation of stochastic differential equations
  driven by semimartingales.
\newblock {\em Stochastics}, 4(3):223--245, 1980/81.

\bibitem{mcinnes2018umap}
Leland McInnes, John Healy, Nathaniel Saul, and Lukas Großberger.
\newblock Umap: Uniform manifold approximation and projection.
\newblock {\em Journal of Open Source Software}, 3(29):861, 2018.

\bibitem{MZ15}
Ian Melbourne and Roland Zweim\"{u}ller.
\newblock Weak convergence to stable {L}\'{e}vy processes for nonuniformly
  hyperbolic dynamical systems.
\newblock {\em Ann. Inst. Henri Poincar\'{e} Probab. Stat.}, 51(2):545--556,
  2015.

\bibitem{moore2019using}
PJ~Moore, TJ~Lyons, John Gallacher, and Alzheimer’s Disease~Neuroimaging
  Initiative.
\newblock Using path signatures to predict a diagnosis of alzheimer’s
  disease.
\newblock {\em PloS one}, 14(9):e0222212, 2019.

\bibitem{morrill2020generalised}
James Morrill, Adeline Fermanian, Patrick Kidger, and Terry Lyons.
\newblock A generalised signature method for multivariate time series feature
  extraction.
\newblock {\em arXiv preprint arXiv:2006.00873}, 2020.

\bibitem{morrill2020utilization}
James~H Morrill, Andrey Kormilitzin, Alejo~J Nevado-Holgado, Sumanth
  Swaminathan, Samuel~D Howison, and Terry~J Lyons.
\newblock Utilization of the signature method to identify the early onset of
  sepsis from multivariate physiological time series in critical care
  monitoring.
\newblock {\em Critical Care Medicine}, 48(10):e976--e981, 2020.

\bibitem{perez2018signature}
Imanol Perez~Arribas, Guy~M Goodwin, John~R Geddes, Terry Lyons, and Kate~EA
  Saunders.
\newblock A signature-based machine learning model for distinguishing bipolar
  disorder and borderline personality disorder.
\newblock {\em Translational psychiatry}, 8(1):274, 2018.

\bibitem{Ree58}
Rimhak Ree.
\newblock Lie elements and an algebra associated with shuffles.
\newblock {\em Ann. of Math. (2)}, 68:210--220, 1958.

\bibitem{rehman2020gait}
Rana Zia~Ur Rehman, Yuhan Zhou, Silvia Del~Din, Lisa Alcock, Clint Hansen,
  Yu~Guan, Tibor Hortob{\'a}gyi, Walter Maetzler, Lynn Rochester, and
  Claudine~JC Lamoth.
\newblock Gait analysis with wearables can accurately classify fallers from
  non-fallers: A step toward better management of neurological disorders.
\newblock {\em Sensors}, 20(23):6992, 2020.

\bibitem{reizenstein2017calculation}
Jeremy Reizenstein.
\newblock Calculation of iterated-integral signatures and log signatures.
\newblock {\em arXiv preprint arXiv:1712.02757}, 2017.

\bibitem{reizenstein2018iisignature}
Jeremy Reizenstein and Benjamin Graham.
\newblock The iisignature library: efficient calculation of iterated-integral
  signatures and log signatures.
\newblock {\em arXiv preprint arXiv:1802.08252}, 2018.

\bibitem{iisignature}
Jeremy Reizenstein and Benjamin Graham.
\newblock {\em {iisignature}}, 2019.

\bibitem{Reizenstein20}
Jeremy~F. Reizenstein and Benjamin Graham.
\newblock Algorithm 1004: The iisignature library: Efficient calculation of
  iterated-integral signatures and log signatures.
\newblock {\em ACM Trans. Math. Softw.}, 46(1), mar 2020.

\bibitem{reizenstein2019iterated}
Jeremy~Francis Reizenstein.
\newblock {\em Iterated-integral signatures in machine learning.}
\newblock PhD thesis, University of Warwick, 2019.

\bibitem{Reutenauer93}
Christophe Reutenauer.
\newblock {\em Free {L}ie algebras}, volume~7 of {\em London Mathematical
  Society Monographs. New Series}.
\newblock The Clarendon Press, Oxford University Press, New York, 1993.
\newblock Oxford Science Publications.

\bibitem{Rudin76}
Walter Rudin.
\newblock {\em Principles of mathematical analysis}.
\newblock International Series in Pure and Applied Mathematics. McGraw-Hill
  Book Co., New York-Auckland-D\"{u}sseldorf, third edition, 1976.

\bibitem{esiglib}
{Terry Lyons}.
\newblock {\em {esig}}, 2023.

\bibitem{Tindel_Chouk_15}
Samy Tindel and Khalil Chouk.
\newblock Skorohod and {S}tratonovich integration in the plane.
\newblock {\em Electron. J. Probab.}, 20:no. 39, 39, 2015.

\bibitem{Whitt02}
Ward Whitt.
\newblock {\em Stochastic-process limits}.
\newblock Springer Series in Operations Research. Springer-Verlag, New York,
  2002.
\newblock An introduction to stochastic-process limits and their application to
  queues.

\bibitem{Williams01}
David R.~E. Williams.
\newblock Path-wise solutions of stochastic differential equations driven by
  {L}\'{e}vy processes.
\newblock {\em Rev. Mat. Iberoamericana}, 17(2):295--329, 2001.

\bibitem{wilson2018path}
Daniel Wilson-Nunn, Terry Lyons, Anastasia Papavasiliou, and Hao Ni.
\newblock A path signature approach to online arabic handwriting recognition.
\newblock In {\em 2018 IEEE 2nd International Workshop on Arabic and Derived
  Script Analysis and Recognition (ASAR)}, pages 135--139. IEEE, 2018.

\bibitem{xie2017learning}
Zecheng Xie, Zenghui Sun, Lianwen Jin, Hao Ni, and Terry Lyons.
\newblock Learning spatial-semantic context with fully convolutional recurrent
  network for online handwritten chinese text recognition.
\newblock {\em IEEE transactions on pattern analysis and machine intelligence},
  40(8):1903--1917, 2017.

\bibitem{yang2022developing}
Weixin Yang, Terry Lyons, Hao Ni, Cordelia Schmid, and Lianwen Jin.
\newblock Developing the path signature methodology and its application to
  landmark-based human action recognition.
\newblock In {\em Stochastic Analysis, Filtering, and Stochastic Optimization:
  A Commemorative Volume to Honor Mark HA Davis's Contributions}, pages
  431--464. Springer, 2022.

\bibitem{ZLT22}
Sheng Zhang, Guang Lin, and Samy Tindel.
\newblock Two-dimensional signature of images and texture classification.
\newblock {\em Proceedings of the Royal Society A: Mathematical, Physical and
  Engineering Sciences}, 478(2266):20220346, 2022.

\end{thebibliography}



==> section_files_tex/0_abstract.tex <==
\begin{comment}
\abstract{
In these notes, we wish to provide an introduction to the signature method, focusing on its basic theoretical properties and recent machine learning applications.

The notes are split into two parts. The first part focuses on the definition and fundamental properties of the signature of a path, or the {\it path signature}. We have aimed for a minimalistic approach, assuming only familiarity with classical real analysis and integration theory, and supplementing theory with straightforward examples. We have chosen to focus in detail on the principle properties of the signature which we believe are fundamental to understanding its role in applications. We also present an informal discussion on some of its deeper properties and briefly mention the role of the signature in rough paths theory, which we hope could serve as a light introduction to rough paths for the interested reader.

The second part of these notes discusses practical applications of the path signature to the area of machine learning. The signature approach represents a non-parametric way for extraction of characteristic features from data. The data are converted into a multi-dimensional path by means of various embedding algorithms and then processed for computation of individual terms of the signature which summarise certain information contained in the data. The signature thus transforms raw data into a set of features which are used in machine learning tasks. Roughly speaking, the signature is a sequence of numbers, associated with a path which captures many of the path's important analytic and geometric properties. As a sequence of numbers, the signature serves as a compact description (dimension reduction) of a path.

We will review current progress in applications of signatures to machine learning problems.
}
\end{comment}

\abstract{
In these notes, we provide an introduction to the signature method, focusing on its theoretical properties and recent machine learning applications.

The notes are split into two parts. The first part focuses on the definition and fundamental properties of the signature of a path.
The signature is a sequence of numbers associated with a path that captures many of the path's important analytic and geometric properties. As a sequence of numbers, the signature serves as a compact description (dimension reduction) of a path.
In presenting its theoretical properties, we assume only familiarity with classical real analysis and integration, and supplement theory with straightforward examples.
We also discuss informally several advanced topics, including and the role of the signature in rough paths theory.

The second part of these notes presents practical applications of the signature to the area of machine learning. The signature method is a non-parametric way of transforming data into a set of features that can be used in machine learning tasks.
In this method, data are converted into multi-dimensional paths by means of embedding algorithms of which the signature is then computed.
We describe this pipeline in detail, making a link with the properties of the signature presented in the first part.
We furthermore review some of the developments of the signature method in machine learning and, as an illustrative example, present a detailed application of the method to hand-written digits classification.
}

==> section_files_tex/1_2.tex <==
\subsection{The signature of a path}
\label{subsec:signature}

\subsubsection{Definition}

Having recalled the path integral of one real-valued path against another, we are now ready to define the signature of a path. For a path $X : [a,b] \to \R^d$, recall that we denote the coordinate paths by $(X^1_t, \ldots X^d_t)$, where each $X^i : [a,b] \to \R$ is a real-valued path. For any single index $i \in \{1,\ldots, d\}$, let us define the quantity
\begin{eqnarray}\label{singInteg}
S(X)^i_{a,t} = \int_{a < s < t} dX^i_s = X^i_t - X^i_a,
\end{eqnarray}
%
which is the increment of the $i$-th coordinate of the path at time $t \in [a,b]$. We emphasise that $S(X)^i_{a,\cdot} : [a,b] \to \R$ is itself a real-valued path. Note that $a$ in the subscript of $S(X)^i_{a,t}$ is only used to denote the starting point of the interval $[a,b]$.

Now for any pair $i,j \in \{1, \ldots, d\}$, let us define the {\it double-iterated} integral
\begin{eqnarray}\label{doublInteg}
S(X)^{i,j}_{a,t} = \int_{a < s < t} S(X)^i_{a,s} \, dX^j_s\;=\;\int_{a < r < s < t} dX^i_{r}\,dX^j_{s},
\end{eqnarray}
%
where $S(X)^i_{a,s}$ is given by~\eqref{singInteg}. 

%and the integration limits are
%
%\begin{equation}\label{triangle}
%a < r < s < t = \begin{cases}
%             a < r < s \\
%             a < s < t.
%       \end{cases} \quad
%\end{equation}
% 
The integration limits in~\eqref{doublInteg} also correspond to integration over a triangle (or, more generally, over a simplex in higher dimension).  We emphasise again that $S(X)^i_{a,s}$ and $X^j_s$ are simply real-valued paths, so the expression~\eqref{doublInteg} is a special case of the path integral, and that $S(X)^{i,j}_{a,\cdot} : [a,b] \to \R$ is itself a real-valued path.
%Remark moreover that $S(X)^{i,j}_{a,t}$ may equivalently be written as
%\[
%S(X)^{i,j}_t = \int_{a < t_1 < t} \int_{a < t_2 < t_1} dX^i_{t_2} dX^j_{t_1}.
%\]
%

Likewise for any triple $i,j,k \in \{ 1, \ldots, d\}$ we define the {\it triple-iterated} integral
\begin{eqnarray}
S(X)^{i,j,k}_{a,t} = \int_{a < s < t} S(X)^{i,j}_{a,s} \, dX^k_s \;=\;\int_{a < q < r < s < t} dX^i_{q}\, dX^j_{r}\,dX^k_{s}.
\end{eqnarray}
%
Again, since $S(X)^{i,j}_{a,s}$ and $X^k_s$ are real-valued paths, the above is just a special case of the path integral, and $S(X)^{i,j,k}_{a,\cdot} : [a,b] \to \R$ is itself a real-valued path.
%
%\[
%S(X)^{i,j}_{a,t} = \int_{a < t_1 < t} \int_{a < t_2 < t_1} \int_{a < t_3 < t_2} dX^i_{t_3} dX^j_{t_2} dX^k_{t_1}.
%\]
%

We can continue recursively, and for any integer $k \geq 1$ and collection of indexes $i_1, \ldots, i_k  \in \{ 1, \ldots, d\}$, we define
\begin{eqnarray}
S(X)^{i_1,\ldots, i_k}_{a,t} = \int_{a< s < t} S(X)^{i_1,\ldots, i_{k-1}}_{a,s} \, dX^{i_k}_s.
\end{eqnarray}
%
As before, since $S(X)^{i_1,\ldots, i_{k-1}}_{a,s}$ and $X^{i_k}_s$ are real-valued paths, the above is defined as a path integral, and $S(X)^{i_1,\ldots, i_k}_{a,\cdot} : [a,b] \to \R$ is a real-valued path. Observe that we may equivalently write
\begin{eqnarray}\label{eq:iter_int_rep}
S(X)^{i_1,\ldots, i_k}_{a,t} = \int_{a < t_k < t} \ldots \int_{a < t_1 < t_{2}} dX^{i_1}_{t_1} \ldots \, dX^{i_k}_{t_k}.
\end{eqnarray}
%
The real number $S(X)^{i_1,\ldots, i_k}_{a,b}$ is called the \emph{k-fold iterated integral} of $X$ along the indexes $i_1,\ldots, i_k$.
%
\begin{definition}[Signature]
The \emph{signature} of a path $X : [a,b] \to \R^d$, denoted by $S(X)_{a,b}$, is the collection (infinite sequence) of all the iterated integrals of $X$. Formally, $S(X)_{a,b}$ is the collection of real numbers
\begin{eqnarray}\label{eq:definSig}
S(X)_{a,b}\;=\; (1, S(X)^1_{a,b}, \ldots, S(X)^d_{a,b}, S(X)^{1,1}_{a,b}, S(X)^{1,2}_{a,b}, \ldots)
\end{eqnarray}
where the ``zeroth'' term, by convention, is equal to $1$, and the index in the superscript runs along the set of all \emph{multi-indexes}
\begin{eqnarray}\label{eq:words_def}
W = \{(i_1,\ldots, i_k) \mid k \geq 0, i_1,\ldots, i_k \in \{1,\ldots, d\}\}.
\end{eqnarray}
\end{definition}


The set $W$ above is also frequently called the set of \emph{words} on the \emph{alphabet} $A = \{1,\ldots, d\}$.
Remark that $W$ contains the empty multi-index $I=\emptyset$, corresponding to $k=0$ in~\eqref{eq:words_def},
and $S(X)^\emptyset_{a,b}=1$, which is the first element on the right-hand side of~\eqref{eq:definSig}.
The motivation for the convention $S(X)^\emptyset_{a,b}=1$ is due to Chen's identity that we discuss in Section~\ref{subsubsec:Chen}.
%
\begin{example}
Consider an alphabet consisting of three letters only: $\{1,2,3\}$. There is an infinite number of words which could be composed from this alphabet, namely:
\begin{equation}
\{1,2,3\} \rightarrow (\emptyset, 1,2,3,11,12,13,21,22,23,31,32,33,111,112,113,121,\dots).
\end{equation}
\end{example}


%The case $k=0$ in the above definition corresponds to the empty multi-index, often denoted $S(X)^0_T$, which we define by convention as $S(X)^0_T = 1$.

An important property of the signature, which we immediately note, is that the iterated integrals of a path $X$ are independent of the starting point of $X$. That is, if for some $x \in \R^d$, we define the path $\widetilde X_t = X_t + x$, then $S(\widetilde X)^{i_1,\ldots, i_k}_{a,b} = S(X)^{i_1,\ldots,i_k}_{a,b}$.

We shall often consider the \emph{$k$-th level} of the signature, defined as the finite collection of all terms $S(X)^{i_1,\ldots,i_k}_{a,b}$ where the multi-index is of length $k$. For example, the first level of the signature is the collection of $d$ real numbers $S(X)^1_{a,b}, \ldots, S(X)^d_{a,b}$, and the second level is the collection of $d^2$ real numbers
\begin{eqnarray}
S(X)^{1,1}_{a,b}, \ldots, S(X)^{1,d}_{a,b}, S(X)^{2,1}_{a,b}, \ldots, S(X)^{d,d}_{a,b}.
\end{eqnarray}


\subsubsection{Examples}

\begin{example}[1-dimensional path]
\label{ex:one-dim path}
The simplest example of a signature is that of a 1-dimensional path. In this case our set of indexes (or alphabet) is of size one, $A = \{1\}$, and the set of multi-indexes (or words) is $W = \{(1,\ldots, 1) \mid k \geq 0 \}$, where $1$ appears $k$ times in $(1,\ldots, 1)$.

Consider the path $X : [a,b] \to \R$, $X_t = t$. One can immediately verify that the signature of $X$ is given by
%\begin{align}
%S(X)^\emptyset_{a,b} &= 1, \nonumber\\
%S(X)^1_{a,b} &= X_b - X_a, \nonumber\\
%S(X)^{1,1}_{a,b} &= \frac{(X_b - X_a)^2}{2!}, \nonumber\\
%S(X)^{1,1,1}_{a,b} &= \frac{(X_b - X_a)^3}{3!}, \nonumber\\
%&\vdots\nonumber
%\end{align}
\begin{eqnarray}
    S(X)^\emptyset_{a,b} &=& 1, \nonumber\\
    S(X)^1_{a,b} &=& X_b - X_a, \nonumber\\
    S(X)^{1,1}_{a,b} &=& \frac{(X_b - X_a)^2}{2!}, \nonumber\\
    S(X)^{1,1,1}_{a,b} &=& \frac{(X_b - X_a)^3}{3!}, \nonumber\\
    &\vdots&\nonumber .
\end{eqnarray}
%
One can in fact show that the above expression of the signature remains true for any path $X : [a,b] \to \R$. Hence, for one-dimensional paths, the signature depends only on the increment $X_b - X_a$.
\end{example}



\begin{example}
We present now a more involved example of the signature for a 2-dimensional path. Our set of indexes is now $A = \{1,2\}$, and the set of multi-indexes is
\begin{equation}
W = \{(i_1,\ldots, i_k) \mid k \geq 0, i_1,\ldots, i_k \in \{1,2\} \},
\end{equation}
the collection of all finite sequences of $1$'s and $2$'s.
%In contrast to the previous example, we will see that the signature does not only depend on the increment of the path.
Consider a parabolic path in $\mathbb{R}^2$ as depicted in Fig.~\ref{fig:exampleOf2DimPath} defined by
\begin{eqnarray}\label{eq:differentialsOfPath}
X_t\;&=&\;\{X^1_t,X^2_t\}\;=\;\{3+t,(3+t)^2\}\;\;\;t\in[0,5]\;,\;(a=0, b=5),\\
dX_t\;&=&\;\{dX^1_t,dX^2_t\}\;=\;\{dt,2(3+t)dt\}.\nonumber
\end{eqnarray}
%
\begin{figure}[H]
\centering
\includegraphics[scale=0.5]{artwork/parabolicPath_n.png}
\caption{Example of a 2-dimensional path parametrised in \eqref{eq:differentialsOfPath}.}
\label{fig:exampleOf2DimPath}
\end{figure}
\noindent
%
A straightforward computation gives:
%
\begin{eqnarray}\label{eq:coefficientsOfPath_Example}
S(X)^\emptyset_{0,5} &=& 1, \\\nonumber
S(X)^1_{0,5}\;&=&\;\int_{0<t<5}dX^{1}_t\;=\;\int_{0}^{5}dt\;=\;X^1_5-X^1_0\;=\;5,\\\nonumber
S(X)^2_{0,5}\;&=&\;\int_{0<t<5}dX^{2}_t\;=\;\int_{0}^{5}2\,(3+t)\,dt\;=\;X^2_5-X^2_0\;=\;55,\\\nonumber
S(X)^{1,1}_{0,5}\;&=&\;\iint_{0<t_1<t_2<5}dX^{1}_{t_1} dX^{1}_{t_2}\;=\;\int_{0}^5\left[\int_{0}^{t_2}dt_1\right]dt_2\;=\;\frac{25}{2},\\\nonumber
S(X)^{1,2}_{0,5} \;&=&\;\iint_{0<t_1<t_2<5}dX^{1}_{t_1} dX^{2}_{t_2}\;=\;\int_{0}^5\left[\int_{0}^{t_2}dt_1\right]2\,(3+t_2)\,dt_2\;=\;\frac{475}{3}, \\\nonumber
S(X)^{2,1}_{0,5} \;&=&\;\iint_{0<t_1<t_2<5}dX^{2}_{t_1} dX^{1}_{t_2}\;=\;\int_{0}^5\left[\int_{0}^{t_2}2\,(3+t_1)\,dt_1\right]dt_2\;=\;\frac{350}{3}, \\\nonumber
S(X)^{2,2}_{0,5} \;&=&\;\iint_{0<t_1<t_2<5}dX^{2}_{t_1} dX^{2}_{t_2}\;=\;\int_{0}^5\left[\int_{0}^{t_2}2\,(3+t_1)\,dt_1\right]2\,(3+t_2)\,dt_2=\frac{3025}{2},\\\nonumber
S(X)^{1,1,1}_{0,5}\;&=&\;\iiint_{0<t_1<t_2<t_3<5}dX^{1}_{t_1} dX^{1}_{t_2}dX^{1}_{t_3}=\int_0^5\left[\int_{0}^{t_3}\left[\int_{0}^{t_2}dt_1\right]dt_2\right]dt_3=\frac{125}{6},\\\nonumber
&\vdots&.
\end{eqnarray}
%
Continuing this way, one can compute every term $S(X)^{i_1,\ldots,i_k}_{0,5}$ of the signature for every multi-index $(i_1,\ldots, i_k)$, $i_1,\ldots, i_k \in \{1,2\}$.

%Since the number of terms in signature is infinite (the number of all possible words composed iteratively from two letters), we may {\it truncate} the signature at level $L$ which corresponds to the maximal number of iterated integral or the length of the words. For example, truncated signature at level 2 of the path $X(t)\;=\;\{t,t^2\}, t\in[0,5]$ is given by the collection of coefficients $\mu_{ij}$:
%%
%\begin{eqnarray}
%S^{(L=2)}(X)\;&=&\;\left(1,\mu_1,\mu_2,\mu_{11},\mu_{12},\mu_{21},\mu_{22}\right)\\
%&=&\;\left(1,5,55,\frac{25}{2},\frac{475}{3},\frac{350}{3},\frac{3025}{2}\right)\nonumber
%\end{eqnarray}
%%
%It is worth emphasizing the fact that the first term of signature is always unity.
\end{example}

We will see later examples of paths, namely piecewise linear paths, whose signature can be computed without the need to evaluate integrals, see Example~\ref{ex:piecewise_linear} and Corollary~\ref{cor:Chen_piecewise_linear}.

\subsubsection{Picard iterations: motivation for the signature}\label{subsubsec:Picard}


Before reviewing the basic properties of the signature, we take a moment to show how the signature arises naturally in the classical theory of ordinary differential equations (ODEs). In a sense, this provides one of the first reasons for our interest in the signature.
%We do not provide all the details, but hope that the reader finds the general idea clear.

%Before we dive into proper mathematical description of signature, 
It is instructive to start the discussion with an intuitive and simplistic example of Picard's method. Let us consider the first order ODE
%
\begin{eqnarray}\label{exampleODE_1}
\frac{dy(t)}{dt} = f(t,y(t)),
%\;\;\;\;\; y(a) = y_0,
\end{eqnarray} 
%
where $y:[a,b] \to \R$ is a real valued function of $t\in [a,b]$. Picard's method allows us to construct an approximate solution to \eqref{exampleODE_1} in the form of an iterative series. The integral form of \eqref{exampleODE_1} is given by
%
\begin{eqnarray}
y(t) = y(a) + \int_{a}^t f(s,y(s))\,ds.
\end{eqnarray}

We now define a sequence of functions $y_k(t)$, $k = 0, 1, \ldots$, where the first term is the constant function $y_0(t) = y(a)$, and for $k \geq 1$, we define inductively
%
\begin{eqnarray}
y_{k}(t)\;=\;y(a) + \int_{a}^t f(t,y_{k-1}(s))\,ds.
\end{eqnarray}
%
The classical Picard--Lindel{\"o}f theorem states that, under suitable conditions, the solution to \eqref{exampleODE_1} is given by $y(t) = \lim_{k\rightarrow\infty} y_k(t)$.
%
\begin{example}
Suppose $y:[0,T]\to \R$ solves the ODE
%
\begin{eqnarray}\label{exampleODE_2}
\frac{dy(t)}{dt} = y(t), \;\;\; y(0)=1.
\end{eqnarray}
%
The first $k$ terms of the Picard iterations are given by:
%
\begin{eqnarray}
y_0(t) &=& 1\\
y_1(t) &=& 1 + \int_{0}^t y_0(t)dt = 1 + t\nonumber\\
y_2(t) &=& 1 + \int_{0}^t y_1(t)dt = 1 + t + \frac{1}{2}t^2\nonumber\\
y_3(t) &=& 1 + \int_{0}^t y_2(t)dt = 1 + t + \frac{1}{2}t^2 + \frac{1}{6}t^3\nonumber\\
y_4(t) &=& 1 + \int_{0}^t y_3(t)dt = 1 + t + \frac{1}{2}t^2 + \frac{1}{6}t^3 + \frac{1}{24}t^4\nonumber\\
&\vdots &\nonumber\\
y_k(t) &=& \sum_{n=0}^k \frac{1}{n!}t^n,\nonumber
\end{eqnarray}
%
which converges to $y(t) = e^t$ as $k\rightarrow\infty$, which is indeed the solution to~\eqref{exampleODE_2}. These approximations are plotted in Fig.~\ref{fig:Picard_approximation}.
\end{example}
%
\begin{figure}[ht] 
\centering
    \includegraphics[width=0.9\textwidth]{artwork/pic_examp} 
\caption{Example of sequential Picard approximation to the true solution.}
\label{fig:Picard_approximation}
\end{figure}
\noindent
%
We are now ready to consider a controlled differential equation and the role of the signature in its solution. Consider a path $X : [a,b] \to \R^d$. Let $\LLL(\R^d, \R^e)$ denote the vector space of linear maps from $\R^d$ to $\R^e$. Equivalently, $\LLL(\R^d, \R^e)$ can be regarded as the vector space of $e \times d$ real matrices. For a path $Z : [a,b] \to \LLL(\R^d, \R^e)$, note that we can define the integral
\begin{equation}\label{eq_pathInt}
\int_a^b Z_t dX_t = \int_a^b Z_t(\dot X_t) dt
\end{equation}
as an element of $\R^e$ in exactly the same way as the usual path integral,
where $Z_t(\dot X_t)$ takes values in $\R^e$ for every $t\in[a,b]$.

\begin{example}
Take $d=2$ and $e=3$, so that $\LLL(\R^d, \R^e)$ can be identified with space of matrices $\R^{e\times d}$.
Consider $a=0,b=1$ and
\begin{equation*}
Z_t = \begin{pmatrix}
1 & t\\
t^2 & 0\\
0 & 2\\
\end{pmatrix}
\;,
\qquad
X_t = \begin{pmatrix}
t \\
t^3
\end{pmatrix}
\end{equation*}
for all $t\in [0,1]$.
Then $
\dot X_t = \begin{pmatrix}
1 \\
3t^2
\end{pmatrix}$
and
\begin{equation*}
Z_t (\dot X_t) = \begin{pmatrix}
1+3t^3 \\
t^2 \\
6t^2 \\
\end{pmatrix}\;,
\end{equation*}
so that the integral in \eqref{eq_pathInt} becomes
\begin{equation*}
\int_0^1 Z_t dX_t = 
\int_0^1 Z_t(\dot X_t) dt
=
\begin{pmatrix}
7/4 \\
1/3 \\
2 \\
\end{pmatrix}\;.
\end{equation*}
\end{example}

For a function $V : \R^e \to \LLL(\R^d, \R^e)$ and a path $Y : [a,b] \to \R^e$, we say that $Y$ solves the controlled differential equation
\begin{equation}
dY_t = V(Y_t)dX_t, \; \; Y_a = y \in \R^e,
\end{equation}
precisely when for all times $t \in [a,b]$
\begin{equation}\label{eq_diffEq}
Y_t = y + \int_a^t V(Y_s)dX_s.
\end{equation}
Such equations are ubiquitous in control theory (see e.g. \cite{Agrachev_Sachkov_04,Brockett_15}), where
the map $V$ is often called a collection of \emph{driving vector fields}, the path $X$ is called the \emph{control}, \emph{input}, or the \emph{driver}, and $Y$ is called the \emph{response}, \emph{output}, or the \emph{solution}.

Keeping $X$ fixed, a standard procedure to obtain a solution to~\eqref{eq_diffEq} is through Picard iterations. For an arbitrary path $Y : [a,b] \to \R^e$, define a new path $F(Y) : [a,b] \to \R^e$ by
\begin{equation}\label{eq:F_def}
F(Y)_t = y + \int_a^t V(Y_s)dX_s.
\end{equation}
Observe that $Y$ is a solution to~\eqref{eq_diffEq} if and only if $F(Y)=Y$, i.e. $Y$ is a fixed point of $F$. Consider the sequence of paths $Y^n_t = F(Y^{n-1})_t$ with initial arbitrary path $Y^0_t$ (often taken as the constant path $Y^0_t = y$). The 
Picard--Lindel{\"o}f theorem implies that, under suitable assumptions,
$F$ possesses a unique fixed point $Y$ and that $Y^n_t$ converges to $Y$ as $n \rightarrow \infty$.

Suppose now $V : \R^e \to \LLL(\R^d, \R^e)$ is a \textit{linear} map.
%and let us examine the sequence of paths $Y^n_t$. 
Note that we may equivalently treat $V$ as a  tuple $V=(V_1,\ldots,V_d)$ where each $V_i \in \LLL(\R^e,\R^e)$ is defined by $V_i(y) = V(y)(e_i)$, where $e_1,\ldots,e_d$ are the canonical basis vectors of $\R^d$.
The ODE~\eqref{eq_diffEq} can then be expressed as
\begin{equation}
Y_t = y + \sum_{i=1}^d \int_a^t  V_i(Y_s)\,dX^i_s.
\end{equation}
Let us start the Picard iterations with the initial constant path $Y^0_t = y$ for all $t \in [a,b]$.
It follows from the fact that each $V_i$ is a linear map that the iterates of $F$ given by~\eqref{eq:F_def} are:
%\begin{align*}
%Y^0_t &= y,  \\
%Y^1_t &= y + \sum_{i=1}^d\int_a^t  V_i(Y^0_s)dX^i_s = y+ \sum_{i=1}^d V_i(y)\int_a^t dX^i_s, \\
%Y^2_t &= y + \sum_{i=1}^d\int_a^t  V_i(Y^1_s)dX^i_s = 
%y + \sum_{i=1}^d V_i(y) \int_a^t dX^i_s
%+ \sum_{i,j=1}^d V_i(V_j(y)) \int_a^t \int_a^s dX^j_u dX^i_s, \\
%&\vdots \\
%Y^n_t &= y + \sum_{i=1}^d\int_a^t V_i(Y^{n-1}_s)dX^i_s \\
%&= y+ \sum_{k = 1}^n \sum_{i_1,\ldots,i_k=1}^d V_{i_k}(\ldots(V_{i_1}(y))\ldots)\int_{a < t_1 < \ldots < t_k < t} dX^{i_1}_{t_1}\ldots %dX^{i_k}_{t_k},\\
%&\vdots \; 
%\end{align*}
%
\begin{eqnarray}
Y^0_t &=& y,  \\\nonumber
Y^1_t &=& y + \sum_{i=1}^d\int_a^t  V_i(Y^0_s)dX^i_s = y+ \sum_{i=1}^d V_i(y)\int_a^t dX^i_s, \\\nonumber
Y^2_t &=& y + \sum_{i=1}^d\int_a^t  V_i(Y^1_s)dX^i_s = 
y + \sum_{i=1}^d V_i(y) \int_a^t dX^i_s
+ \sum_{i,j=1}^d V_i(V_j(y)) \int_a^t \int_a^s dX^j_u dX^i_s, \\\nonumber
&\vdots& \\\nonumber
Y^n_t &=& y + \sum_{i=1}^d\int_a^t V_i(Y^{n-1}_s)dX^i_s \\\nonumber
&=& y+ \sum_{k = 1}^n \sum_{i_1,\ldots,i_k=1}^d V_{i_k}(\ldots(V_{i_1}(y))\ldots)\int_{a < t_1 < \ldots < t_k < t} dX^{i_1}_{t_1}\ldots dX^{i_k}_{t_k},\\\nonumber
&\vdots&\nonumber
\end{eqnarray}
%


We recognize in the final expression the signature of $X$
\[
S(X)^{i_1,\ldots,i_k}_{a,t} = \int_{a < t_1 < \ldots < t_k < t} dX^{i_1}_{t_1}\ldots dX^{i_k}_{t_k}.
\]
Furthermore, one can show that the above series converges at every time $t\in[a,b]$, as the following exercise shows.
\begin{exercise}
Show that there exists $C>0$, depending only on the path $X:[a,b]\to \R^d$, the vector fields $V_1,\ldots, V_d\in\LLL(\R^e,\R^e)$, and initial point $y\in\R^e$, such that for all $k \geq 1$ and $t\in [a,b]$,
\begin{equation}\label{eq:factorial decay}
\Big\|\sum_{i_1,\ldots,i_k=1}^d V_{i_k}(\ldots(V_{i_1}(y))\ldots)\int_{a < t_1 < \ldots < t_k < t} dX^{i_1}_{t_1}\ldots dX^{i_k}_{t_k}\Big\| \leq \frac{C^k}{k!}.
\end{equation}
\end{exercise}

The factorial decay in~\eqref{eq:factorial decay} ensures that the limit $\lim_{n\to\infty} Y^n_t$ exists for all $t\in[a,b]$.
The conclusion we obtain is that the solution $Y_t$ is completely determined by the signature $S(X)_{a,t}$ for every $t \in [a,b]$. In particular, if the signatures of two controls $X$ and $\widetilde X$ coincide at time $t \in [a,b]$, that is, $S(X)_{a,t} = S(\widetilde X)_{a,t}$, then the corresponding solutions to~\eqref{eq_diffEq} will also agree at time $t$ for any choice of the linear vector fields $V$.

An important, but far less obvious result, is that the same conclusion holds true for non-linear vector fields $V$. This result was first obtained by Chen~\cite{Chen58} for a certain class of piecewise smooth paths, and more recently extended by Hambly and Lyons~\cite{Hambly10} to paths of bounded variation, and by Boedihardjo, Geng, Lyons and Yang~\cite{Boedihardjo14} to a completely non-smooth setting of geometric rough paths (for which the signature is still well-defined, see Section~\ref{subsec:furtherTopics}). The latter class of paths is of particular interest in stochastic analysis.

We end the discussion on ODEs with one of the motivations behind the applications of signatures in machine learning.
Suppose we have an instrument that is able to detect differences between two points $x,\tilde x\in \R^d$ whenever $|x-\tilde x|>\epsilon$, where $\epsilon >0 $ represents the precision of the instrument.
Suppose we are now given two paths (e.g. time-series) $X,\tilde X:[a,b]\to \R^d$.
What is an effective test to determine whether $X$ and $\tilde X$ differ?
Of course we can apply our instrument to test whether $X_t=\tilde X_t$ for a selection of times $t\in[a,b]$, but this may fail to see a difference in the case that $X$ and $\tilde X$ are very close, e.g. when $\sup_{t\in[a,b]}|X_t-\tilde X_t|<\epsilon$.

A curious fact is that ODEs provide another test that may be more effective.
Namely, suppose the signals $X$ and $\tilde X$ interact with another system that we may observe;
we suppose this system is given by solutions to the ODEs
$dY = V(Y)dX$ and $\tilde Y=V(\tilde Y)d\tilde X$ with $Y(a)=\tilde Y(a)$.
Then, to determine if $X$ and $\tilde X$ differ, we can instead apply our instrument to test whether $Y_b \neq \tilde Y_b$; indeed, $Y_b \neq \tilde Y_b$ clearly implies $X\neq\tilde X$.
While this statement may at first appear void of interest,
it turns out that the difference between $Y$ and $\tilde Y$ may be much easier to detect than the difference between $X$ and $\tilde X$, i.e. it is possible that $\sup_t |X_t-\tilde X_t|<\epsilon$ while $Y_b-\tilde Y_b$ is much larger than $\epsilon$ -- see Figure~\ref{fig:ODE_diff} for an illustration.
As stated above, the signatures $S(X)_{a,b}, S(\tilde X)_{a,b}$ completely determine the solutions $Y_b,\tilde Y_b$ respectively
(and in fact themselves can be seen as solutions to linear ODEs driven by $X,\tilde X$),
which motivates the signature as a descriptive feature of time-ordered data.



\begin{figure}
\centering
    \begin{minipage}{.49\textwidth}
        \centering
        $X$ 
        \includegraphics[trim=10mm 10mm 10mm 10mm,clip,height=43mm]{artwork/SDE_W_N=10000.png}
    \end{minipage}%
    \begin{minipage}{0.49\textwidth}
        \centering
        $d Y_t = V(Y_t) d X_t$ 
        \includegraphics[trim=8mm 10mm 10mm 10mm,clip,height=43mm]{artwork/SDE_X_N=10000.png}
    \end{minipage}

    \vspace{6mm}
    \begin{minipage}{.49\textwidth}
        \centering
        $\tilde X$ 
        \includegraphics[trim=10mm 10mm 10mm 10mm,clip,height=43mm]{artwork/SDE_W_per_N=10000.png}
    \end{minipage}%
   \begin{minipage}{0.49\textwidth}
        \centering
        $d \tilde Y_t = V(\tilde Y_t)d \tilde X_t$ 
        \includegraphics[trim=8mm 10mm 10mm 10mm,clip,height=43mm]{artwork/SDE_X_per_N=10000.png}
    \end{minipage}
    \caption{The two paths $X,\tilde X : [0,T]\to \R^2$
    are close in uniform norm: $X$ is an approximation of Brownian motion and $\tilde X$ is a small perturbation of $\tilde X$ at every point. The horizontal axis denotes times and the orange and blue lines indicate the two components $X^1,X^2$, likewise for $\tilde X$.
    The solutions $Y,\tilde Y:[0,T] \to \R$ to the same ODE driven by $X,\tilde X$ respectively, however, differ significantly.}
    \label{fig:ODE_diff}
\end{figure}


\subsubsection{Geometric intuition for the first two levels}\label{subsubsec:geoIntuition}


While the signature is defined analytically using path integrals, we briefly discuss here the geometric meaning of the first two levels. As already mentioned, the first level, given by the terms $(S(X)^1_{a,b},\ldots, S(X)^d_{a,b})$, is simply the increment of the path $X : [a,b] \to \R^d$.
% (as can be seen, for example, in~\eqref{eq:coefficientsOfPath_Example}).
For the second level, the term $S(X)^{i,i}_{a,b}$ is equal to $(X^i_b-X^i_a)^2/2$; this relation is a special case of the shuffle product which we
review in Section~\ref{subsubsec:shuffle}. To give meaning to the term $S(X)^{i,j}_{a,b}$ for $i \neq j$, consider the {\it L\'evy area} (illustrated in Fig.~\ref{fig:exampleOfSignedLevyArea})% for $i=1$ and $j=2$)
, which is a {\it signed} area enclosed by the path (solid red line) and the chord (blue straight dashed line) connecting the endpoints. The L{\'e}vy area of a 2-dimensional path $\{X^1_t,X^2_t\}$ is given by
%
\begin{eqnarray}\label{eq:LevyArea}
A\;=\;\frac{1}{2}\left(S(X)^{1,2}_{a,b}-S(X)^{2,1}_{a,b}\right).
\end{eqnarray}
See Section~\ref{sec:signature_of_a_path} for an example computation of the signature where this geometric meaning is further highlighted.
%
%In the next Fig.\ref{fig:exampleOfSignedLevyArea} we demonstrate the signed area enclosed by a path $X : [a,b] \to \R^2$ (red) and a straight line (blue dotted chord) connecting the two endpoints. 
%
\begin{figure}[H]
\centering
\includegraphics[width=1.0\textwidth]{artwork/curve_1.png}
\caption{Example of the signed L\'evy area of a curve.
Areas above and under the chord connecting the two endpoints are negative and positive ares and are denoted by $A_{-}$ and $A_{+}$ respectively. The increments along each coordinate are denoted by $\Delta X^1$ and $\Delta X^2$.
}
\label{fig:exampleOfSignedLevyArea}
\end{figure}
\noindent


%The higher order terms in signature are less intuitively interpretable in terms of geometrical objects, so we will not seek any explanations beyond the second level of truncation. Concluding this part, we would like to draw readers' attention to the fact, that the explicit computation of all infinite terms of signature are straightforward and conceptually clear. Computing more terms of signature will reveal more information about the path in close analogy to Taylor approximation of functions, where more terms of expansion approximate better the original function. It was shown [cite Terry and others] that using non-truncated signature (which contains infinite number of terms) one can recover the original path $X$ from the inverse transformation of signature if this path, namely:





==> section_files_tex/1_3.tex <==
\subsection{Important properties of signature}
\label{subsec:important_properties}


We now review several fundamental properties of the signature, providing complete proofs for most of them. Several deeper results are discussed in the following Section~\ref{subsec:furtherTopics}, but only on an informal level.

\subsubsection{Invariance under time reparametrisations}
\label{subsubsec:repar_invar}

We call a surjective, continuous, non-decreasing function $\psi : [a,b] \to [a,b]$ a \emph{reparametrization}. For simplicity, we shall only consider smooth reparametrizations, although, just like in the definition of the path integral, this is not strictly necessary. 

Let $X, Y : [a,b] \to \R$ be two real-valued paths and $\psi : [a,b] \to [a,b]$ a reparametrization. Define the paths $\widetilde X, \widetilde Y : [a,b] \to \R$ by $\widetilde X_t = X_{\psi(t)}$ and $\widetilde Y_t = Y_{\psi(t)}$. Observe that
\begin{eqnarray}
\dot{\widetilde X}_t = \dot{X}_{\psi(t)} \dot{\psi}(t),
\end{eqnarray}
from which it follows that
\begin{eqnarray}
\int_a^b \widetilde Y_t d\widetilde X_t = \int_a^b Y_{\psi(t)} \dot{X}_{\psi(t)} \dot{\psi}(t) dt = \int_a^b Y_u dX_u,
\end{eqnarray}
where the last equality follows by making the substitution $u = \psi(t)$. This shows that path integrals are invariant under a time reparametrization of both paths.

Consider now a multi-dimensional path $X : [a,b] \to \R^d$ and a reparametrization $\psi:[a,b] \to [a,b]$. As before, denote by $\widetilde X :[a,b] \to \R^d$ the reparametrized path $\widetilde X_t = X_{\psi(t)}$. Since every term of the signature $S(X)^{i_1,\ldots,i_k}_{a,b}$ is defined as an iterated path integral of $X$, it follows from the above that
\begin{eqnarray}
S(\widetilde X)^{i_1,\ldots,i_k}_{a,b} = S(X)^{i_1,\ldots,i_k}_{a,b}, \; \; \forall k \geq 0, \; i_1,\ldots, i_k \in \{1,\ldots, d\}.
\end{eqnarray}
That is to say, the signature $S(X)_{a,b}$ is invariant under time reparametrizations of $X$.



\subsubsection{Shuffle product}\label{subsubsec:shuffle}

As alluded to in the introduction, the signature is a natural generalisation of polynomials to the space of (possibly unparametrised) paths. We already saw a simple example of this in Example~\ref{ex:one-dim path} where the signature of a 1-dimensional path encodes the powers of its increment.


The way that signatures generalise polynomials to multi-dimensional paths is through the \textit{shuffle product identity}.
This identity, shown originally by Ree~\cite{Ree58}, implies that the product of two terms $S(X)^{i_1,\ldots, i_k}_{a,b}$ and $S(X)^{j_1,\ldots, j_m}_{a,b}$ can always be expressed as a sum of another collection of terms of $S(X)_{a,b}$ which only depends on the multi-indexes $(i_1,\ldots, i_k)$ and $(j_1,\ldots, j_m)$;
this is akin to how to the product of two polynomials is again a polynomial.
More precisely, 
$$S(X)^{i_1,\ldots, i_k}_{a,b}S(X)^{j_1,\ldots, j_m}_{a,b} = \sum_K S(X)^K_{a,b},$$
where the sum is over all multi-indexes $K$
obtained by `shuffling' $(i_1,\ldots, i_k)$ and $(j_1,\ldots, j_m)$ together in a way that preserves their respective orders.
See Example~\ref{ex:shuffle_polynomials} for a relation with classical multiplication of polynomials, as well as Section~\ref{subsec:normalised_moments} 
for the relevance of the shuffle product to statistical learning.

To make this statement precise, we next define the shuffle product of two multi-indexes. For integers $k,m\geq 0$, a permutation $\sigma$ of the set $\{1,\ldots, k+m\}$ is called a $(k,m)$-shuffle if $\sigma^{-1}(1) < \ldots < \sigma^{-1}(k)$ and $\sigma^{-1}(k+1) < \ldots < \sigma^{-1}(k+m)$.
The list $(\sigma(1),\ldots, \sigma(k+m))$ is also called a shuffle of $(1,\ldots, k)$ and $(k+1,\ldots, k+m)$.

\begin{example}
Consider $k=2$ and $m=3$ and the permutation $\sigma : \{1,\ldots, 5\} \to \{1,\ldots, 5\}$ defined by
\[
(\sigma(1),\sigma(2),\sigma(3),\sigma(4),\sigma(5)) = (3,1,4,5,2).
\]
Then $\sigma$  is a $(2,3)$-shuffle, i.e., $(3,1,4,5,2)$ is a shuffle of $(1,2)$ and $(3,4,5)$, because
\[
\sigma^{-1}(1)=2 < \sigma^{-1}(2) = 5 \quad \text{and} \quad
\sigma^{-1}(3)=1 < \sigma^{-1}(4) = 3 < \sigma^{-1}(5)=4.
\]
\end{example}


\begin{definition}[Shuffle product]
Let $\Shuffles(k,m)$ denote the set of all $(k,m)$-shuffles.
Consider two multi-indexes $I = (i_1,\ldots, i_k)$ and $J = (j_1,\ldots, j_m)$ with $i_1,\ldots,i_k,j_1,\ldots, j_m \in \{ 1,\ldots, d\}$. Define the multi-index
\begin{eqnarray}
(r_1,\ldots, r_k, r_{k+1}, \ldots r_{k+m}) = (i_1,\ldots, i_k, j_1,\ldots, j_m).
\end{eqnarray}
The shuffle product of $I$ and $J$, denoted $I \shuffle J$, is a finite multi-set of multi-indexes of length $k+m$ defined as follows
\begin{eqnarray}
I \shuffle J = \{(r_{\sigma(1)},\ldots, r_{\sigma(k+m)}) \mid \sigma \in \Shuffles(k,m) \}.
\end{eqnarray}
\end{definition}

\begin{example}
The following example shows the shuffle product between $(1,2,1)$ and $(2,3)$, which we color in red and blue 
respectively to distinguish the elements of the two multi-indexes (we drop parentheses for notaional simplicity):
\begin{eqnarray}
\rd{121} \shuffle \nb{23}
= \{\rd{121}\nb{23},\rd{12}\nb{2}\rd{1}\nb{3},
\rd{1}\nb{2}\rd{21}\nb{3}, \nb{2}\rd{121}\nb{3},
\rd{12}\nb{23}\rd{1},
\rd{1}\nb{2}\rd{2}\nb{3}\rd{1}, \nb{2}\rd{12}\nb{3}\rd{1}, \rd{1}\nb{23}\rd{21},
\nb{2}\rd{1}\nb{3}\rd{21},\nb{23}\rd{121}\}.\nonumber
\end{eqnarray}
\end{example}

We make several important remarks about the above definition.
\begin{enumerate}
\item The number of elements in $I \shuffle J$ is $\binom{k+m}{k}$, which is equal to the total number of $(k,m)$-shuffles.

\item $I \shuffle J$ is a \textit{multi-set} (not just a set) as it may contain multiple instances of a single multi-index, e.g. $(i)\shuffle (i) = \{(i,i),(i,i)\}$ for any $i\in\{1,\ldots, d\}$ since both permutations of $\{1,2\}$ are $(1,1)$-shuffles.

\item The shuffle product is \textit{commutative}, that is, $I\shuffle J=J\shuffle I$.

\item If $k=0$, then $I\shuffle J$ is a singleton containing the multi-index $J$.
\end{enumerate}

\begin{theorem}[Shuffle product identity]\label{thm:shuffle}
Consider a path $X : [a,b] \to \R^d$ and two multi-indexes $I = (i_1,\ldots, i_k)$ and $J = (j_1,\ldots, j_m)$ with $i_1,\ldots,i_k,j_1,\ldots, j_m \in \{ 1,\ldots, d\}$. Then
\begin{eqnarray}\label{eq:shuffle_iden}
S(X)^I_{a,b} S(X)^J_{a,b} = \sum_{K \in I \shuffle J} S(X)^K_{a,b}.
\end{eqnarray}
\end{theorem}


\begin{proof}
For $k=0$, we have $I=\emptyset$, and thus $I\shuffle J$ is a singleton containing the multi-index $J$.
In this case~\eqref{eq:shuffle_iden} becomes $S(X)^\emptyset_{a,b} S(X)^J_{a,b} = S(X)^J_{a,b}$, which is true since $S(X)^\emptyset_{a,b}=1$ by definition.
This proves the result for $k=0$, and, by symmetry, for $m=0$.

It remains to consider $k,m\geq 1$.
We proceed by induction on $k+m$.
For the inductive step, suppose~\eqref{eq:shuffle_iden} holds for all (possibly empty) multi-indexes of combined length $k+m-1$.
Then for $I$ and $J$ as in the theorem statement,
\begin{align*}
S(X)^I_{a,b} S(X)^J_{a,b}
&= \int_a^b S(X)^{i_1,\ldots, i_{k-1}}_{a,s} d X^{i_k}_s
\int_a^b S(X)^{j_1,\ldots, j_{m-1}}_{a,t} d X^{j_m}_t
\\
&= \int_{s,t\in[a,b]^2} S(X)^{i_1,\ldots ,i_{k-1}}_{a,s}
S(X)^{j_1,\ldots, j_{m-1}}_{a,t}
d X^{i_k}_sd X^{j_m}_t
\\
&=
\int_{a<s<t<b} S(X)^{i_1,\ldots, i_{k-1}}_{a,s}d X^{i_k}_s S(X)^{j_1,\ldots, j_{m-1}}_{a,t}d X^{j_m}_t
\\
&\qquad +\int_{a<t<s<b} S(X)^{j_1\ldots j_{m-1}}_{a,t}
d X^{j_m}_t
S(X)^{i_1\ldots i_{k-1}}_{a,s}d X^{i_k}_s
\\
&=
\int_{a}^b S(X)^{I}_{a,t}
S(X)^{j_1\ldots j_{m-1}}_{a,t}
d X^{j_m}_t
+\int_{a}^b S(X)^{J}_{a,s}
S(X)^{i_1\ldots i_{k-1}}_{a,s}d X^{i_k}_s
\\
&=
\int_{a}^b \sum_{K\in I\shuffle j_1\ldots j_{m-1}} S(X)^{K}_{a,t}
d X^{j_m}_t
+\int_{a}^b \sum_{K\in i_1\ldots i_{k-1}\shuffle J} S(X)^{K}_{a,s}d X^{i_k}_s\;,
\end{align*}
where we used Fubini's theorem in the second equality and the inductive hypothesis together with the earlier cases $m-1=0$ or $k-1=0$ in the final equality.
We finally remark the combinatorial identity
\begin{align*}
I\shuffle J
&= \{(K , j_m)\,:\, K\in I\shuffle (j_1,\ldots, j_{m-1})\}
\cup \{(K , i_k)\,:\, K\in (i_1,\ldots, i_{k-1})\shuffle J\}\;,
\end{align*}
where the two sets on the right-hand side are disjoint and
the proof of which is left as an exercise for the reader.
We thus obtain~\eqref{eq:shuffle_iden} for $I,J$ of combined length $k+m$ for $k,m\geq 1$,
which completes the inductive step.
\end{proof}


\begin{example}
Consider a 2-dimensional path $X : [a,b] \to \R^2$. The shuffle product identity \eqref{eq:shuffle_iden} implies that
\begin{eqnarray}
S(X)^1_{a,b} S(X)^2_{a,b} &=& S(X)^{1,2}_{a,b} + S(X)^{2,1}_{a,b},\nonumber
\\
S(X)^{1,2}_{a,b} S(X)^1_{a,b} &=& 2 S(X)^{1,1,2}_{a,b} + S(X)^{1,2,1}_{a,b}.\nonumber
\end{eqnarray}
\end{example}
%
\begin{example}\label{ex:shuffle_polynomials}
We now show that the shuffle product generalises the familiar multiplication of (multivariate) polynomials.

As the simplest example, consider the one-dimensional case with $x\in \R$ and the linear path $X:[0,1]\to \R$, $X_t=tx$.
Following Example~\ref{ex:one-dim path},
for any multi-index $(1,\ldots, 1)$ of length $k$,
\begin{eqnarray}\label{eq:poly_sig}
S(X)^{1,\ldots, 1}_{0,1} = \frac{x^k}{k!}.
\end{eqnarray}
Consider two multi-indexes $I$ and $J$ of length $k$ and $m$ (consisting only of $1$'s).
Then, by~\eqref{eq:poly_sig},
\begin{eqnarray}\label{eq:1D_shuffle_1}
S(X)^{I}_{0,1}S(X)^{J}_{0,1} = \frac{x^{k+m}}{k!m!}.
\end{eqnarray}
On the other hand, there are $\binom{k+m}{k}$ ways to shuffle $I$ and $J$, and all shuffles lead to the same multi-index with $1$ appearing $k+m$ times.
Therefore, by~\eqref{eq:shuffle_iden},
\begin{eqnarray}\label{eq:1D_shuffle_2}
S(X)^{I}_{0,1}S(X)^{J}_{0,1} = \binom{k+m}{k}\frac{x^{k+m}}{(k+m)!}.
\end{eqnarray}
Since $\binom{k+m}{k}=(k+m)!/(k!m!)$, we see that the expressions~\eqref{eq:1D_shuffle_1} and~\eqref{eq:1D_shuffle_2} match.

Consider now the multi-dimensional case $x=(x_1,\ldots,x_d)\in \R^d$ and the linear path $X:[0,1]\to \R^d$, $X_t=tx$ as before.
For $I=(i_1,\ldots,i_k)$, one can verify that
\begin{eqnarray}\label{eq:poly_sig_beta}
S(X)^{I}_{0,1} = \frac{x_1^{\beta_1}\cdots x_d^{\beta_d}}{k!},
\end{eqnarray}
where $\beta_n$ is the number of times $n$ appears in $i_1,\ldots, i_k$.
In particular, $S(X)^{I}_{0,1}$ depends only on the elements in $I$, not their order,
and encodes a multivariate monomial of $x$.

It follows that, for another multi-index $J=(j_1,\ldots,j_m)$,
\begin{eqnarray}\label{eq:dD_shuffle}
S(X)^{I}_{0,1}S(X)^{J}_{0,1} = \frac{x_1^{\beta_1+\gamma_1}\cdots x_d^{\beta_d+\gamma_d}}{k!m!},
\end{eqnarray}
where $\gamma_n$ is the number of times $n$ appears in $j_1,\ldots,j_m$.

On the other hand, there are again $\binom{k+m}{k}$ multi-indexes in $I\shuffle J$, which may now be distinct, but each $n\in\{1,\ldots, d\}$ appears $\beta_n+\gamma_n$ times in each multi-index in $I\shuffle J$.
Therefore, by~\eqref{eq:shuffle_iden},
\begin{eqnarray}
S(X)^{I}_{0,1}S(X)^{J}_{0,1} = \binom{k+m}{k}\frac{x^{\beta_1+\gamma_1}_1\cdots x_d^{\beta_d+\gamma_d}}{(k+m)!},
\end{eqnarray}
which again agrees with~\eqref{eq:dD_shuffle}.
\end{example}
%
The shuffle product implies that the product of two terms of the signature can be expressed as a linear combination of higher order terms. This fact has important theoretical and practical consequences, some of which we discuss in Section~\ref{subsec:normalised_moments}.


\subsubsection{Chen's identity}
\label{subsubsec:Chen}

We now describe a property of the signature known as Chen's identity, which provides an algebraic relationship between paths and their signatures. It furthermore provides a powerful tool in the computation of the signature once its value is known on subintervals (see Example~\ref{ex:piecewise_linear} below).
The simplest version of Chen's identity is the following.

\begin{theorem}[Chen's identity]\label{thm:Chen_1}
Suppose $a<b<c$ and $X:[a,c]\to \R^d$ is a path.
Then for any multi-index $(i_1, \ldots, i_k)$
\begin{eqnarray}\label{eq:Chen_1}
S(X)^{i_1,\ldots, i_k}_{a,c} = \sum_{m=0}^k S(X)^{i_1,\ldots, i_m}_{a,b} S(X)^{i_{m+1},\ldots, i_k}_{b,c}.
\end{eqnarray}
\end{theorem}

\begin{proof}
We proceed by induction on $k$. The case $k=0$ is obvious since both the left- and right-hand sides are equal to $1$ in this case.
Suppose now~\eqref{eq:Chen_1} holds for $k-1$ with $k\geq 1$.
Then
\begin{align*}
S(X)^{i_1,\ldots, i_k}_{a,c}
&=\int_a^b S(X)^{i_1,\ldots, i_{k-1}}_{a,t} d X_t^{i_k} + \int_b^c S(X)^{i_1,\ldots ,i_{k-1}}_{a,t} d X_t^{i_k}
\\
&= S(X)^{i_1,\ldots, i_{k}}_{a,b}
+\int_b^c \sum_{m=0}^{k-1} S(X)^{i_1,\ldots ,i_{m}}_{a,b}S(X)^{i_{m+1},\ldots ,i_{k-1}}_{b,t}
 d X_t^{i_k}
\\
&=  S(X)^{i_1,\ldots, i_{k}}_{a,b} + \sum_{m=0}^{k-1}
S(X)^{i_1,\ldots, i_{m}}_{a,b}S(X)^{i_{m+1},\ldots, i_{k-1}, i_k}_{b,c}
\\
&= \sum_{m=0}^{k}
S(X)^{i_1,\ldots, i_{m}}_{a,b}S(X)^{i_{m+1}, \ldots, i_k}_{b,c}\;,
\end{align*}
where we used the inductive hypothesis in the second equality.
\end{proof}

The next example shows that Chen's identity is an effective method to compute the signatures of piecewise linear paths.

\begin{example}[Signature of piecewise linear path]
\label{ex:piecewise_linear}
Consider the path
$X\colon[0,2]\to\R^2$ which is linear on the intervals $[0,1]$ and $[1,2]$ and
$X_0 = (3,0), X_1=(3,1), X_2=(0,1)$,  see Figure~\ref{fig:piecewise_linear_path}.

 \begin{figure}
\centering
      \begin{tikzpicture}
          \begin{axis}[
			  unit vector ratio*=1 1 1,
              height       = 1.9in,
%			  x			   = 0.5,
%			  y			   = 0.5,
              xmax         = 3.3,
              ymax         = 1.3,
			  grid=both,
              xtick        = {0.0, 1,2, 3.0},
              xticklabels  = {0, $1$,$2$,$3$},
              ytick        = {0.0, 1 },
              yticklabels  = {0, $1$},
              axis lines   = center,
              line cap=round
              ]
              \addplot[->,color=red,very thick] coordinates { (3,1) (0,1) };
              \addplot[->,color=red,very thick] coordinates { (3,0) (3,1) };
          \end{axis}
      \end{tikzpicture}
\caption{}\label{fig:piecewise_linear_path}
\end{figure}
Then
\begin{align*}
(S(X)^{\emptyset}_{0,1},S(X)^2_{0,1},S(X)^{22}_{0,1}) &= (1,1,1/2)\;,
\end{align*}
with $S(X)^{I}_{0,1} = 0$ for all other multi-indexes $I$ of length at most $2$,
and
\begin{align*}
(S(X)^{\emptyset}_{1,2},S(X)^1_{1,2},S(X)^{11}_{1,2}) &= (1,-3,9/2)\;,
\end{align*}
with $S(X)^{I}_{1,2} = 0$ for all other multi-indexes $I$ of length at most $2$.

Then by Chen's identity
\begin{align*}
(S(X)^{1}_{0,2},S(X)^{2}_{0,2})
&= (S(X)^{1}_{0,1} + S(X)^{1}_{1,2},S(X)^{2}_{0,1} + S(X)^{2}_{1,2})
\\
&= (-3+0,0+1)\;,
\end{align*}
as expected from the fact that $S(X)^i_{a,b}=X^i_b-X^i_a$.
Furthermore, again by Chen's identity,
\begin{align*}
S(X)^{12}_{0,2}
&= S(X)^{12}_{0,1} + S(X)^{1}_{0,1}S(X)^{2}_{1,2} + S(X)^{12}_{1,2}
= 0 + 0\times 0 + 0 = 0,
\\
S(X)^{21}_{0,2}
&= S(X)^{21}_{0,1} + S(X)^{2}_{0,1}S(X)^{1}_{1,2} + S(X)^{21}_{1,2}
= 0 + 1\times (-3) + 0 = -3,
\end{align*}
which is less obvious and which is consistent with the L\'evy area identity \eqref{eq:LevyArea}.
\end{example}

There is a way to formulate
Chen's identity in a more algebraic way.
To do so, we need to introduce the algebra of formal power series, which should appear natural in light of the definition of the signature.

\begin{definition}[Formal power series]\label{def:formal_power_series}
Let $e_1,\ldots, e_d$ be $d$ formal indeterminates. The algebra of (non-commuting) \emph{formal power series} in $d$ indeterminates is the vector space of all formal series of the form
\begin{eqnarray}
\sum_{k = 0}^\infty \sum_{i_1,\ldots, i_k \in \{1,\ldots d\}} \lambda_{i_1,\ldots,i_k}e_{i_1}\ldots e_{i_k},
\end{eqnarray}
where the second summation runs over all multi-indexes $(i_1,\ldots, i_k)$, $i_1,\ldots, i_k \in \{1,\ldots, d\}$, and $\lambda_{i_1,\ldots, i_k}$ are real numbers.
\end{definition}

A (non-commuting) formal polynomial is a formal power series for which only a finite number of coefficients $\lambda_{i_1,\ldots, i_k}$ are non-zero. The terms $e_{i_1}\ldots e_{i_k}$ are called monomials. The term corresponding to $k = 0$ is simply just a real number $\lambda_0$.
The space of formal power series is also called the \emph{space of tensor series} over $\R^d$.
We stress that the power series we consider are non-commutative; for example, the elements $e_1e_2$ and $e_2e_1$ are distinct.

The space of formal power series may be naturally equipped with a vector space structure by defining addition and scalar multiplication as
\begin{multline}
\left(\sum_{k = 0}^\infty \sum_{i_1,\ldots, i_k \in \{1,\ldots d\}} \lambda_{i_1,\ldots,i_k}e_{i_1}\ldots e_{i_k}\right) +
\left(\sum_{k = 0}^\infty \sum_{i_1,\ldots, i_k \in \{1,\ldots d\}} \mu_{i_1,\ldots,i_k}e_{i_1}\ldots e_{i_k}\right) \\
= \sum_{k = 0}^\infty \sum_{i_1,\ldots, i_k \in \{1,\ldots d\}} (\lambda_{i_1,\ldots,i_k} + \mu_{i_1,\ldots, i_k})e_{i_1}\ldots e_{i_k}
\end{multline}
and
\begin{eqnarray}
c\left(\sum_{k = 0}^\infty \sum_{i_1,\ldots, i_k \in \{1,\ldots d\}} \lambda_{i_1,\ldots,i_k}e_{i_1}\ldots e_{i_k}\right) 
= \sum_{k = 0}^\infty \sum_{i_1,\ldots, i_k \in \{1,\ldots d\}} c\lambda_{i_1,\ldots,i_k}e_{i_1}\ldots. e_{i_k}.
\end{eqnarray}

Moreover, one may define the product $\otimes$ between monomials by joining together multi-indexes
\begin{eqnarray}
e_{i_1}\ldots e_{i_k} \otimes e_{j_1}\ldots e_{j_m} = e_{i_1}\ldots e_{i_k}e_{j_1}\ldots e_{j_m}.
\end{eqnarray}
The product $\otimes$ then extends uniquely and linearly to all power series. We demonstrate the first few terms of the product in the following expression
\begin{multline}\label{eq:otimes_example}
\left(\sum_{k = 0}^\infty \sum_{i_1,\ldots, i_k \in \{1,\ldots d\}} \lambda_{i_1,\ldots,i_k}e_{i_1}\ldots e_{i_k}\right)
\otimes \left(\sum_{k = 0}^\infty \sum_{i_1,\ldots, i_k \in \{1,\ldots d\}} \mu_{i_1,\ldots,i_k}e_{i_1}\ldots e_{i_k} \right) \\
= \lambda_0\mu_0 + \sum_{i=1}^d (\lambda_0\mu_i + \lambda_i\mu_0)e_i + \sum_{i,j=1}^d \left( \lambda_0 \mu_{i,j} + \lambda_i\mu_j + \lambda_{i,j}\mu_0\right)e_ie_j + \ldots.
\end{multline}
The space of formal power series becomes an algebra when equipped with this vector space structure and product $\otimes$, i.e. $\otimes$ is associative and distributive over addition.
Note, however, that $\otimes$ is not commutative as \eqref{eq:otimes_example} demonstrates.


The reader may have noticed that the indexing set of the monomials $e_{i_1}\ldots e_{i_k}$ coincides with the indexing set of the terms of the signature of a path $X : [a,b] \to \R^d$, namely the collection of all multi-indexes $(i_1,\ldots, i_k)$, $i_1,\ldots, i_k \in \{1,\ldots, d\}$. It follows that a convenient way to express the signature of $X$ is by a formal power series where the coefficient of each monomial $e_{i_1}\ldots e_{i_k}$ is set to be $S(X)^{i_1,\ldots, i_k}_{a,b}$. We use the same symbol $S(X)_{a,b}$ to denote this representation
\begin{eqnarray}
S(X)_{a,b} = \sum_{k = 0}^\infty  \sum_{i_1,\ldots, i_k \in \{1,\ldots d\}} S(X)^{i_1,\ldots, i_k}_{a,b} e_{i_1}\ldots e_{i_k},
\end{eqnarray}
where, as before, the ``0-th'' level of the signature is $S(X)^\emptyset_{a,b} = 1$ (corresponding to $k=0$).

\begin{example}\label{ex:linear_path_sig}
Consider $x=(x_1,\ldots, x_d)\in\R^d$ as a formal power series by
$(x^1,\ldots, x^d) \mapsto \sum_{i=1}^d x^ie_i$.
For $x\in \R^d$, define the power series $e^x$ by
\[
e^x = \sum_{k=0}^\infty \frac{x^{\otimes k}}{k!} = \sum_{k=0}^\infty \frac{(\sum_{i=1}^d x^ie_i)^{\otimes k}}{k!}\;.
\]
Explicitly, the coefficient of $e_{i_1}\ldots e_{i_k}$ in $e^x$ is $x_1^{\beta_1}\ldots x_d^{\beta_d}/k!$,
where $\beta_n$ is the number of times $n$ appears in $i_1,\ldots, i_k$.

Then, for the path $X:[0,1]\to\R^d$ defined by $X_t=tx$, one has
\[
S(X)_{0,1} = e^x\;,
\]
which is essentially the claim we saw already in~\eqref{eq:poly_sig_beta} from Example~\ref{ex:shuffle_polynomials}.
\end{example}

To state Chen's identity in an algebraic way, it remains to define the concatenation of paths.

\begin{definition}[Concatenation]
For two paths $X : [a,b] \to \R^d$ and $Y: [b,c] \to \R^d$, we define their \emph{concatenation} as the path $X * Y : [a,c] \to \R^d$ for which $(X * Y)_t = X_t$ for $t \in [a,b]$ and $(X * Y)_t = X_b + (Y_t - Y_b)$ for $t \in [b,c]$.
\end{definition}

\begin{figure}
\[
      \begin{tikzpicture}
          \begin{axis}[
			  unit vector ratio*=1 1 1,
			  disabledatascaling,
              height       = 1.6in,
              xmax         = 3.3,
xmin         = -1.3,
              ymax         = 4.3,
			  grid=both,
              xtick        = {-1,0.0, 1,2, 3.0},
              xticklabels  = {$-1$, $0$, $1$,$2$,$3$},
              ytick        = {0.0, 1,2,3,4 },
              yticklabels  = {0, $1$,$2$,$3$,$4$},
              axis lines   = center,
              line cap=round,
              ]
              \addplot[->,color=red,very thick] coordinates { (3,1) (0,1) };
              \addplot[->,color=red,very thick] coordinates { (3,0) (3,1) };
			 \draw[very thick, color=blue, ->] (2,2) arc (-90:180:1);
\node at (2.5, 0.5) () {\small{$X$}};
\node at (2.5, 3) () {\small{$Y$}};
          \end{axis}
      \end{tikzpicture}
\qquad  \qquad
      \begin{tikzpicture}
          \begin{axis}[
			  unit vector ratio*=1 1 1,
			  disabledatascaling,
              height       = 1.6in,
              xmax         = 3.3,
xmin         = -1.3,
              ymax         = 4.3,
			  grid=both,
              xtick        = {-1,0.0, 1,2, 3.0},
              xticklabels  = {$-1$, $0$, $1$,$2$,$3$},
              ytick        = {0.0, 1,2,3,4 },
              yticklabels  = {0, $1$,$2$,$3$,$4$},
              axis lines   = center,
              line cap=round,
              ]
              \addplot[->,color=red,very thick] coordinates { (3,1) (0,1) };
              \addplot[->,color=red,very thick] coordinates { (3,0) (3,1) };
			 \draw[very thick, color=blue, ->] (0,1) arc (-90:180:1);
\node at (1.9, 1.5) () {\small{$X*Y$}};
          \end{axis}
      \end{tikzpicture}
\]
\caption{Example of two paths $X$ and $Y$ and the resulting concatenation $X*Y$.}\label{fig:concat_example}
\end{figure}

See Figure~\ref{fig:concat_example} for a visual depiction of concatenation.
Observe that the space of paths forms a semigroup with concatenation $*$ as the product.
We can now recast Chen's identity (Theorem~\ref{thm:Chen_1}) in an algebraic light, namely that the signature is a semigroup morphism from the space of paths, equipped with concatenation, into the space of formal power series equipped with the product $\otimes$. More precisely, we have the following result.

\begin{theorem}[Chen's identity]\label{thm:Chen_2}
For two paths $X : [a,b] \to \R^d$ and $Y: [b,c] \to \R^d$,
\begin{eqnarray}
S(X * Y)_{a,c} = S(X)_{a,b} \otimes S(Y)_{b,c}.
\end{eqnarray}
\end{theorem}

The contents of Theorems~\ref{thm:Chen_1} and~\ref{thm:Chen_2} are identical.
We only state the latter version of Chen's identity to highlight a useful algebraic structure.
In particular, it allows us to state the following corollary that extends the computations from Examples~\ref{ex:piecewise_linear} and \ref{ex:linear_path_sig}.

\begin{corollary}[Signature of piecewise linear path]\label{cor:Chen_piecewise_linear}
Let $X: [0,n] \to \R^d$ be a path that is linear on each interval $[0,1],\ldots,[n-1,n]$.
Then
\[
S(X)_{0,n} = e^{X_1-X_0} \otimes\ldots \otimes e^{X_n-X_{n-1}}\;.
\]
\end{corollary}

\subsubsection{Time-reversal}

The time-reversal property informally states that the signature $S(X)_{a,b}$ of a path $X : [a,b] \to \R^d$ is precisely the inverse under the product $\otimes$ of the signature obtained from running $X$ backwards in time. To make this precise, we make the following definition.

\begin{definition}[Time-reversal]
For a path $X : [a,b] \to \R^d$, we define its time-reversal as the path $\overleftarrow X : [a,b] \to \R^d$ for which $\overleftarrow X_t = X_{a + b-t}$ for all $t \in [a,b]$.
\end{definition}

See Figure~\ref{fig:time_revers} for a depiction of the time reversal of paths.

\begin{figure}
\[
      \begin{tikzpicture}
          \begin{axis}[
			  unit vector ratio*=1 1 1,
			  disabledatascaling,
              height       = 1.6in,
              xmax         = 3.3,
xmin         = -1.3,
              ymax         = 4.3,
			  grid=both,
              xtick        = {-1,0.0, 1,2, 3.0},
              xticklabels  = {$-1$, $0$, $1$,$2$,$3$},
              ytick        = {0.0, 1,2,3,4 },
              yticklabels  = {0, $1$,$2$,$3$,$4$},
              axis lines   = center,
              line cap=round,
              ]
              \addplot[->,color=red,very thick] coordinates { (3,1) (0,1) };
              \addplot[->,color=red,very thick] coordinates { (3,0) (3,1) };
			 \draw[very thick, color=blue, ->] (2,2) arc (-90:180:1);
\node at (2.5, 0.5) () {\small{$X$}};
\node at (2.5, 3) () {\small{$Y$}};
          \end{axis}
      \end{tikzpicture}
\qquad  \qquad
      \begin{tikzpicture}
          \begin{axis}[
			  unit vector ratio*=1 1 1,
			  disabledatascaling,
              height       = 1.6in,
              xmax         = 3.3,
xmin         = -1.3,
              ymax         = 4.3,
			  grid=both,
              xtick        = {-1,0.0, 1,2, 3.0},
              xticklabels  = {$-1$, $0$, $1$,$2$,$3$},
              ytick        = {0.0, 1,2,3,4 },
              yticklabels  = {0, $1$,$2$,$3$,$4$},
              axis lines   = center,
              line cap=round,
              ]
              \addplot[->,color=red,very thick] coordinates { (0,1) (3,1) };
              \addplot[->,color=red,very thick] coordinates {  (3,1) (3,0) };
			 \draw[very thick, color=blue, ->] (1,3) arc (180:-90:1);
\node at (2.5, 0.5) () {\small{$\overleftarrow X$}};
\node at (2.5, 3) () {\small{$\overleftarrow Y$}};
          \end{axis}
      \end{tikzpicture}
\]
\caption{Example of two paths $X$ and $Y$ and their respective reversals $\overleftarrow{X}$ and $\overleftarrow{Y}$.}\label{fig:time_revers}
\end{figure}

\begin{theorem}[Time-reversed signature]\label{thm:time_revers}
For a path $X : [a,b] \to \R^d$, it holds that
\begin{eqnarray}\label{eq:time_rever}
S(X)_{a,b} \otimes S(\overleftarrow X)_{a,b} = 1.
\end{eqnarray}
Explicitly, for all multi-indexes $(i_1,\ldots, i_k)$,
\begin{eqnarray}\label{eq:reversal_identity}
S(\overleftarrow X)^{i_1,\ldots ,i_k}_{a,b}=(-1)^kS(X)^{i_k,\ldots, i_1}_{a,b}.
\end{eqnarray}
\end{theorem}

\begin{remark}
The element $1$ in~\eqref{eq:time_rever} should be understood as the formal power series where $\lambda_0 = 1$ and $\lambda_{i_1,\ldots, i_k} = 0$ for all $k \geq 1$ and $i_1,\ldots, i_k \in \{1,\ldots, d\}$, which is the identity element under the product $\otimes$.
\end{remark}

\begin{proof}
We will prove~\eqref{eq:reversal_identity}.
As before, we proceed by induction.
The claim is clearly true for $k=0$ since $S(X)_{a,b}^\emptyset=1$.
Suppose now that~\eqref{eq:reversal_identity} is true for some $k-1\geq 0$.
Then
\begin{eqnarray}
S(\overleftarrow X)^{i_1,\ldots ,i_k}_{a,b} &=&
\int_a^b S(\overleftarrow X)^{i_1,\ldots ,i_{k-1}}_{a,t} d\overleftarrow X^{i_k}_t
\\
&=& \int_a^b (-1)^{k-1}S(X)^{i_{k-1},\ldots ,i_{1}}_{a+b-t,b} dX^{i_k}_{a+b-t}
\\
&=&\int_a^b (-1)^{k}S(X)^{i_{k-1},\ldots ,i_{1}}_{s,b} dX^{i_k}_{s}
\\
&=& (-1)^{k}S(X)^{i_k,i_{k-1},\ldots ,i_{1}}_{a,b},
\end{eqnarray}
where we used the inductive hypothesis in the second equality, the change of variable $s=a+b-t$ in the third equality,
and in the final equality we used the identity
\begin{eqnarray}
S(X)^{j_1,\ldots ,j_k}_{a,b} = \int_a^b S(X)^{j_2,\ldots ,j_k}_{t,b} dX^{j_1}_t
\end{eqnarray}
which itself follows from~\eqref{eq:iter_int_rep}.
\end{proof}




\subsubsection{Log signature}\label{subsubsec:logSig}

We now define a transform of the path signature called the log signature. The log signature is nothing but the logarithm of the signature in the algebra of formal power series.
For a power series
\begin{eqnarray}
x = \sum_{k = 0}^\infty \sum_{i_1,\ldots, i_k \in \{1,\ldots d\}} \lambda_{i_1,\ldots,i_k}e_{i_1}\ldots e_{i_k}
\end{eqnarray}
for which $\lambda_0 > 0$, define its logarithm as the power series given by
\begin{eqnarray}
\log x = \log(\lambda_0) - \sum_{n \geq 1}\frac{1}{n}\left(1-\frac{x}{\lambda_0}\right)^{\otimes n},
\end{eqnarray}
where $\otimes n$ denotes the $n$-th power with respect to the product $\otimes$.

In the case that $\lambda_0=1$, which is the most important case for us, the logarithm reduces to
\begin{eqnarray}
\log x = -\sum_{n \geq 1}\frac{1}{n}\left(1 - x\right)^{\otimes n}.
\end{eqnarray}


For example, for a real number $\lambda \in \R$ and the series
\begin{eqnarray}
x = 1 + \sum_{k \geq 1} \frac{\lambda^k}{k!} e_{1}^{\otimes k},
\end{eqnarray}
one can readily check that
\begin{eqnarray}
\log x = \lambda e_1.
\end{eqnarray}

In general, $\log x$ is a series with an infinite number of terms. However for every multi-index $(i_1,\ldots, i_k)$, the coefficient of $e_{i_1}\ldots e_{i_k}$ in $\log x$ depends only on the coefficients of $x$ of the form $\lambda_{j_1,\ldots,j_m}$ with $m \leq k$, of which there are only finitely many, so that $\log x$ is well-defined without the need to consider convergence of infinite series.


\begin{definition}[Log signature]
For a path $X : [a,b] \to \R^d$, the log signature of $X$ is defined as the formal power series $\log S(X)_{a,b}$.
\end{definition}

For two formal power series $x$ and $y$, let us define their Lie bracket by
\begin{eqnarray}\label{eq:lie_brackets}
[x,y] = x\otimes y - y \otimes x.
\end{eqnarray}
A direct computation shows that the first few terms of the log signature are given by
\begin{eqnarray}\label{eq:direct_computation_logsig}
\log S(X)_{a,b} = \sum_{i=1}^d S(X)^i_{a,b}e_i + \sum_{1 \leq i < j \leq d} \frac{1}{2}\left(S(X)^{i,j}_{a,b}-S(X)^{j,i}_{a,b}\right)[e_i,e_j] + \ldots.
\end{eqnarray}
In particular one can see that the coefficient of the polynomials $[e_i,e_j]$ in the log signature is precisely the L{\'e}vy area introduced in Section~\ref{subsubsec:geoIntuition}.

\begin{example}
Consider the two-dimensional path
\begin{eqnarray}
X : [0,2] \to \R^2, \; \; X_t = 
\begin{cases} \{t,0\} &\mbox{if } t \in [0,1], \\ 
\{1,t-1\} &\mbox{if } t \in [1,2].
\end{cases}
\end{eqnarray}
Note that $X$ is the concatenation of the two linear paths, $Y : [0,1] \to \R^2$, $Y_t = \{t,0\}$, and $Z:[1,2] \to \R^2$, $Z_t \to \{1,t-1\}$. One can readily check (see Example~\ref{ex:linear_path_sig}) that the signatures of $Y$ and $Z$ (as formal power series) are given by
\begin{eqnarray}
S(Y)_{0,1} = 1 + \sum_{k \geq 1} \frac{1}{k!}e_{1}^{\otimes k}, \; \; S(Z)_{1,2} = 1 + \sum_{k \geq 1} \frac{1}{k!}e_{2}^{\otimes k}.
\end{eqnarray}
It follows by Chen's identity that
\begin{eqnarray}
S(X)_{0,2} = S(Y)_{0,1} \otimes S(Z)_{1,2} = 1 + e_1 + e_2 + \frac{1}{2!}e_1e_1 + \frac{1}{2!}e_2e_2 + e_1e_2 + \ldots.
\end{eqnarray}
Hence the first few terms of the log signature of $X$ are
\begin{eqnarray}
\log S(X)_{0,2} = e_1 + e_2 + \frac{1}{2}[e_1,e_2] + \ldots.
\end{eqnarray}
\end{example}

In fact, one can readily check that coefficients of $\log S(X)_{0,2}$ in the above example are given precisely by the classical Baker--Campbell--Hausdorff formula.

The above example demonstrates the general fact that the log signature can always be expressed as a power series composed entirely of so-called Lie polynomials. This is the content of the following theorem due to Chen~\cite{Chen57}, which generalizes the Baker--Campbell--Hausdorff theorem.

\begin{theorem}\label{thm:log_sig_Lie}
Let $X : [a,b] \to \R^d$ be a path. Then there exist real numbers $\lambda_{i_1,\ldots, i_k}$ such that 
\begin{eqnarray}\label{thm:log_sig_series}
\log S(X)_{a,b} = \sum_{k \geq 1} \sum_{i_1,\ldots, i_k \in \{1,\ldots, d\}} \lambda_{i_1,\ldots, i_k} [e_{i_1},[e_{i_2},\ldots,[e_{i_{k-1}},e_{i_k}]\ldots ]].
\end{eqnarray}
\end{theorem}

Note that the coefficients $\lambda_{i_1,\ldots, i_k}$ are in general not unique since the polynomials of the form $[e_{i_1},[e_{i_2},\ldots,[e_{i_{k-1}},e_{i_k}]\ldots ]]$ are not linearly independent (e.g., $[e_1,e_2] = -[e_2,e_1]$).

Theorem \ref{thm:log_sig_Lie} is the only result in this subsection which we do not prove since all proofs, to our knowledge, require a non-trivial detour into Lie algebras.
See \cite[Cor.~3.5]{Reutenauer93} or \cite[Sec.~7.5]{FrizVictoir10} for two (different) proofs.

==> section_files_tex/1_4.tex <==
\subsection{Expected signatures as moments of path-valued random variables}
\label{subsec:normalised_moments}

We saw in Example~\ref{ex:shuffle_polynomials}
that the signature generalises multivariate polynomials to the space of paths
and that the shuffle product (Theorem~\ref{thm:shuffle})
generalises the classical product of polynomials.
In this subsection, we highlight the relevance of these observations to the theory of statistical learning by interpreting the expectation of the signature as the moments of path-valued random variables.
We suppose the reader is familiar with the basics of probability theory, such as measures and expectation;
see, e.g.~\cite{Billingsley12} for background material.
See also Section~\ref{subsubsec:moments} for a further discussion on signatures, moments of random variables, and the Fourier transform.

Consider a probability measure $\PP$ on $\R$.
The moments of $\PP$, defined as the numbers $\int_\R x^k \PP(dx)$ for $k=0,1,\ldots$,
encode important information about $\PP$ (whenever they are well-defined)
and play a prominent role in statistics.
To see why, we recall the classical Weierstrass approximation theorem.

\begin{theorem}[Weierstrass 1885]\label{thm:Weierstrass}
Let $f:[a,b]\to\R$ be a continuous function and $\epsilon>0$. Then there exists a polynomial $p(x)=a_0+a_1x+\cdots +a_kx^k$ with real coefficients $a_i$ such that $|f(x)-p(x)| < \epsilon$ for all $x\in[a,b]$.
\end{theorem}

The relevance of this theorem to probability theory is that the expectation
\[
\PP(p) := \int_\R p(x) \PP(dx)
\]
of any polynomial $p$ under $\PP$ is determined by the moments of $\PP$ due to linearity of integration.
Furthermore, recall that two probability measure $\PP$ and $\QQ$ are equal if and only if $\PP(f)=\QQ(f)$ for all continuous functions $f:\R\to\R$, see~\cite{Billingsley12}. These two remarks provide a simple way to test whether two probability measures on a finite interval are equal.

\begin{corollary}\label{cor:moments}
Suppose $\PP$ and $\QQ$ are probability measures on $[a,b]$. Then $\PP=\QQ$ if and only if the moments of $\PP$ and $\QQ$ are equal.
\end{corollary}

\begin{proof}
The direction $\Rightarrow$ is obvious, so we prove now $\Leftarrow$.
Consider $f:[a,b]\to\R$ continuous and let $\epsilon>0$.
By Theorem~\ref{thm:Weierstrass} there exists a polynomial $p$ such that $|f(x)-p(x)|<\epsilon$ for all $x\in[a,b]$.
In particular, by the triangle inequality applied to integrals, $|\PP(f)-\PP(p)|<\epsilon$ and likewise for $\QQ$.
But since $\PP(p)=\QQ(p)$ by the assumption that the moments of $\PP$ and $\QQ$ match, we see that $|\PP(f)-\QQ(f)|<2\epsilon$.
Since $\epsilon$ was arbitrary, it follows that $\PP(f)=\QQ(f)$ for any continuous function $f:[a,b]\to\R$ and thus $\PP=\QQ$. 
\end{proof}

\begin{remark}\label{rem:Carleman}
It is crucial that $\PP$ and $\QQ$ in the above theorem are defined on a bounded interval $[a,b]$ instead of on $\R$.
Indeed, one can find two probability measures on $\R$ whose moments match but which are distinct.
Nonetheless, there exists an essentially sharp criterion on the growth rate of the moments of $\PP$ (Carelman's condition) which guarantees that $\PP$ is  determined by its moments, see~\cite{Carleman_cond_98}.
\end{remark}

We now recall a substantial generalisation of Theorem~\ref{thm:Weierstrass}, known as the Stone--Weierstrass theorem (see~\cite[Theorem~7.32]{Rudin76}).

\begin{theorem}\label{thm:SW}
Let $\mcX$ be a compact space. Suppose $\mcF$ is a vector space of functions $f\colon\mcX\to \R$ such that
\begin{enumerate}[label=(\roman*)]
    \item every $f\in\mcF$ is continuous,
\item the constant function $1$ is in $\mcF$
\item\label{pt:algebra} for every $f,g\in\mcF$, one has $fg\in\mcF$, and
\item\label{pt:point_sep} for all distinct $x,y\in\mcX$, there exists $f\in\mcF$ such that $f(x)\neq f(y)$.
\end{enumerate}
Then, for any continuous function $g\colon\mcF\to\R$ and $\epsilon>0$, there exists $f\in\mcF$ such that
$|f(x)-g(x)|<\epsilon$ for all $x\in\mcX$.
\end{theorem}

Put more succinctly, every point-separating algebra of 
continuous functions that contains $1$ is dense in $C(\mcX) = \{f:\mcX\to\R,\:\, f \textnormal{ is continuous}\}$.
(`Algebra' refers to item~\ref{pt:algebra} and `point-separating' refers to item~\ref{pt:point_sep}.)
We leave it as an exercise for the reader to verify that if $\mcX=[a,b]$ and $\mcF$ is the space of polynomials, then $\mcF$ verifies the assumptions of Theorem~\ref{thm:SW}, and thus Theorem~\ref{thm:SW} implies Theorem~\ref{thm:Weierstrass}.

Turning back to the path signature, let $\mcX$ denote 
the set of paths $X:[a,b]\to\R^d$ that we equip with the bounded variation norm $\|X\|_{BV} := |X_a| + \int_a^b |\dot X_t|dt$.
Let $\mcF$ denote the space of all functions $f:\mcX\to \R$ of the form
\begin{equation}\label{eq:mcF}
X \mapsto \sum_{i=1}^n \lambda_i S(X)^{I_i}_{a,b},
\end{equation}
where $n\geq 1$, $\lambda_i\in\R$, and $I_i$ is a mutli-index.
We claim that all the conditions of Theorem~\ref{thm:SW} \textit{except}~\ref{pt:point_sep} are satisfied:
\begin{enumerate}[label=(\roman*)]
\item For the every multi-index $I$, the function $X\mapsto S(X)^I_{a,b}$ is continuous,
%(for the bounded variation norm),
the verification of which we leave as an exercise for the reader,
hence every $f\in\mcF$ is continuous.

\item Since $S(X)^\emptyset_{a,b}=1$, we clearly have $1\in\mcF$.

\item For the every multi-index $I$ and $J$, by the shuffle product (Theorem~\ref{thm:shuffle}), the function $X\mapsto S(X)^I_{a,b}S(X)^J_{a,b}$ is in $\mcF$,
which implies that $fg\in\mcF$ whenever $f,g\in\mcF$.
\end{enumerate}
Unfortunately, it is clear that the point-separating property~\ref{pt:point_sep} is not satisfied. There are three reasons for this:
%(listed in increasing order of severity):
\begin{itemize}
    \item The signature is base-point invariant, i.e. $S(X)_{a,b}=S(X+x)_{a,b}$, so no two paths that differ by a shift in $\R^d$ can be separated by functions in $\mcF$.
    \item The signature is parametisation invariant (see Section~\ref{subsubsec:repar_invar}), so no two paths that differ by a reparametrisation of $[a,b]$ can be separated.
   \item By Chen's identity (Theorem~\ref{thm:Chen_2}) and the time-reversal property (Theorem~\ref{thm:time_revers}), if $X$ can be written as $X=Y*\overleftarrow Y$ for a path $Y$, then $S(X)_{a,b} = 1$ (understood as the formal power series), which is equal to the signature of a constant path $Z$, i.e. $Z_t=z$ for all $t\in[a,b]$ for some fixed $z\in\R^d$.
   Therefore, $X$ and $Z$ cannot be separated, i.e. $f(X)=f(Z)$ for all $f\in\mcF$.
\end{itemize}
Nonetheless, it is possible to recover~\ref{pt:point_sep} after a suitable adjustment of the space of paths $\mcX$.
The minimal adjustment necessary to achieve~\ref{pt:point_sep}
is to suitably quotient $\mcX$ by the kernel of $S$, which is known to consist of all tree-like paths (see Section~\ref{subsubsec:path_uniqueness}).

However, we will demonstrate a simpler, more pragmatic approach to achieve~\ref{pt:point_sep}, which is to shrink $\mcX$.
More precisely, let us fix $y\in\R^{d-1}$ and consider the set of paths
\[
\mcY = \{Y = (Y^1,\ldots, Y^d) \colon[a,b]\to\R^d  \,:\, \forall t\in[a,b]\;\; Y^1_t=t,\;\; Y_a = (a,y)\in\R^d \} \subset \mcX.
\]
In plain words, $\mcY$ consists of those path $Y\colon [a,b]\to\R^d$ in $\mcX$ such that $Y^1$ is the time-component and whose initial point is $(a,y)$.
(The fact that the first component is time, is not at all crucial. What is crucial is that every $Y\in\mcY$ is of them form $Y_t=(f_t,\bar Y_t)$ for some fixed strictly monotone function $f:[a,b]\to\R$.)
The next result shows that the signature separates the points of $\mcY$.

\begin{proposition}\label{prop:signature_unique}
Suppose that $X,Y\in\mcY$ with $S(X)^I_{a,b}=S(Y)^I_{a,b}$ for all multi-indexes $I$.
Then $X=Y$.
\end{proposition}

\begin{proof}
Recall from Example~\ref{ex:one-dim path} that $S(X)^{1,\ldots,1}_{a,t}=\frac{(t-a)^k}{k!}$ where `$1$' appears $k$ times in $1,\ldots,1$.
Then,
for any $i=2,\ldots,d$,
\begin{equation}
    S(X)^{1,\ldots, 1, i}_{a,b} = \int_a^b S(X)^{1,\ldots,1}_{a,t}\dot X^i_t dt = \int_a^b \frac{(t-a)^k}{k!} \dot X^i_t dt.
\end{equation}
It follows that the sequence $S(X)^{i}_{a,b},S(X)^{1,i}_{a,b},S(X)^{1,1, i}_{a,b},\ldots$
encodes all the \textit{moments} of the functions $\{\dot X^i_t\}_{i=2}^d$, and thus uniquely determines $\dot X^i$
(we leave this implication as an exercise to the reader with the hint that one should use Theorem~\ref{thm:Weierstrass}).
Since $S(X)=S(Y)$, it follows that $\dot X=\dot Y$.
Since $X_a= Y_a$, it follows that $X=Y$.
\end{proof}

We therefore see that the set of functions $\mcF$ defined by~\eqref{eq:mcF} separates the points of $\mcY$.
Consequently, as we already verified all the other conditions for Theorem~\ref{thm:SW}, we obtain the following result which shows that arbitrary continuous functions on paths can be approximated by linear functions of the signature.
%for every compact set $K\subset \mcY$ and a continuous function $g\colon K\to \R$ and $\epsilon>0$, there exists $f\in\mcF$ such that $|f(X)-g(X)|<\epsilon$ for all $X\in K$.

\begin{proposition}\label{prop:SW_paths}
    Consider a compact set $K\subset \mcY$, continuous function $g\colon K\to \R$, and $\epsilon>0$.
    Then there exists $f\in\mcF$ such that $|f(X)-g(X)|<\epsilon$ for all $X\in K$.
    More precisely, there exists an integer $n\geq 1$, real numbers $\lambda_1,\ldots,\lambda_n$,
    and multi-indexes $I_1,\ldots, I_n$ such that, for all $X\in K$,
    \[
    \Big|g(X) - \sum_{i=1}^n \lambda_i S(X)^{I_i}_{a,b}\Big| < \epsilon.
    \]
\end{proposition}

By precisely the same argument used to prove Corollary~\ref{cor:moments}, we obtain the following corollary of Proposition~\ref{prop:SW_paths} that justifies the title of this subsection.

\begin{corollary}\label{cor:moment_prob_compact}
    Suppose $\PP$ and $\QQ$ are probability measures on a compact set $K\subset\mcY$ with equal expected signatures, i.e. $\int_K S(X)^I_{a,b} \PP(dX)=\int_K S(X)^I_{a,b} \QQ(dX)$ for all multi-indexes $I$.
    Then $\PP=\QQ$.
\end{corollary}

\begin{remark}
It is possible to significantly extend this result, in particular dropping the assumption that $\PP$ and $\QQ$ are defined on a compact subset of paths,
%In particular, it is known that many stochastic processes, e.g. multi-dimensional Brownian motion (with time added as a component),
%are uniquely determined in law by their expected signatures,
see Section~\ref{subsubsec:moments}.
\end{remark}




==> section_files_tex/1_5.tex <==
\subsection{Further topics and extensions}\label{subsec:furtherTopics}

We conclude the first part of these notes with a brief discussion on several more advanced topics.
In particular, we discuss
\begin{enumerate}
    \item the signature of rough paths,
    \item the extent to which the signature determines the underlying path,
    \item extensions to jump processes,
    \item the role of the signature in the moment problem for random paths,
    \item extensions to higher dimensions.
\end{enumerate}

\subsubsection{Rough paths}\label{subsubsec:roughPaths}

Our discussion of the signature has so far been restricted to paths which are piecewise differentiable (or more generally of bounded variation). This restriction was needed to ensure that the iterated integrals of the path existed as Riemann-Stieltjes integrals. More generally, one can define the iterated integrals of a path using the Young integral for any path of finite $p$-variation with $1 \leq p < 2$. The Young integral goes beyond the ``classical'' definition of the integral and is already able to cover a class of paths substantially more irregular than those of bounded variation. 
%However its role in stochastic analysis remains limited due to the fact that sample paths of Brownian motion have almost surely infinite $p$-variation for $p \leq 2$ (but have almost surely finite $p$-variation for any $p > 2$).  remains limited in stochastic analysis due to the properties of 

A problem that arises for paths of infinite $p$-variation for all $p < 2$ (which is a situation of great interest in stochastic analysis due to the fact that the sample paths of Brownian motion have almost surely finite $p$-variation if and only if $p > 2$), is that one can show there is no well-defined notion of an iterated integral for such paths. We stress that this is not due to any technical limitation of the Young integral, but rather due to the fact that there is no unique candidate for the iterated integrals. That is to say, there is not necessarily only one unique way to define the iterated integrals.

One of the key observations of T. Lyons in his introduction of rough paths in~\cite{Lyons1998} was that if one \emph{defines} the first $\floor{p}$ iterated integrals of a path $X$ of finite $p$-variation, then there is a unique way to obtain all the other iterated integrals, and hence the signature of $X$. This notion of a path of finite $p$-variation, along with its first $\floor p$ iterated integrals (which may be defined arbitrarily provided that they satisfy Chen's identity and possess finite $p$-variation), is precisely the definition of a $p$-rough path.

A key result in the theory of rough paths, known as the \emph{universal limit theorem}, is that one is able to give meaning to controlled differential equations where the driver is a so-called \emph{geometric} $p$-rough path, and where the solution depends in a continuous way on the driver provided that the space of $p$-rough paths is equipped with a suitable topology (known as the $p$-variation metric).
We refer the interested reader to the St. Flour lecture notes of Lyons--Caruana--L{\'e}vy~\cite{Lyons07} for an introduction to the theory of rough paths and to the monograph of Friz--Hairer~\cite{FrizHairer14} for a recent treatment of the topic.
%that naturally leads to an introduction of Hairer's theory of regularity structures in the study of stochastic partial differential equations.

\subsubsection{Path uniqueness}
\label{subsubsec:path_uniqueness}

As discussed in Section~\ref{subsubsec:Picard}, the signature of a path $X : [a,b] \mapsto \R^d$ is all that is needed to determine the endpoint of the solution to a linear (and, less trivially, non-linear) differential equation driven by $X$.
This was first shown by Chen~\cite{Chen58} in the smooth setting, and later extended by Hambly--Lyons~\cite{Hambly10} and Boedihardjo--Geng--Lyons--Yang~\cite{Boedihardjo14} to less regular paths.
The works of these authors in fact shows that the signature captures deep geometric properties of a path, which we briefly discuss here.

A natural question one may ask is the following: is a path completely determined by its signature?
The answer is no for the reasons described above Proposition~\ref{prop:signature_unique}.
For example, one can never recover from the signature the exact speed at which the path is traversed (due to invariance under time reparametrizations), nor can one tell apart the signature of a trivial constant path and that of a path concatenated with its time-reversal.

However, a highly non-trivial fact is that this is essentially the only information one loses from the signature.
For example, for a path $X$ which never crosses itself, the signature is able to completely describe the image and direction of traversal of the path (that is, all the points that $X$ visits and the order in which it visits them), modulo its starting point.
This demonstrates the signature's ability to completely determine the geometric properties of a path which does not possess degeneracies consisting of movements going directly back onto itself.
More precisely, it is shown in~\cite{Hambly10, Boedihardjo14} that, for two paths $X,Y$, one has $S(X)= S(Y)$ if and only if $X$ and $Y$ are \emph{tree-like equivalent}.
It remains however a challenging problem to effectively recover properties of a path from its signature: see Lyons--Xu~\cite{LyonsXu15I, LyonsXu15II} and Geng~\cite{Geng15} for progress on this question.

\subsubsection{Paths with jumps}

For many theoretical and practical applications, it is necessary to consider paths with jumps (i.e. discontinuous paths).
This is important, for example, in finance~\cite{ContTankov04}, superdiffusive dynamical systems~\cite{CFKM20,MZ15},
and queuing theory~\cite{Whitt02}.
It turns out that, under suitable regularity assumptions on the path (satisfied, for example, by almost every sample path of semi-martingales),
there exists a meaningful way to build a signature.

The basic idea is to connect the jumps of a discontinuous path $X:[a,b]\to \R^d$ with straight lines by adding an `infinitesimal' extra time $\delta$ to the interval.
The resulting object is a continuous path $X^\delta:[a,b+\delta] \to \R^d$, for which the signature can be computed as normal and is independent of the extra time $\delta$.
For example, if $X$ is piecewise constant with finitely many jumps, the signature of $X^\delta$ is the same as that of the piecewise linear path connecting the jumps of $X$ in the respective order.
This procedure to build a continuous path $X^\delta$ from $X$ works under natural regularity assumptions, e.g. for $X$ c\`adl\`ag (right-continuous with left-limits), and does not require that $X$ has finitely many jumps.
These ideas stem from the work of Marcus~\cite{Marcus78,Marcus80} (see also~\cite{KPP95, Applebaum09,ChechkinPavlyukevich14} and the references therein)
and later developed in the context of rough paths~\cite{Williams01,FS17,Chevyrev18,CF19} (see in particular~\cite{Chevyrev18,CF19} where the requirement that the jumps of $X$ are connected with straight lines is relaxed).

We mention also another way to interpret rough paths with jumps that relies on so-called forward (or It\^o) integration~\cite{FZ17} and also leads to a notion of signature, but the resulting object is most naturally interpreted in the sense of branched rough paths~\cite{Gubinelli10} as it no longer satisfies the shuffle product identity.


\subsubsection{Moment problem and random paths}
\label{subsubsec:moments}

The moment problem in probability theory is the following: given two probability measures $\PP$ and $\QQ$ on $\R$ with equal moments, i.e. $\int_\R x^k\PP(dx) = \int_\R x^k\QQ(dx)$ for all $k \geq 0$,
does it hold that $\PP=\QQ$?
As alluded to Remark~\ref{rem:Carleman}, the answer is, in general, negative, but there exist sufficient (and necessary) conditions on the growth of the moments  $\int_\R x^k\PP(dx)$ under which the answer is positive.

Recall also from Section~\ref{subsec:normalised_moments}, especially Corollary~\ref{cor:moment_prob_compact},
that the shuffle product identity and the Stone--Weierstrass theorem together imply that
a probability measure on a \textit{compact} set of paths (on which the signature map is injective) is uniquely determined by its expected signature.
This gives a positive answer to the moment problem in the simplest possible case (compact support of measures).

Given that, for probability measures on $\R$, compactness of support is a sufficient but not necessary condition to solve the moment problem,
it is natural to ask whether one can relax the compactness assumption in the solutoin to the moment problem for signatures.
The answer turns out to be `yes' and the following sufficient condition was found in~\cite{CL16}:
provided that the expectations $\mathbb{E}[S(X)^{i_1,\ldots,i_k}_{a,b}]$ decay with $k$ faster than any geometric sequence, then these expectations uniquely determine the law of $S(X)_{a,b}$.\footnote{It is necessary to speak of the \textit{law of the signature} $S(X)_{a,b}$
instead of the \textit{law of the path} $X$ because the signature does not, in general, uniquely determined the path, see Proposition~\ref{prop:signature_unique} and the discussion beforehand.}

The condition of \cite{CL16} is satisfied, for example, by classes of L{\'e}vy processes including Brownian motion (suitably interpreted as geometric rough paths), for which the expected signature is explicitly known~\cite{FS17},
and for classes of Gaussian and Markovian processes for which the expected signature is not explicitly known~\cite{CassOgrodnik17,CL16}.
In turn, it is known~\cite{BDMN21,LiNi22} that certain processes (e.g. Brownian motion stopped upon exiting a domain) do \textit{not} satisfy the necessary moment decay condition of~\cite{CL16}, and it remains open whether the law of their signatures is determined by its expected value.
A related open problem is to find sufficient and \textit{necessary} conditions for a solution to the moment problem for signatures, akin to the sharp Carelman's condition (see Remark~\ref{rem:Carleman}).

The method used in~\cite{CL16} to resolve the moment problem for signatures is to introduce a suitable noncommutative Fourier transform, which, as in the classical case, uniquely determines the law of any random variable without any assumptions on the moments.
Again for L\'evy processes, it is possible to derive a L\'evy--Khintchine formula that determines the Fourier transform explicitly, see~\cite[Sec.~5.3.2]{Chevyrev18}.

\subsubsection{Higher dimensions}

%\ilya{Just added this section - see if it makes sense.}

We conclude this section by mentioning several recent works that aim to extend the concept of signatures to functions defined over \textit{multi-dimensional space}, i.e. functions $X:\Omega \to \R^d$ where $\Omega\subset \R^n$ and possibly $n\geq 1$, instead of just paths $X\colon[a,b]\to\R^d$.
Due to lack of a canonical ordering on points in $\R^n$ for $n\ge 2$, it is non-trivial how to extend the notion of signature to such $X$ in a way that preserves properties like the shuffle product and Chen's identity from Section~\ref{subsec:important_properties}.
Nonetheless, such an extension clearly has value since many types of data, e.g. images, are spatial (vs. temporal) and lack a time-ordered structure.

Zhang--Lin--Tindel~\cite{ZLT22}, inspired by~\cite{Tindel_Chouk_15}, recently defined 2D signatures and applied this concept to image and texture classification.
Their approach was based on rectangular increments and was restricted to level-1 and level-2 (generalisations of) signatures.
Giusti--Lee--Nanda--Oberhauser~\cite{GLNO22} provided an elegant (essentially topological) extension of signatures based on cubical mapping spaces
that applies to arbitrary dimension and to arbitrary level.
The authors therein show generalisations of the shuffle product and Chen's identity
and are able to partially address the uniqueness question discussed in Section~\ref{subsubsec:path_uniqueness}.
See also~\cite{CGW21} that provides a candidate for a multi-dimensional signature based on the notion of a \textit{model} from the theory of regularity structures~\cite{Hairer14}, which is used in the analysis of singular stochastic partial differential equations.
This generalisation, however, relies on several (a priori ad hoc) choices, including an integration operator that replaces the (somewhat canonical) Heaviside function in the one-dimensional case; it remains open if important properties of the signature extend to this construction.
Finally, we mention \cite{2022arXiv221014247D} that introduces two-parameter sums signatures with applications to a multi-dimensional version of dynamic time warping.

==> section_files_tex/2_1.tex <==
\section{Practical Applications}

One of the practical applications of the signature transformation lies in the field of machine learning algorithms. As already been discussed, the signature summarises important information about a path. When the path is composed of a sequential data stream $\{X_i\}$, the terms of the signature $S(X)^{ijk...}$ are good candidates for characteristic {\it features} of the data stream. The shuffle product property allows us to represent a non-linear function of the signature as a linear combination of iterated integrals. This is similar to basis function expansion and naturally applies to computations of regression models.
In the next sections we will demonstrate numerical computations of signatures of paths from various data streams and applications of signatures to machine learning problems, namely classification.


\subsection{Elementary ingredients and their properties}% with signature transformation}

In the following sections we introduce the essential ingredients of the signature method, demonstrate how to perform basic computations and applications to machine learning.

\subsubsection{Paths from discrete data}
\label{subsubsec:paths_from_discrete_data}

Our initial task is to transform discrete sequential (i.e., time-series) data into continuous paths, as signatures are typically defined for continuous paths, rather than a collection of discrete data points. We start with basic computations of the signature applied to data streams. Let $X$ be a data stream defined as a set of $N$ points observed at times $t_0 < t_1 < t_2 < ... < t_N$ in $d$-dimensions ($X\in\mathbb{R}^d$):
%
\begin{eqnarray}\label{eq:data_stream}
X=\left\{\Bigl(X^{1}_{t_i},X^2_{t_i},X^3_{t_i},...,X^d_{t_i}\Bigr)\right\}_{i=0}^N.
\end{eqnarray}
One can think of $\Bigl(X^{1}_{t_i},X^2_{t_i},X^3_{t_i},...,X^d_{t_i}\Bigr)$ as a coordinate of a data point recorded at time $i$ in $\mathbb{R}^d$.
%
For example, consider two one-dimensional sequences of length four:
%
\begin{eqnarray}
\{X^1_{t_i}\}_{i=0}^{N=3} &=& \{1,3,8,6\}\label{eq:twoOneDimSeq_2}\\
\{X^2_{t_i}\}_{i=0}^{N=3} &=& \{1,4,2,5\}\label{eq:twoOneDimSeq_3}
\end{eqnarray}
%where the variable $\{t_i\}$ corresponds to the ordering of the terms in \eqref{eq:twoOneDimSeq_1}-\eqref{eq:twoOneDimSeq_2} and is usually interpreted as {\it time}. 
We are interested in transforming this discrete series into a continuous path. Among various ways to find this transformation we focus on two main approaches: 
%
\begin{enumerate}[label=(\alph*)]
\item \textbf{Piece-wise linear interpolation.}

This interpolation method is given by a set of linear segments (local linear approximation) connecting a set of data points. The resulting continuous path is a piece-wise combination of linear functions. Formally, for each pair of points $X_i$ and $X_{i+1}$ on the interval $t\in [t_i, t_{i+1}]$, the path is defined as:
%
\begin{equation*}
    \hat{X_t} = X_{t_i} + \frac{t-t_i}{t_{i+1} - t_i}\left(X_{t_{i+1}} - X_{t_i}\right).
\end{equation*}
%
By concatenating linearly interpolated paths, one arrives at the continuous path $\hat{X_t}$ defined for any $t\in[t_0, t_N]$. %The application of the piece-wise linear interpolation to streams in \eqref{eq:twoOneDimSeq_2} and \eqref{eq:twoOneDimSeq_3} is presented in Fig.~\ref{fig:piece_wise_interpolation}.
%
%\begin{figure}
%    \centering
%    \includegraphics[width=0.75\linewidth]{artwork/fig_21.pdf}
%    \caption{Examples of a piece-wise linear interpolation applied to one dimensional streams $\{X^1\}$, $\{X^2\}$ and to a 2-dimensional stream $\{(X^1, X^2)\}$ from \eqref{eq:twoOneDimSeq_2} and \eqref{eq:twoOneDimSeq_3}.}
%    \label{fig:piece_wise_interpolation}
%\end{figure}
%\noindent
%

\item \textbf{Rectilinear interpolation} (i.e. {\it axis path}).

Another way to connect $X_{t_i}$ and $X_{t_{i+1}}$ data points is by keeping the value of a path along each axis constant until updated at a new time point. Formally, for $t\in[t_i, t_{t+1})$ with $i=0,1, ..., N-1$:
\begin{equation*}
    \hat{X_t} = X_{t_i},
\end{equation*}
so that at each time point $t_{i+1}$, for $i = 0, . . . ,N-1$, the path jumps to value $X_{t_{i+1}}$.

%\begin{figure}
%    \centering
%    \includegraphics[width=\linewidth]{artwork/fig_22.pdf}
%    \caption{Examples of a rectilinear interpolation applied to one dimensional streams $\{X^1\}$, $\{X^2\}$ and to a 2-dimensional stream $\{(X^1, X^2)\}$ from \eqref{eq:twoOneDimSeq_2} and \eqref{eq:twoOneDimSeq_3}.}
%    \label{fig:rectilinear_interpolation}
%\end{figure}
%\noindent
%
\end{enumerate}

The piece-wise linear and rectilinear interpolation schemes using data streams in \eqref{eq:twoOneDimSeq_2} and \eqref{eq:twoOneDimSeq_3} are presented in Fig.~\ref{fig:piecewise_interp} and Fig.~\ref{fig:rectilinear_interp} respectively. Note that the auxiliary points denoted by empty red circles were added to construct the rectilinear paths. 

\begin{figure}[ht]
     \centering
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{artwork/fig_2_piecewise_interp.pdf}
         \caption{}
         \label{fig:piecewise_interp}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{artwork/fig_2_rectilinear_interp.pdf}
         \caption{}
         \label{fig:rectilinear_interp}
     \end{subfigure}
     \caption{Examples of a piece-wise linear (a) and rectilinear (b) interpolation schemes applied to one dimensional streams $\{X^1\}$, $\{X^2\}$ from \eqref{eq:twoOneDimSeq_2} and \eqref{eq:twoOneDimSeq_3}.}
     \label{fig:path_interps}
\end{figure}

%\begin{figure}[h]
%    \centering
%    \includegraphics[width=0.6\linewidth]{artwork/fig_2_interpolations_v.pdf}
%    \caption{Examples of a piece-wise linear (left column) and rectilinear (right column) interpolation schemes applied to one dimensional streams $\{X^1\}$, $\{X^2\}$ from \eqref{eq:twoOneDimSeq_2} and \eqref{eq:twoOneDimSeq_3}.}
%    \label{fig:path_interps}
%\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Auxiliary path transformations}

Whilst data points can be transformed directly into paths as in  Section~\ref{subsubsec:paths_from_discrete_data}, in certain cases, auxiliary data transformations may improve statistical learning with signatures for downstream tasks. More specifically, the auxiliary transformation $\phi$ can be represented as:

\begin{equation*}\label{eq:path_augmentation}
    \phi: X\in\mathbb{R}^d \rightarrow \Tilde{X}\in\mathbb{R}^p, \;\;\;d,p\in\mathbb{N}
\end{equation*}
where the original sequence $X\in\mathbb{R}^d$ is transformed into a new sequence $\Tilde{X}\in\mathbb{R}^p$. Various path transformations and augmentations may lead to a more effective representation of sequential data, remove redundant information in signature terms, lower the dimension $d$ of the data streams and, as a result, reduce the number of higher order signature terms and thus computer memory consumption. 


\subsubsection*{Cumulative sum}
    
%For various numerical applications, the original data may be mapped into different forms to exhibit its structure. 
A cumulative sum, also known as a running total, is a sequence of partial sums of a given sequence of numbers. In other words, it is a sequence of sums of the elements of the original sequence, where each sum is calculated by adding the previous sum to the current element of the sequence.
%One of the examples of such a mapping is the \emph{cumulative sum}, or sequence of partial sums. 
More precisely the cumulative sum is defined by
%
\begin{eqnarray}\label{eq:cumSumDef}
CS(\{X_{t_i}\}_{i=0}^{N}) = \{X_{t_0},X_{t_0}+X_{t_1},\dots,S_k,\dots,S_N\}\;;\;\;\;\;S_k = \sum_{i=0}^{k}X_{t_i}.
\end{eqnarray}
%
Using again the previous example \eqref{eq:twoOneDimSeq_2} and \eqref{eq:twoOneDimSeq_3}, the new data streams become
%
\begin{eqnarray}\label{eq:cumsum_x1}
\{\tilde{X^1}\} = CS(X^1) &=& \{1, 4, 12, 18\}\\
\{\tilde{X^2}\} = CS(X^2) &=& \{1, 5, 7, 12\}.\nonumber
\end{eqnarray}
%
\subsubsection*{Base-point augmentation}

As discussed in Section \ref{sec:First}, the signature transformation is translation invariant, meaning that paths at different locations in $\mathbb{R}^d$ will produce the same signature. In some cases, it may be useful to remove this translation invariance. For example, to capture the absolute values of data streams rather than their increments. To do this, an anchor data point, typically the origin (0), can be added at the beginning of the data stream. This removes the translation invariance of the signature transformation. Using examples \eqref{eq:twoOneDimSeq_2} and \eqref{eq:twoOneDimSeq_3}, the augmented data streams with $N+1$ data points become
%
\begin{eqnarray}\label{eq:bp_augmentation}
BP(\{X^1_{t_i}\}_{i=0}^{N=3}) = \{0, \{X^1_{t_i}\}_{i=0}^{N=3}\} &=& \{\textbf{0},1,3,8,6\}\\
BP(\{X^2_{t_i}\}_{i=0}^{N=3}) = \{0, \{X^2_{t_i}\}_{i=0}^{N=3}\} &=& \{\textbf{0},1,4,2,5\}.
\end{eqnarray}

\subsubsection*{Time augmentation}

This type of sequential data transformation is defined by adding a univariate component with monotonically increasing or decreasing values that can be interpreted as \textit{auxiliary time}. For example, consider a new (unevenly sampled) stream $\{t\}$
\begin{equation}
    \{t_i\}_{i=0}^{N=3} = \{0,1,3,6\},
\end{equation}
and augmenting $\{X^1\}_{i=0}^{N=3}$, $\{X^2\}_{i=0}^{N=3}$ and $\{(X^1, X^2)\}_{i=0}^{N=3}$ from \eqref{eq:twoOneDimSeq_2} and \eqref{eq:twoOneDimSeq_3} leads to:
\begin{eqnarray}\label{eq:ta_augmentation}
    TA(\{X^1_{t_i}\}_{i=0}^{N=3}) &=& \{(t_i, X^1_{t_i})\}_{i=0}^{N=3} = \{(0,1), (1,3), (3,8), (6,6)\}\\
    TA(\{X^2_{t_i}\}_{i=0}^{N=3}) &=& \{(t_i, X^2_{t_i})\}_{i=0}^{N=3} = \{(0,1), (1,4), (3,2), (6,5)\}\nonumber\\
    TA(\{(X^1_{t_i}, X^2_{t_i}\}_{i=0}^{N=3}) &=& \{(t_i, X^1_{t_i}, X^2_{t_i})\}_{i=0}^{N=3} = \{(0,1,1), (1,3,4), (3,8,2), (6,6,5)\}\nonumber
\end{eqnarray}
The signature of a stream integrated against a monotonic auxiliary stream (`time') can capture the stream-specific effects and can be related to common statistics (e.g., mean). Intuitively, the integral of a stream against auxiliary time component will describe the area under the path, which in some applications may capture important properties of the data process via the path and serve as a salient feature for downstream analytical tasks.

In some cases, knowing the difference between the timestamps may be informative, in particular for unevenly distributed data. To illustrate this scenario, consider streams $\{X^1\}$ and $\{X^2\}$ and their respective timestamps $\{t_i\}$ as shown in Table~\ref{tab:table1_time_diff_a}:

\begin{table}[h]
\begin{subtable}[t]{0.48\textwidth}
    \centering
    \begin{tabular}{c|c|c}
        $t_i$       & $X^2$ & $X^2$ \\\hline\hline
        01-January  &  1    &   1   \\
        02-January  &  3    &   4   \\
        04-January  &  8    &   2   \\
        07-January  &  6    &   5   \\
        08-January  &  9    &   3   \\\hline
    \end{tabular}
\caption{}
\label{tab:table1_time_diff_a}
\end{subtable}
%\hspace{\fill}
\begin{subtable}[t]{0.48\textwidth}
    \centering
    \begin{tabular}{c|c|c|c|c}
        $t_i$       &   $\hat{t}_i$ & $\Delta t_i$ & $X^2$ & $X^2$ \\\hline\hline
        01-January  &     0         &      -       &   1    &   1   \\
        02-January  &     1         &      1       &   3    &   4   \\
        04-January  &     3         &      2       &   8    &   2   \\
        07-January  &     6         &      3       &   6    &   5   \\
        08-January  &     7         &      1       &   9    &   3   \\\hline
    \end{tabular}
\caption{}
\label{tab:table1_time_diff_b}
\end{subtable}
\caption{Example}
\label{tab:table1}
\end{table}
In addition to the original timestamp stream $\{t_i\}$, we can introduce two auxiliary time-related streams:
\begin{eqnarray}
    \hat{t}_i &=& \{t_i - t_0\}_{i=0}^{N=4}  = \{0, 1, 3, 6, 7\}\\
    \Delta t_i &=&  \{t_{i} - t_{i-1}\}_{i=1}^{N=4} = \{1, 2, 3, 1\}\nonumber
\end{eqnarray}
Putting all streams together and aligning them in time, we get a 5-dimensional stream as shown in Table~\ref{tab:table1_time_diff_b}. Intuitively, $\{\hat{t}_i\}$ corresponds to time since the beginning and $\{\Delta t_i\}$ to time differences between two consecutive timestamps. Note that, since there is no time difference for the first data point, some heuristics can be used to fill in the missing value, such as arbitrarily setting it to zero.


\subsubsection*{Lead-lag transformation}\label{seq:lead_lag_section}
%\input{lead_lag}

A lead-lag transformation is a mathematical operation that shifts the phase of a time-series by a specified amount. In a lead-lag transformation, a time-series can be either ``led'' or ``lagged'' by a certain number of time steps. Leading a signal means that it is shifted forward in time, while lagging a signal means that it is shifted backward in time. Lead-lag transformations can be used to analyse the relationships between different signals. For example, the lead-lag transformation can map a one-dimensional path into a two-dimensional path. Certain statistics, such as the quadratic variation of a stochastic process can be represented in terms of the signature of the lead-lag transformed process (see Section~\ref{subsec:further_relationship}).

Let $X$ \eqref{eq:data_stream} be a $d$-dimensional data stream with $N$ data points. Following the definition \cite{gyurko2014extracting}, its Lead and Lag transformed streams $\{X^{Lead}_j\}_{j=0}^{2N}$ and $\{X^{Lag}_j\}_{j=0}^{2N}$ with $2N+1$ data points are defined as:

\begin{equation}\label{eq:lead_stream}
X^{Lead}_{t_j} \mapsto 
\begin{cases}
             X_{t_i} & \text{if} \;\; j=2i\\
             X_{t_i} & \text{if} \;\; j=2i-1\\
\end{cases}
\end{equation}
and
\begin{equation}\label{eq:lag_stream}
X^{Lag}_{t_j} \mapsto 
\begin{cases}
             X_{t_i} & \text{if} \;\; j=2i\\
             X_{t_i} & \text{if} \;\; j=2i+1.\\
\end{cases}
\end{equation}
It's clear from \eqref{eq:lead_stream} and \eqref{eq:lag_stream} that for each value of $i$ corresponds to three values of $j$:
\begin{eqnarray}
    j &=& 2i-1\nonumber\\
    j &=& 2i\nonumber\\
    j &=& 2i+1.\nonumber
\end{eqnarray}
For example, given a one-dimensional sequence with four values:
\begin{equation}
    \{X_{t_i}\}_{i=0}^{N=3} = \{X_{t_0}, X_{t_1}, X_{t_2}, X_{t_3}\},    
\end{equation}
by substituting $i\in[0,1,2,3]$ in \eqref{eq:lead_stream} the components of the lead stream of $\{X_{t_i}\}$ become
%
\begin{eqnarray}
 & & X^{Lead}_{t_0} = X_{t_0},\;\; X^{Lead}_{t_1} = X^{Lead}_{t_2} = X_{t_1} \\
    X^{Lead}_{t_3}  & = & X^{Lead}_{t_4} = X_{t_2},\;\; X^{Lead}_{t_5} = X^{Lead}_{t_6} = X_{t_3}, \nonumber
\end{eqnarray}
and correspondingly of the lag \eqref{eq:lag_stream} stream of $\{X_{t_i}\}$:
\begin{eqnarray}
    X^{Lag}_{t_0} & = & X^{Lag}_{t_1} = X_{t_0},\;\; X^{Lag}_{t_2} = X^{Lag}_{t_3} = X_{t_1} \\
    X^{Lag}_{t_4}  & = & X^{Lag}_{t_5} = X_{t_2},\;\; X^{Lag}_{t_6} = X^{Lag}_{t_7} = X_{t_3}, \nonumber 
\end{eqnarray}
or more compactly:
\begin{eqnarray}
    Lead: \{X_{t_i}\}_{i=0}^{3}\mapsto\{X^{Lead}_{t_j}\}_{j=0}^{6} & = & \{X_{t_0}, X_{t_1}, X_{t_1}, X_{t_2}, X_{t_2}, X_{t_3}, X_{t_3}\} \\
    Lag: \{X_{t_i}\}_{i=0}^{3}\mapsto\{X^{Lead}_{t_j}\}_{j=0}^{6} & = & \{X_{t_0}, X_{t_0}, X_{t_1}, X_{t_1}, X_{t_2}, X_{t_2}, X_{t_3}\}. \nonumber
\end{eqnarray}
One can immediately see that lead and lag transforms are derived from the original data stream by repeating and shifting its data points and deleting the first and last data points. They are repeated and time-shifted versions of each other.

Considering the sequence $X^1$ \eqref{eq:twoOneDimSeq_2} its Lead-Lag (LL) mapping is given by:
%
\begin{equation}\label{eq:leadLagAlgo_X1}
LL\;:\;X^1 = \left\{1, 3, 8, 6\right\} \mapsto 
\begin{cases}
             X^{1,Lead}&= \left\{1, 3, 3, 8, 8, 6, 6\right\}\\
             X^{1,Lag} &= \left\{1, 1, 3, 3, 8, 8, 6\right\}\\
\end{cases}
\end{equation}
%
and illustrated in Fig.~\ref{fig:lead_lag_of_x1}.
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{artwork/fig_2_lead_lag_x1.pdf}
    \caption{Lead and lag paths of $X^1$.}
    \label{fig:lead_lag_of_x1}
\end{figure}
%
The corresponding lead-lag transformation of $X^2$ \eqref{eq:twoOneDimSeq_3} is given by
%
\begin{equation}\label{eq:leadLagAlgo_X2}
LL\;:\;X^2 = \left\{1, 4, 2, 6\right\} \mapsto 
\begin{cases}
             X^{2,Lead}&= \left\{1, 4, 4, 2, 2, 6, 6\right\}\\
             X^{2,Lag} &= \left\{1, 1, 4, 4, 2, 2, 6\right\}
\end{cases}
\end{equation}
%
as presented in Fig.~\ref{fig:lead_lag_of_x2}.
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{artwork/fig_2_lead_lag_x2.pdf}
    \caption{Lead and lag paths of $X^2$.}
    \label{fig:lead_lag_of_x2}
\end{figure}


\subsubsection*{Multivariate time-series as a path in \texorpdfstring{$\mathbb{R}^d$}{Rd}}

The advantage of using the path representation of sequential data is in the fact that a $d$-dimensional process can be embedded as a path in $\mathbb{R}^d$. %If one is interested in the cross-correlation between different variables ($\{X^1_i\},\{X^2_i\},...\{X^d_i\}$) then one has to create a multi-dimensional path in $\mathbb{R}^d$. 
For example, two univariate streams $\{X^1\}\in\mathbb{R}$ \eqref{eq:twoOneDimSeq_2} and $\{X^2\}\in\mathbb{R}$ \eqref{eq:twoOneDimSeq_3} can be embedded into a path in $\mathbb{R}^2$ as:
\begin{eqnarray}
    \{X_{t_i}\}_{i=0}^{N=3} &=& \{\bigl(X^1_{t_i}, X^2_{t_i} \bigr)\}_{i=0}^{N=3}\\
    &=& \{(1, 1), (3, 4), (8, 2), (6, 5)\},\nonumber
\end{eqnarray}
%
and displayed in Fig.~\ref{fig:2_from_1_paths}. 
\begin{figure}[h]
    \centering
    \includegraphics[width=0.6\linewidth]{artwork/fig_2_x1x2.pdf}
    \caption{Example of embedding two paths in $\mathbb{R}$ into a single path in $\mathbb{R}^2$ using piece-wise linear (left) and rectilinear (right) interpolations respectively.}
    \label{fig:2_from_1_paths}
\end{figure}


This can be easily extended to $\mathbb{R}^3$ if we add another univariate stream of the same length:
\begin{equation}
    \{X^3_{t_i}\}_{i=0}^{N=3} = \{9,2,7,1\}\label{eq:twoOneDimSeq_4}\\
\end{equation}
resulting in
\begin{eqnarray}
    \{X_{t_i}\}_{i=0}^{N=3} &=& \{\bigl(X^1_{t_i}, X^2_{t_i}, X^3_{t_i} \bigr)\}_{i=0}^{N=3}\\
    &=& \{(1, 1, 9), (3, 4, 2), (8, 2, 7), (6, 5, 1)\}.\nonumber
\end{eqnarray}
The resulting paths in 3-dimensions using piece-wise linear (left) and rectilinear (right) interpolations are shown in Fig.~\ref{fig:x1x2x3}.

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{artwork/fig_2_x1x2x3_piecewise_and_rectilinear.pdf}
    \caption{Example of embedding three paths each in $\mathbb{R}$ into a single path in $\mathbb{R}^3$ using piece-wise linear (left) and rectilinear (right) interpolations respectively.}
    \label{fig:x1x2x3}
\end{figure}


Another example of a multidimensional embedding involves the lead-lag transform. Suppose we are interested in capturing the quadratic variation in one of the multivariate streams. As we will see in Section~\ref{subsec:further_relationship}, we can compute the quadratic variation using the lead-lag transformation. Since the lead-lag transformation increases the number of original $N$ points to $2N+1$ (cf. Section \ref{seq:lead_lag_section}), all other stream lengths should be adjusted accordingly. It is worth noticing that, due to re-parametrization invariance, the signatures of the lead and lag transformations of streams are equivalent:
\begin{equation}
    S\Bigl(\bigl\{\bigl(X^1, X^2\bigr)\bigr\}\Bigr) \equiv S\Bigl(\{\bigl(X^{1, Lead}, X^{2, Lead}\bigr)\}\Bigr) \equiv S\Bigl(\{\bigl(X^{1, Lag}, X^{2, Lag}\bigr)\}\Bigr).
\end{equation}
%One way of adjusting the length of all other streams is to compute their \textit{lead} or \textit{lag} (or both) transformations. For example, given two univariate streams $\{X^1\}$ and $\{X^2\}$, we are only interested in capturing the quadratic variation in $\{X^2\}$. The solution is to create a 3-dimensional stream:
%\begin{equation}
%    \{\bigl(X^1, X^2\bigr)\} \mapsto \{\bigl(X^{1,Lead}, X^{2,Lead}, X^{2,Lag}\bigr)\}
%\end{equation}
%and the signature terms of $\{\bigl(X^{2,Lead}, X^{2,Lag}\bigr)\}$ will yield the quadratic variation of $\{\bigl(X^{2}\bigr)\}$.


\subsubsection*{Further path transformations}

In this subsection, we showed several examples of different path augmentations, but there exist many others that serve various purposes. For example, invisibility-reset augmentation that adds information on the initial position of the path,
coordinate projections that allow to compute the signature of a subset of coordinates individually, data rescalling,
and random projections that project a high-dimensional path onto a lower-dimensional subspace using a random matrix. For further details, see \cite{morrill2020generalised}.


\begin{comment}
Here we include the time vector $t=\{0,1,2,3,4\}$ with $X=\{0,1,3,5,2\}$ and compute the lead-lag transform of $X$. The red dots represent the actual data points of the Cartesian ordered tuple:
%
\ilya{There is a typo here, the lead and lag are identical. Same with the graph?}
\begin{eqnarray}
\{(t^{lead},X^{lead},X^{lag})_i\}\;=\;\{(0,0,0),(1,1,1),(2,3,3),(3,5,5),(4,2,2)\}.
\end{eqnarray}
%
Applying the axis-path interpolation, we get the path presented in Fig.~\ref{fig:3D_lead_lag_pic}.
%
\begin{figure}[ht] 
\centering
    \includegraphics[width=0.75\linewidth]{artwork/3D_lead_lag} 
\caption{Example of a three dimensional lead-lag transform of the data $\{(t^{lead},X^{lead},X^{lag})_i\}$. The path is build by means of sequential increments along each Cartesian direction. This path allows to study the variance of $\{X\}$ as well as its time-dependent properties.}
\label{fig:3D_lead_lag_pic}
\end{figure}
\noindent

%we can construct paths in $\mathbb{R}^2$ and $\mathbb{R}^3$ spaces, presented in Fig.~\ref{fig:2D} and Fig.~\ref{fig:3D} respectively.


%consider the linear piece-wise embedding of \eqref{eq:twoOneDimSeq_1}-\eqref{eq:twoOneDimSeq_3} in a 2-dim path $X(t) = \{X^1_i,X^2_i\}$ and 3-dim $X(t) = \{t_i,X^1_i,X^2_i\}$ which are plotted in Fig.~\ref{fig:2D} and Fig.~\ref{fig:3D} respectively.
%
%\begin{figure}[ht] 
%\centering
%\captionsetup[subfigure]{justification=centering}
%  \begin{subfigure}[b]{0.45\linewidth}
%    \centering
%    \includegraphics[width=0.75\linewidth]{artwork/curve_2D} 
%    \caption{2-dim path from two 1-dim paths $\{X^1_i,X^2_i\}$.} 
%    \label{fig:2D} 
%    \vspace{4ex}
%  \end{subfigure}%% 
%  \begin{subfigure}[b]{0.5\linewidth}
%    \centering
%    \includegraphics[width=0.75\linewidth]{artwork/curve_3D} 
%    \caption{3-dim path from three 1-dim paths $\{t_i,X^1_i,X^2_i\}$.} 
%    \label{fig:3D} 
%    \vspace{4ex}
%  \end{subfigure} 
%\caption{Examples of embedding a collection of one-dimensional paths into a single multi-dimensional path.}
% $\{\mathbb{R}_1,\mathbb{R}_2,...,\mathbb{R}_d\}\mapsto \{\mathbb{R}^d\}$.}
%\label{fig:embedding2DAnd3D}
%\end{figure}
%\noindent
%and the resulting embedded path is presented in Fig.~\ref{fig:newLeadLag} with three additional points $\{(1,4),(4,2),(2,6)\}$.  
%
%\begin{figure}[ht] 
%\centering
%    \includegraphics[width=0.4\linewidth]{new_LeadLag} 
%    \caption{Lead-Lag transform of $\{X^2_i\}$.} 
%    \label{fig:newLeadLag} 
%\end{figure}
%\noindent
%
%We can define a {\it rectilinear} operator $\mathscr{R}$ which maps a discrete set of points into a continuous function on a rectangular grid:
%
%\begin{itemize}
%\item Rectilinear path (Fig.~\ref{fig:bRectilinear}): $\mathscr{R}(\{t_i, %X^2_i\})$ 
%\item Rectilinear cumulative sum path (Fig.~\ref{fig:bRectilinearCumSum}): $\mathscr{R}(\{t_i ,CS(X^2_i)\})$ 
%\item Lead-Lag path (Fig.~\ref{fig:newLeadLag}): $\mathscr{R}(\{X^{2,Lag}_i , %X^{2,Lead}_i\})$ 
%\end{itemize}
%
%This operator $\mathscr{R}$ increases the number of points in a sequence from $N$ to $2N-1$, resulting in additional coordinate points (indicated previously by empty red circles).
%: $\mathscr{R}: \{X^2_i\}_i=1^N\mapsto \{X^2_i\}_{i=1}^{2N-1}$
%We do not define here the operator $\mathscr{R}$ explicitly, but rather present the general idea. For real practical applications this operator is easily implemented with any programming software, being guided by the above examples.
%definition \eqref{eq:leadLagAlgo}.
%{\bf UNDERSTAND HOW TO DERIVE THIS OPERATOR $\mathscr{R}$ !!! Thanks Guy Flint.}
%
\end{comment}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
\begin{figure}[ht] 
\centering
\captionsetup[subfigure]{justification=centering}
  \begin{subfigure}[b]{0.45\linewidth}
    \centering
    \includegraphics[width=\linewidth]{curve_2} 
    \caption{Example of the change of the area enclosed by the curve and chord at different endpoints.} 
    \label{fig:exampleOfPositiveNEgativeArea} 
    \vspace{4ex}
  \end{subfigure}%% 
  \begin{subfigure}[b]{0.5\linewidth}
    \centering
    \includegraphics[width=\linewidth]{rose} 
    \caption{Example of relative signs of data streams $\{X^1, X^2\} = \{\pm t, \pm t^2\}$ and their resulting signed areas.} 
    \label{fig:rose} 
    \vspace{4ex}
  \end{subfigure} 
\caption{Right panel (b): example of relative signs of data streams $\{X^1, X^2\} = \{\pm t, \pm t^2\}$ and their resulting signed areas. Red and blue areas correspond to positive and negative correlations respectively. The $``+,+"$ combination corresponds to the first quadrant $\{t, t^2\}$, $``-,+"$ corresponds to the second quadrant $\{-t, t^2\}$, and so on. Black arrows represent the direction of movement along the path.}
\label{fig:aabbcc}
\end{figure}
\noindent
\end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%In order to gain more intuition about the geometric properties of different embeddings, such as in Fig.~\ref{fig:twoInterpolations}, we should explore their properties in more details. 
%The signed area of the embedded path  (Fig.~\ref{fig:twoInterpolations}) is proportional to the relative {\it correlation} between the data streams. For example, two negatively (resp. positively) correlated data streams will result in a negative (resp. positive) area of the combined path. 

%The following example demonstrates this idea. 
%\begin{example}
%Consider the two dimensional data stream $\{X^1_t, X^2_t\}$ with $X^1(t) = t$, $X^2(t) = t^2$, ($t \in [0,10]$). Then there are four possibilities for embedding the data into a single path: $X = \{\pm t, \pm t^2\}$ which are depicted in Fig.~\ref{fig:rose}. A relative minus sign between $X^1$ and $X^2$ means that one component decreases while the other one increases, and vice versa.
%
%\begin{figure}[htb]
%\centering
%\includegraphics[scale=.4]{rose}
%\centering
%\caption{Example of relative signs of data streams $\{X^1, X^2\} = \{\pm t, \pm t^2\}$ and their resulting signed areas. Red and blue areas correspond to positive and negative correlations respectively. The $``+,+"$ combination corresponds to the first quadrant $\{t, t^2\}$, $``-,+"$ corresponds to the second quadrant $\{-t, t^2\}$, and so on. Black arrows represent the direction of movement along the path.}
%\label{fig:rose}
%\end{figure}
%\noindent
%This example illustrates the indicative property which relates the signed area of the embedded path to the relative correlation of individual data streams. 
%\end{example}



%There are particular advantages and disadvantages of using different path parametrizations and the choice depends on the concrete application at hand. One of the widely used approaches is to compute the lead-lag transformation and use the axis path parametrization. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Signed area}
\label{sec:signed_area}
Before we continue, it is important to emphasise the significance of the direction in which we travel along a path and the sign of the area which it encloses. Intuitively, the signed area enclosed by a path is a measure of the 2-dimensional region enclosed by the path. It is calculated by taking the absolute value of the area and then assigning a positive or negative sign to it depending on the orientation of the path. A positively oriented path (or \textit{a curve}) is a simple closed path in the plane such that when following the path, the interior of the path is always on the left side. For a negatively oriented path, the interior is on the right side instead of the left side. In other words, the orientation of a path is determined by the direction in which the path appears to turn as it is traced. If the path turns clockwise, it is negatively oriented. If the path turns counterclockwise, it is positively oriented.

For example, if a path is traced in a clockwise direction, the signed area of the enclosed region would be negative (Fig.~\ref{fig:negative_area}). If the path is traced in a counterclockwise direction, the signed area would be positive (Fig.~\ref{fig:positive_area}). A combination of positively and negatively oriented paths and their respective areas is shown in Fig.~\ref{fig:positive_and_neagative_area}. The sign of an area is also related to the sign of the winding number of a path~\cite{BoedihardjoNi14}. 

\begin{figure}[h]
     \centering
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{artwork/fig_2_signed_area_negative.pdf}
         \caption{Negative area $A_{-}$.}
         \label{fig:negative_area}
     \end{subfigure}
     %\hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{artwork/fig_2_signed_area_positive.pdf}
         \caption{Positive area $A_{+}$.}
         \label{fig:positive_area}
     \end{subfigure}
     %\hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{artwork/fig_2_signed_area_positive_negative.pdf}
         \caption{Positive and negative areas.}
         \label{fig:positive_and_neagative_area}
     \end{subfigure}    
     \caption{Examples of signed areas defined by the orientation of a path enclosing them.}
     \label{fig:signed_area_examples}
\end{figure}

\subsubsection*{The relative movement as a signed area}

%Consider two processes $\{X_t\}$ and $\{Y_t\}$ which follow each other's paths. Certain properties of the lead-lag process are easily captured by the signature of the path comprised of these processes $\{X_t,Y_t\}$~\cite{flint2015discretely}. This is demonstrated in the following example. 
Consider a path in $\mathbb{R}^2$ given by $X = \{X^1,X^2\}$. If an increase (resp. decrease) of the component $X^1$ is followed by an increase (resp. decrease) in the component $X^2$, then the area $A$ given by \eqref{eq:LevyArea} is positive (Fig.~\ref{fig:positive_area2}). If the relative moves of the components $X^1$ and $X^2$ are in the opposite direction, then the area $A$ is negative (Fig.~\ref{fig:negative_area2}). 

\begin{figure}[H]
\centering
\includegraphics[width=0.8\linewidth]{artwork/slow_fast.pdf}
\caption{Example of a positive L{\'e}vy area that corresponds to two paths, $\{X^1\}$ and $\{X^2\}$, with relative movement in the same directions.}
\label{fig:positive_area2}
\end{figure}
\noindent

\begin{figure}[H]
\centering
\includegraphics[width=0.8\linewidth]{artwork/neg_area.pdf}
\caption{Example of a negative L{\'e}vy area that corresponds to two paths, $\{X^1\}$ and $\{X^2\}$, with relative movement in the opposite directions.}
\label{fig:negative_area2}
\end{figure}
\noindent


%\subsubsection*{Change of signed area }

%The notation here is: $A_{[X^1_i,X^1_f]}$ area between two points, where $(i,f)$ are {\it initial} and {\it final} endpoints along the direction of $X^1$. Moving at first from left to right (increasing the parameter $t$), $X^1$ and $X^2$ both increase, resulting in the increasing area $A_{ij}$: $A_{[0,3]} = 35$, $A_{[0,5]} = 179$. At some point ($X^1 = 6.72$) the area attains its maximum value $A_{[0,6.72]} = 296$ and after this point the area decreases as we increase the value of $X^1$. The total area between the two endpoints is $A_{[0,9]} = -393$.  

%\begin{figure}[H]
%\centering
%\includegraphics[width=0.7\linewidth]{artwork/curve_2.png}
%\caption{Example of the change of the area enclosed by the curve and the chord at different endpoints.}
%\label{fig:exampleOfPositiveNEgativeArea}
%\end{figure}
%\noindent



%with a small time lag:
%
%\begin{eqnarray}
%X_{t+k} \propto Y_{t},\;\; k>0,
%\end{eqnarray}
%
%giving the name {\it Lead-Lag process}. Certain properties of the lead-lag process are easily captured by the signature of the path comprised of these processes $\{X_t,Y_t\}$~\cite{flint2015discretely}. This is demonstrated in the following example. Consider a path in $\mathbb{R}^2$ given by $X = \{X^1,X^2\}$. If an increase (resp. decrease) of the component $X^1$ is followed by an increase (resp. decrease) in the component $X^2$, then the area $A$ given by
%\eqref{eq:LevyArea} is positive. If the relative moves of the components $X^1$ and $X^2$ are in the opposite direction, then the area $A$ is negative. In Fig.\ref{fig:exampleOfPositiveNEgativeArea} we can see how the area changes as we increase the endpoint.
%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Computation and geometry of the signature}
\label{sec:signature_of_a_path}
% statistical learning and inference for sequential data using the signature as a feature set that concisely characterises sequential data embedded as a path in $d$-dimensions. %statistical learning and inference for sequential data using the signature as a feature set that concisely characterises sequential data embedded as a path in $d$-dimensions. In this section, we illustrate how to compute the signature of multidimensional data stream 
%the signature as faithful representation or a feature set that concisely characterised a path.

%For a given path, one can compute its signature according to the rules and definition in the Sec.~\ref{sec:First}. We will present computations of signatures for various embeddings as presented in Figs.~\ref{fig:twoInterpolations}-\ref{fig:embedding2DAnd3D} and discuss their properties.

In Section~\ref{sec:First}, we outlined the mathematical foundations of the signature of a path and defined the signature terms as multiple iterated integrals. In this subsection, we give another example of a computation and the geometrical meaning of the signature. Consider the two univariate streams $\{(X^1, X^2)\}$:
\begin{eqnarray}\label{eq:sig_x1x2}
    \{(X^1)\} &=& \{0, 1, 2, 3, 4, 5\}\\
    \{(X^2)\} &=& \{8, 4, 5, 1, 10, 3\}\nonumber
\end{eqnarray}
embedded into a piece-wise linear path in $\mathbb{R}^2$ (Fig.~\ref{fig:sig_raw}). Using the definition of the signature \eqref{eq:definSig}, we compute its first terms truncated at level $L=2$:
\begin{table}[h]
    \centering
    \begin{tabular}{lrrrrrrr}
        $S(X)$ = & (1, & $S^{(1)}$, & $S^{(2)}$, & $S^{(1,1)}$, & $S^{(1,2)}$, & $S^{(2,1)}$, & $S^{(2,2)}$)  \\
               & $(1$, & $5$,       & $-5$,      & $12.5$,      & $-10.5$,     & $-14.5$,     & $12.5$)  
    \end{tabular}
\end{table}

\begin{figure}[h]
     \centering
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{artwork/fig_2_signature_raw.pdf}
         \caption{A piece-wise linear path $\{(X^1, X^2)\} \in\mathbb{R}^2$ constructed from $\{(X^1)\}$ and $\{(X^2)\}$ using data point \eqref{eq:sig_x1x2}.}
         \label{fig:sig_raw}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{artwork/fig_2_signature_s1s2.pdf}
         \caption{Geometric meaning of the first two terms $S^{(1)}$ and $S^{(2)}$ of the signature of the path $\{(X^1, X^2)\}$.}
         \label{fig:sig_s1s2}
     \end{subfigure}
     \caption{Examples of two univariate data streams \eqref{eq:sig_x1x2} embedded in $\mathbb{R}^2$ (a) and the geometric meaning of their signature terms $S^{(1)}$ and $S^{(2)}$ (b).}
     \label{fig:signature_terms_raw_s1s2}
\end{figure}
One can easily confirm (cf.~\eqref{singInteg}) that the first order signature terms correspond to the total increments along each data stream:
\begin{eqnarray}
    S^{(1)} &=& \int dX^1_t = X^1_{t_5} - X^1_{t_0} = 5-0 = 5\\
    S^{(2)} &=& \int dX^2_t = X^2_{t_5} - X^2_{t_0} = 3-5 = -5\nonumber
\end{eqnarray}
that are depicted in Fig.~\ref{fig:sig_s1s2}. The second order signature terms are computed using double iterated integrals (cf. \eqref{doublInteg}):
\begin{eqnarray}\label{eq:four_sig_numerical}
    S^{(1,1)} &=& \int S^{(1)}dX^1_t = \int \int dX^1_t dX^1_t = \frac{1}{2!}\left(\int dX^1_t\right)^2 = \frac{1}{2!}\left(S^{(1)}\right)^2 = 12.5\\
    S^{(1,2)} &=& \int S^{(1)}dX^2_t = \int \int dX^1_t dX^2_t = -10.5\nonumber\\
    S^{(2,1)} &=& \int S^{(2)}dX^1_t = \int \int dX^2_t dX^1_t = -14.5\nonumber\\
    S^{(2,2)} &=& \int S^{(2)}dX^2_t = \int \int dX^2_t dX^2_t = \frac{1}{2!}\left(\int dX^2_t\right)^2 = \frac{1}{2!}\left(S^{(2)}\right)^2 = 12.5\nonumber
\end{eqnarray}
The second order signature terms $S^{(1,2)}$ and $S^{(2,1)}$ and their geometric interpretation as areas are presented in \fig{fig:signature_terms_s12_s21}.
\begin{figure}[h]
     \centering
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{artwork/fig_2_signature_s12.pdf}
         \caption{Area represented by the term $S^{(1,2)}$.}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{artwork/fig_2_signature_s21.pdf}
         \caption{Area represented by the term $S^{(2,1)}$.}
     \end{subfigure}
     \caption{The geometric meaning of the terms $S^{(1,2)}$ and $S^{(2,1)}$ of $\{(X^1, X^2)\}$ defined in \eqref{eq:sig_x1x2}. The left panel (a) represents the area enclosed by the path and two perpendicular dashed lines passing through the endpoints of the path, while the right panel (b) shows another possibility for the area to be enclosed by the path and two perpendicular dashed lines passing through the endpoints.}
     \label{fig:signature_terms_s12_s21}
\end{figure}
Switching the order of integration over the path in the terms $S^{(1,2)}$ and $S^{(2,1)}$ gives rise to two areas which complete each other and add up to the total area of a rectangle with side lengths $X^1$ and $X^2$, which also corresponds to the shuffle product relation:
%
\begin{eqnarray}
S^{(1)}\cdot S^{(2)}  &=& S^{(1,2)} + S^{(2,1)}\nonumber\\
(-5)\cdot 5 &=& -10.5 + (-14.5).
\end{eqnarray}
%
The geometric interpretation of the higher order terms is less intuitive and we omit this discussion. It is worth noticing, that the areas that correspond to the second order signature terms ($S^{(1,2)}$ and $S^{(2,1)}$) have positive and negative signs depending on their position relative to the horizontal straight line. If we split the areas in Fig.~\ref{fig:signature_terms_s12_s21} into individual areas that lie above and underneath the horizontal dashed lines, we get the following partitions as shown in Fig.~\ref{fig:signature_terms_s12_s21_split}:
\begin{figure}[h]
     \centering
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{artwork/fig_2_signature_s12_3parts.pdf}
         \caption{The total area $S^{(1,2)} = A_1 +  A_2 + A_3$.}
         \label{fig:sig_s12}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{artwork/fig_2_signature_s21_3parts.pdf}
         \caption{The total area $S^{(2,1)} = \tilde{A}_1 + \tilde{A}_2 + \tilde{A}_3$.}
     \end{subfigure}
     \caption{A schematic partitioning of the areas $S^{(1,2)}$ (a) and $S^{(2,1)}$ (b) enclosed by the path and their corresponding dashed lines into a sum of individual contributions. Circles denote the point of intersection of the path and the corresponding dashed lines.}
     \label{fig:signature_terms_s12_s21_split}
\end{figure}

The intersection points, denoted by red circles in Fig.~\ref{fig:signature_terms_s12_s21_split} can be easily computed:
\begin{eqnarray}
    A &=& (5/2, 3), \;\;\;B = (29/9, 3)\nonumber\\
    \tilde{A} &=& (34/9, 8), \;\;\;\tilde{B} = (30/7, 8).\nonumber
\end{eqnarray}
Subsequently, one can directly compute the individual areas
\begin{eqnarray}
    A_1 &=& -5, \;\;\; A_2 = 13/18, \;\;\; A_3 = -56/9\nonumber\\
    \tilde{A}_1 &=& -119/9, \;\;\; \tilde{A}_2 = 32/63, \;\;\; \tilde{A}_3 = -25/14\nonumber
\end{eqnarray}
and demonstrate that the results
\begin{eqnarray}
    S^{(1,2)} &=& A_1 + A_2 + A_3 = -10.5\nonumber\\
    S^{(2,1)} &=& \tilde{A}_1 + \tilde{A}_2 + \tilde{A}_3 = -14.5\nonumber
\end{eqnarray}
correspond to the direct computation of the signature terms as shown in \eqref{eq:four_sig_numerical}. Note that the sign of an area is determined by the direction of the path that encloses the area, as demonstrated in Fig.~\ref{fig:signed_area_examples}.


The L{\'e}vy area \eqref{eq:LevyArea} of the path $\{(X^1, X^2)\}$ \eqref{eq:sig_x1x2} is shown in Fig~\ref{fig:signature_levy_area} and is given by
\begin{eqnarray}\label{eq:signature_levy_x1x2}
    A_{L\acute{e}vy}\;=\;\frac{1}{2}\left(S^{(1,2)}-S^{(2,1)}\right) = 2.
\end{eqnarray}

\begin{figure}
    \centering
    \includegraphics[width=0.75\textwidth]{artwork/fig_2_signature_levy_area.pdf}
    \caption{Example of the signed L{\'e}vy area enclosed by a piece-wise linear path and the
chord that connects two endpoints. The light blue area is negative and pink area is positive according to the direction of travel along the path (from left to right).}
    \label{fig:signature_levy_area}
\end{figure}
Using the intersection point $(3.4, 4.6)$ between the chord and the linear segment between $t_3$ and $t_4$, one can easily compute the areas $A_{+}=6.8$ and $A_{-}=-4.8$ and confirm that $A_{L\acute{e}vy} = A_{+}+A_{-}$ is equivalent to \eqref{eq:signature_levy_x1x2}.

\subsubsection{The log-signature of a path}

The shuffle product identity \eqref{thm:shuffle} implies that any polynomial function on signatures can be written as a linear combination of signature elements.
These relations however imply that the signature contains `repeated information', e.g. $S(X)^{i,i}_{a,b}$ can always be determined from the level 1 signature since $S(X)^{i,i}_{a,b}=\frac12 (S(X)^i_{a,b})^2$; for some tasks (e.g. linear regression) this repetition can be useful, as it increases the number of potentially useful features, but in some cases one may wish to remove it.
The log-signature (also known as a logarithmic signature), as defined in Section \ref{subsubsec:logSig}, is a condensed form of the signature that removes this repeated information: it contains the same information as the signature but with fewer terms. 

For example, consider a two-dimensional data stream $\{X\}\in\mathbb{R}^2$ in the vector space of formal series in two non-commuting indeterminates $\{e_1, e_2\}$ \eqref{def:formal_power_series}. Recalling the definition of the log-signature as a series expansion \eqref{thm:log_sig_series}, the log-signature truncated at level $L=4$ can be written as
\begin{eqnarray}
    \log S(X) &=& \lambda_{1}e_1 + \lambda_{2}e_2 + \lambda_{12}[e_1, e_2] + \lambda_{112}[e_1,[e_1,e_2]] + \lambda_{212}[e_2,[e_1,e_2]] \\
    &+&\lambda_{1112}[e_1,[e_1,[e_1,e_2]]] + \lambda_{2112}[e_2,[e_1,[e_1,e_2]]] + \lambda_{2212}[e_2,[e_2,[e_1,e_2]]], \nonumber
%    \\
%    &+& \lambda_{11112}[e_1,[e_1,[e_1,[e_1,e_2]]]] + \lambda_{21112} [e_2,[e_1,[e_1,[e_1,e_2]]]] + \lambda_{22112} [e_2,[e_2,[e_1,[e_1,e_2]]]]\nonumber\\ &+& \lambda_{22212} [e_2,[e_2,[e_2,[e_1,e_2]]]] + \lambda_{12112}[[e_1,e_2],[e_1,[e_1,e_2]]] + \lambda_{12212} [[e_1,e_2],[e_2,[e_1,e_2]]]\nonumber
\end{eqnarray}
where $\lambda_{i_1,...i_k}$ are coefficients and $[x,y] = x\otimes y - y \otimes x$ is the Lie bracket as defined in \eqref{eq:lie_brackets}.
In contrast to $S(X)$, the log-signature $\log S(X)$ has no \textit{a priori} relations on its elements, i.e. all combinations of numbers $\lambda_1,\ldots, \lambda_{2212}$ may appear.
Since $S(X)$ and $\log S(X)$ determine each other, this shows that $\log S(X)$ is a compressed version of $S(X)$.

Recalling the direct computation \eqref{eq:direct_computation_logsig}, one can readily verify the correspondence between the signature and log-signature terms. For example, up to the level $L=3$, the correspondence between the coefficients of the signature and log-signature is
\begin{eqnarray}\label{eq:sig_logsig_correspondence_l_3}
    \lambda_1 &=& S^{(1)}, \;\;\;\lambda_2 = S^{(2)}, \;\;\;\lambda_{12} = \frac{1}{2!}\left(S^{(1,2)} - S^{(2,1)}\right)\\
    \lambda_{112} &=& \frac{1}{3!}\left(S^{(1,1,2)} + S^{(2,1,1)} - 2 S^{(1,2,1)}\right),\;\;\lambda_{212} = -\frac{1}{3!}\left(S^{(1,2,2)} + S^{(2,2,1)} - 2 S^{(2,1,2)}\right),\nonumber
\end{eqnarray}
however, it is straightforward to show the correspondence for any truncation level $L$. 


Let us illustrate the geometric intuition for the low-order log-signature terms. Using the relationships in \eqref{eq:sig_logsig_correspondence_l_3}, the log-signature coefficients up to level $L=3$ of a two-dimensional path $X = \{(X^1, X^2)\}$ from \eqref{eq:sig_x1x2} are:
\begin{table}[!h]
    \centering
    \begin{tabular}{lrrrrrrr}
        $\log S(X)$ = & ($\lambda_{1}$, & $\lambda_{2}$, & $\lambda_{12}$, & $\lambda_{112}$, & $\lambda_{212}$ ) \\
                  & ($5$,       & $-5$,      & $2$,      & $-12$,     & $-35/6$)  
    \end{tabular}
    \label{tab:log_sig_x1_x2}
\end{table}

One can immediately see that $\lambda_1$ and $\lambda_2$ are the total increments along each of the axes and $\lambda_{12}$ corresponds to the L{\'e}vy area \eqref{eq:LevyArea} as depicted in Fig.~\ref{fig:signature_levy_area}. The higher order log-signature terms $L\ge3$ correspond to ``areas of areas'' \cite{reizenstein2019iterated} and can be represented as iterated Lie brackets of non-commuting indeterminates.
The log-signature, containing the same information as the signature, can likewise be used as a feature set in statistical and machine learning applications, at times with more efficiency, see e.g. \cite{2019arXiv190808286L,Liao22,Reizenstein20}.

\subsubsection{Numerical computation of the signature}
%In the previous sections, we have introduced a theoretical background of the signature transformation as an infinite series of iterated integrals of a path, constructed by interpolating data points. We demonstrated some applications of the signature as a feature map of multidimensional data streams. However, nothing has been mentioned about numerical recipes and how to compute the iterated integrals.
In order to streamline the development and application of the signature method, several numerical packages with Python interfaces have been developed for the comutation of the signature. The `ESig' package is implemented in C++ with an intuitive Python interface \cite{esiglib}. This packages computes the signature and log-signature coefficients, provides additional auxiliary tools and can be run on CPU and, if available, on GPUs to accelerate computations. Another package with Python interface `iisignature' can be installed from the `pypi.org' repository \cite{iisignature} and its implementation details are described in \cite{reizenstein2017calculation, reizenstein2018iisignature}. More recently, the `signatory' Python packages, that is available in `pypi.org' repository \cite{signatory}, has been developed to enable the integration of the signature transformation layer in deep learning applications \cite{kidger2020signatory}. More information about the usage of these numerical packages can be found in their respective documentations.





\begin{comment}
Consider the six possibilities in Fig.~\ref{fig:signedArePossibilities}
%
\begin{figure}[H]
\centering
	\subcaptionbox{}%
	  [.3\linewidth]{\includegraphics[height=3.5cm]{artwork/pos_1}}
	\subcaptionbox{}%
	  [.3\linewidth]{\includegraphics[height=3.5cm]{artwork/pos_2}}
	\subcaptionbox{}%
	  [.3\linewidth]{\includegraphics[height=3.5cm]{artwork/pos_3}}
	\subcaptionbox{}%
	  [.3\linewidth]{\includegraphics[height=3.5cm]{artwork/neg_1}}
	\subcaptionbox{}%
	  [.3\linewidth]{\includegraphics[height=3.5cm]{artwork/neg_2}}
	\subcaptionbox{}%
	  [.3\linewidth]{\includegraphics[height=3.5cm]{artwork/neg_3}}    
\caption{Various possibilities of signed area. The first row (a)-(c) corresponds to counter clock-wise movement along the path, and the bottom row (d)-(f) to clock-wise movement.}
\label{fig:signedArePossibilities}
\end{figure}
\noindent
%
where we clearly see how direction of movement along the axis paths corresponds to the sign of the enclosed area. This is intimately related to the sign of the winding number of the path~\cite{BoedihardjoNi14}. 


In order to gain more intuition about the geometric properties of different embeddings, such as in Fig.~\ref{fig:twoInterpolations}, we should explore their properties in more details. The signed area of the embedded path is proportional to the relative {\it correlation} between the data streams. For example, two negatively (resp. positively) correlated data streams will result in a negative (resp. positive) area of the combined path. The following example demonstrates this idea. 

\begin{example}
Consider the two dimensional data stream $\{X^1_t, X^2_t\}$ with $X^1(t) = t$, $X^2(t) = t^2$, ($t \in [0,10]$). Then there are four possibilities for embedding the data into a single path: $X = \{\pm t, \pm t^2\}$ which are depicted in Fig.~\ref{fig:rose}. A relative minus sign between $X^1$ and $X^2$ means that one component decreases while the other one increases, and vice versa.
%
\begin{figure}[htb]
\centering
\includegraphics[scale=.4]{rose}
\centering
\caption{Example of relative signs of data streams $\{X^1, X^2\} = \{\pm t, \pm t^2\}$ and their resulting signed areas. Red and blue areas correspond to positive and negative correlations respectively. The $``+,+"$ combination corresponds to the first quadrant $\{t, t^2\}$, $``-,+"$ corresponds to the second quadrant $\{-t, t^2\}$, and so on. Black arrows represent the direction of movement along the path.}
\label{fig:rose}
\end{figure}
\noindent
This example illustrates an indicative property which relates the signed area of the embedded path to the relative correlation of individual data streams. 
\end{example}
\end{comment}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Further relationship between the signature terms and data points}
\label{subsec:further_relationship}

We now exemplify how the signature allows us to compute statistical moments between data streams.
%In the next sections we present a close relation between the statistical moments of a set of data $X$ and the terms of signature $S(X)^{I}$.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsubsection*{The lead-lag and the variance of data}
%\subsubsection*{Relationship between the lead-lag transformation and the variance of data}
Consider the lead-lag path (Fig.~\ref{fig:threeTriangls}) constructed from \eqref{eq:twoOneDimSeq_2} and its Lead-Lag transformation \eqref{eq:leadLagAlgo_X1}. We can decompose this figure into three right-angled isosceles triangles Fig.~\ref{fig:threeTriangls}. Note the direction of movement along this path, starting from the point $X^1_{t_0}$ and moving towards the endpoint $X^1_{t_3}$ corresponds to a negative sign, thus the total area will be negative. All three triangles have the same direction of movement resulting in the sum of their individual contributions. 
\begin{figure}[H]
\centering
%\includegraphics[scale = 0.3]{artwork/threeTriang}
\includegraphics[scale = 0.99]{artwork/leadlag_variance.pdf}
\caption{Decomposition of the full lead-lag path into three individual parts. The direction of movement along the path is shown by arrows.}
\label{fig:threeTriangls}
\end{figure}
\noindent
%
The absolute value of the total area is given by the sum of half areas of squares:
%
\begin{eqnarray}\label{eq:areaExample}
|A| &=& \frac{1}{2}\left[\left(X^{1}_{t_1} - X^{1}_{t_0}\right)\left(X^{1}_{t_1} - X^{1}_{t_0}\right)\right.\\\nonumber
&+& \left.\left(X^{1}_{t_2} - X^{1}_{t_1}\right)\left(X^{1}_{t_2} - X^{1}_{t_1}\right)\right.\\\nonumber
&+& \left.\left(X^{1}_{t_3} - X^{1}_{t_2}\right)\left(X^{1}_{t_3} - X^{1}_{t_2}\right)\right]\\\nonumber
&=& \frac{1}{2}\left[(3-1)^2 + (8-3)^2 + (6-8)^2\right] = 16.5
\end{eqnarray}
which exactly equals to the L{\'e}vy area enclosed by the lead-lag path $\{X^1\}$ and the straight line connecting the endpoints and can be computed via the signature terms \eqref{eq:LevyArea}.
%
Let us write:
%
\begin{eqnarray}\label{eq:quadraticVar}
[X]_t = \sum_{i=1}^{N}\left(X_{t_{i}}- X_{t_{i-1}}\right)^2,
\end{eqnarray}
which has the simple meaning of the \emph{quadratic variation} of the path constructed from $\{X_{t_i}\}_{i=0}^N$ and is related to the \emph{variance} of the path. Thus one can generally write for any sequence $\{X_{t_i}\}_{i=0}^N$:
%
\begin{eqnarray}\label{eq:qvar}
A_{\text{L{\'e}vy}}^{\{(X^{Lead}, X^{Lag})\}} = \frac{1}{2}[X].
\end{eqnarray}
%
For example, for the Lead-Lag path $\{(X^{1, Lead}, X^{1, Lag})\}$ \eqref{eq:leadLagAlgo_X1}, originated from a unidimensional sequence \eqref{eq:twoOneDimSeq_2}, the first order log-signature terms correspond to the total increments along each dimensions, and the second order  term is the L\'{e}vy area which equals to the quadratic variation of the unidimensional sequence:
%
%and equal to:
%
%\begin{eqnarray}\label{eq:increas}
%\Delta X^{2,Lead} = \Delta X^{2,Lag} = X^2_{4} - X^2_{1} = 6-1 = 5.
%\end{eqnarray}
%
%Putting all the terms together and omitting all unessential notation, we obtain the truncated log signature of $\{X^2\}$ from \eqref{eq:twoOneDimSeq_2} at level $L=2$:
%
\begin{eqnarray}\label{eq:logSigExampl}
\log S\left(\{(X^{1, Lead}, X^{1, Lag})\}\right) &=& \left(\Delta X^{1, Lead}, \Delta X^{1, Lag}, \frac{1}{2}[X^1], ...\right) \\\nonumber
&=& (5, 5, 16.5, ...)
\end{eqnarray}
%
%The only reason we are using the log signature above to present our result is because of its compactness and simplicity.
Equivalently, one can write the above result in terms of the signature with all the terms included:
%
\begin{eqnarray}
S\left(\{(X^{1, Lead}, X^{1, Lag})\}\right) = (1, 5, 5, 12.5, 29, -4, 12.5, ...).
\end{eqnarray}
%
and confirm that
\begin{eqnarray}
[\{X^1\}] = S^{(1,2)}\left(\{(X^{1, Lead}, X^{1, Lag})\}\right) - S^{(2,1)}\left(\{(X^{1, Lead}, X^{1, Lag})\}\right).
\end{eqnarray}
%We are free to work with either of these two representations of the signature, but certain applications will dictate the rationale behind a particular choice.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\subsubsection*{Mean and variance from composite path augmentations}

Next we demonstrate certain properties of paths which originate from composite transformations. Consider a series of subsequent transformations applied to a unidimensional sequence $\{X^1 \}$ \eqref{eq:twoOneDimSeq_2}, such as cumulative sum $CS(.)$ \eqref{eq:cumSumDef}, followed by base-point augmentation $BP(.)$ \eqref{eq:bp_augmentation} and followed by lead-lag transformation $LL(.)$ \eqref{eq:lead_stream}-\eqref{eq:lag_stream}. The resulting sequence could be written as composition of transformations:
%
\begin{eqnarray}\label{eq:composition_transformations}
\{\tilde{X}^1\} = LL \circ BP \circ CS(\{X^1\}) = LL\big(BP\big(CS(\{X^1\})\big)\big).
\end{eqnarray}
%
It follows that:
%Choosing even integer sequence for time augmentation $\{t_i\} = \{0,1, ..., i\}_{i=0}^{N}$, we get:
\begin{eqnarray}\label{eq:composition_transformations_example}
\{X^1_{t_i}\}_{i=0}^{N=3} &=& \{1,3,8,6\}\\
CS(\{X^1\}) &=& \{1,4,12,18\}\nonumber\\
\{Y^1\} := BP\big(CS(\{X^1\})\big) &=& \{0,1,4,12,18\}\nonumber\\
\{\tilde{X}^1\} = LL\big(BP\big(CS(\{X^1\})\big)\big) = \{(Y^{1,Lead}, Y^{1,Lag})\} &=& \{(0,0),(1,0),(1,1),(4,1),\nonumber\\&&(4,4),(12,4),(12,12),\nonumber\\&&(18,12),(18,18)\}.\nonumber
\end{eqnarray}
%
The resulting $\{\tilde{X}^1\}$ path is depicted in Fig. \ref{fig:ll_bp_cs}.
\begin{figure}[H]
\centering
%\includegraphics[scale = 0.3]{artwork/threeTriang}
\includegraphics[width=\linewidth]{artwork/ll_bp_cs.pdf}
\caption{The subsequent transformations of the original path $\{X^1\}$ into a resulting path $\{\tilde{X}^1\} = LL\big(BP\big(CS(\{X^1\})\big)\big)$ as shown in \eqref{eq:composition_transformations_example}.}
\label{fig:ll_bp_cs}
\end{figure}
\noindent
%
Explicitly \eqref{eq:composition_transformations_example} can be written as:
%\ilya{inserted zeros here}
\begin{eqnarray}
    Y^{1,Lead} &=& \{0, S_0, S_0, S_1, S_1, S_2, S_2, S_3, S_3\}\\
    Y^{1,Lag} &=& \{0,0,S_0, S_0, S_1, S_1, S_2, S_2, S_3\},\nonumber
\end{eqnarray}
where $S_k$ is a partial sum defined in \eqref{eq:cumSumDef}. We denote the signature of the composite transformation $\{\tilde{X}^1\}$ \eqref{eq:composition_transformations} of $\{X^1\}$ \eqref{eq:twoOneDimSeq_2} as:
\begin{eqnarray}\label{eq:xtilde_sig}
    \tilde{S} = S(\{\tilde{X}^1\}) = (1, \tilde{S}^{(1)}, \tilde{S}^{(2)}, \tilde{S}^{(1,1)}, \tilde{S}^{(1,2)}, \tilde{S}^{(2,1)}, \tilde{S}^{(2,2)}, ...).
\end{eqnarray}
%
Numerical evaluation of the expression in \eqref{eq:xtilde_sig} yields:
\begin{eqnarray}\label{eq:xtilde_sig_num}
    \tilde{S} = (1, 18,  18, 162, 217, 107, 162, ...).
\end{eqnarray}
%
From the definition of the signature terms and the cumulative sum, it follows that:
\begin{eqnarray}
    \tilde{S}^{(1)} &=& \int d {Y}^{1,Lag} = {Y}^{1,Lag}_{t_{N}} - {Y}^{1,Lag}_{t_0} = \Delta{X^{1,Lag}}\\ &=& BP\big(CS(\{X^1\})\big)_{t_4} - BP\big(CS(\{X^1\})\big)_{t_0}\nonumber\\ &=& S_{k=3} - 0\nonumber\\ &=& X^1_{t_0}+X^1_{t_1}+X^1_{t_2}+X^1_{t_3} - 0\nonumber\\ &=& 1+3+8+6 = 18.
\end{eqnarray}
%    \sum_{i=0}^{4}X^1_{t_i} - \sum_{i=0}^{0}X^1_{t_i}\nonumber\\ &=& 0 + \sum_{i=1}^{4}X^1_{t_i} - 0\nonumber,
%
Similarly, one can show that $\tilde{S}^{(2)} = \tilde{S}^{(1)}$. Therefore, the first order terms of the signature of the transformed sequence $\{\tilde{X}^1\}$ equal to the sum of the original sequence $\{{X}^1\}$:
\begin{eqnarray}
    \tilde{S}^{(1)} = \tilde{S}^{(2)} &=& \Delta{Y^{1,Lead}} = \Delta{Y^{1,Lag}}.
\end{eqnarray}
This result can be easily confirmed numerically by comparing the corresponding terms in \eqref{eq:xtilde_sig} and \eqref{eq:xtilde_sig_num}. In a similar fashion, one can demonstrate that quadratic variation \eqref{eq:quadraticVar} of the transformed sequence $[\{\tilde{X^1}\}]$ is proportional to \textit{variance} of the original $\{X^1\}$ \eqref{eq:twoOneDimSeq_2}.


\begin{comment}



Next, we demonstrate the quadratic variation \eqref{eq:quadraticVar} of the transformed sequence $[\{\tilde{X^1}\}]$ is proportional to \textit{variance} of the original $\{X^1\}$ \eqref{eq:twoOneDimSeq_2}. From the definition:
\begin{eqnarray}
   [\tilde{X}^{1,Lag}] &=& \sum_{i=0}^{N-1}\left(\tilde{X}^{1,Lag}_{i+1} - \tilde{X}^{1,Lag}_{i}\right)^2 =
\end{eqnarray}





\textbf{--------------- OLD stuff to ignore ---------------}


We choose to transform data points points using cumulative sums. Consider again the example \eqref{eq:twoOneDimSeq_2}. According to \eqref{eq:cumSumDef} and \eqref{eq:cumsum_x1}, its cumulative sum is:
%
\begin{eqnarray}
\tilde{X^1} &=& \{X^1_{t_0}, X^1_{t_0}+X^1_{t_1}, X^1_{t_0}+X^1_{t_1}+X^1_{t_2},X^1_{t_0}+X^1_{t_1}+X^1_{t_2}+X^1_{t_3}\}\\
&=& \{1,4,12,18\}. \nonumber
\end{eqnarray}
%
Pairing the above expression with the time component \eqref{eq:twoOneDimSeq_3}, we get a 2-dim path as shown in Fig.~\ref{fig:bRectilinearCumSum}. Augmenting the original series $\{X_i\}$ with base-point \eqref{eq:bp_augmentation} and truncating the signature of the new series $\{\tilde{X}\}$
\ilya{Maybe some of these $\{X\}$ and $\{\tilde X\}$ should be $\{X_i\}$ and $\{\tilde X_i\}$, particualrly in the next equation?} 
at level $L$ will determine the statistical moments up to level $L$ of the original sequence. Explicitly, for any general sequence $\{X_i\}$:
%
\begin{eqnarray}\label{eq:zerocumSum}
\{X\}_i \rightarrow \{0,\{X\}_{i=1}^N\} \rightarrow CS(\{X\}_i) = \{\tilde{X}\}_{i=0}^N = \left\{0,X_1,X_1 + X_2,\dots  \right\}.
\end{eqnarray}
%
One should pay attention to the indexing of the sequence, $i=1\rightarrow i=0$. As we have learnt from \eqref{eq:areaExample}-\eqref{eq:logSigExampl}, we can apply the lead-lag transform to the augmented sequence, compute the truncated signature at level $L=2$, and we will obtain quantities which are proportional to the first two statistical moments of the data points, namely \emph{mean} and \emph{variance}. For an arbitrary series $\{X\}_{i=1}^N$ and its cumulative sum representation $\{\tilde{X}\}_{i=1}^N$:
%
\begin{eqnarray}\label{eq:cumSumFirstTerm}
\Delta\tilde{X} &=& \sum_{i=1}^N X_i\\
QV(\tilde{X}) &=& \sum_{i=0}^{N-1}\left(\tilde{X}_{i+1} - \tilde{X}_{i}\right)^2 = \sum_{i=1}^{N} \left(X_i\right)^2
\end{eqnarray}


It is easy to see that these expressions are related to the {\it mean} and {\it variance} of $X$ if one makes use of the expected value. Namely, for a collection of data points $\{X_i\}_{i=1}^N$:
%
\begin{eqnarray}
%E[X]\;&=&\; \sum_{i=1}^N X_i \omega(X_i)\\
Mean(X)\;&=&\;E[X]\;=\;\frac{1}{N}\sum_{i=1}^N X_i\nonumber\;=\; \frac{\Delta\tilde{X}}{N}\;\;\;\text{(uniformly distributed data)}\\
Var(X)\;&=&\;E[\left( X-E[X]\right)^2]\;=\;E[X^2] - (E[X])^2\;=\;\frac{1}{N} \left( QV(\tilde{X}) - \frac{1}{N}(\Delta\tilde{X})^2\right)\nonumber
\end{eqnarray}
%
%where $\omega(X_i)$ is a distribution function (relative weight of each element) and, in the case of uniformly distributed $N$ values, equals to $\omega(X_i) = 1/N$.
Recall that the first two levels of the signature (log or full) correspond to the total increment and the L{\'e}vy area, which shows how these signature terms determine the first two statistical moments. Similarly, it is straightforward to demonstrate that the higher statistical moments can be obtained from the higher order signature terms.

\subsubsection*{Signature terms as a function of data points}


To make a closer connection and develop further the intuition behind the first terms of the signature of a data stream, we shall present two different examples of an embedding and the related signature terms.  First, consider the cumulative lead-lag embedding of $N$ data points $\{X_i\}_{i=1}^N$ (according to \eqref{eq:zerocumSum}) into a continuous path [cf. Fig.~\ref{fig:newLeadLag}], then the resulting truncated signature at level $L=2$ is simply given by:
%
\begin{eqnarray}
S(\tilde{X})|_{L=2}\;=\;\left(1,S^{(1)},S^{(2)},S^{(1,1)},S^{(1,2)},S^{(2,1)},S^{(2,2)} \right)
\end{eqnarray}
%
with
\ilya{Simone wrote this: In eq. (2.24) we have the formula for the terms $S^{(1,2)}$ and $S^{(2,1)}$ in the lead-lag embedding for the cumulative sum. It is clear that from the form that $S^{(1,2)}$ describes the area underneath the path (since we add the sum $\sum_i^N X_i^2$ to the other term) and for $S^{(2,1)}$ we subtract this term from the sum, hence $S^{(2,1)}$ describes 
the area over the graph. If I take a look back on p. 23 in fig. 12 it is explained the other way around.}
%
\begin{eqnarray}\label{eq:cumsumLeadLagSigTerms}
S^{(1)}\;=\;S^{(2)}\;&=&\;\sum_{i}^NX_i\\
S^{(1,1)}\;=\;S^{(2,2)}\;&=&\;\frac{1}{2}\left(\sum_{i}^NX_i\right)^2\nonumber\\
S^{(1,2)}\;&=&\;\frac{1}{2}\left[\left(\sum_{i}^NX_i\right)^2 + \sum_{i}^NX_i^2\right]\nonumber\\
S^{(2,1)}\;&=&\;\frac{1}{2}\left[\left(\sum_{i}^NX_i\right)^2 - \sum_{i}^NX_i^2\right].\nonumber
\end{eqnarray}
%
Note that, although we computed the signature of the transformed data $\{\tilde{X}\}$, the final result is given in terms of the original untransformed data $\{X_i\}$.


Next, we consider the untransformed original data $\{X_i\}$ with the same lead-lag embedding which results in the following expression for the signature:
%
\begin{eqnarray}
S(X)|_{L=2}\;=\;\left(1,S^{(1)},S^{(2)},S^{(1,1)},S^{(1,2)},S^{(2,1)},S^{(2,2)} \right)
\end{eqnarray}
%
with
%
\begin{eqnarray}\label{eq:bareLeadLagSigTerms}
S^{(1)}\;=\;S^{(2)}\;&=&\;\sum_{i}^{N-1}\left(X_{i+1}-X_i\right)\\
S^{(1,1)}\;=\;S^{(2,2)}\;&=&\;\frac{1}{2}\left(\sum_{i}^{N-1}\left(X_{i+1}-X_i\right)\right)^2\nonumber\\
S^{(1,2)}\;&=&\;\frac{1}{2}\left[\left(\sum_{i}^{N-1}\left(X_{i+1}-X_i\right)\right)^2 + \sum_{i}^{N-1}\left(X_{i+1}-X_i\right)\right]\nonumber\\
S^{(2,1)}\;&=&\;\frac{1}{2}\left[\left(\sum_{i}^{N-1}\left(X_{i+1}-X_i\right)\right)^2 - \sum_{i}^{N-1}\left(X_{i+1}-X_i\right)\right].\nonumber
\end{eqnarray}
%
Comparing \eqref{eq:cumsumLeadLagSigTerms} with \eqref{eq:bareLeadLagSigTerms}, one can immediately see how the cumulative sum of the terms affects the result. This observation is crucial for further applications of the signature approach, since each individual problem should be treated in the most suitable way. As an illustrative example, one can derive the empirical sample mean and sample variance from the signature terms. Considering data $\{X_i\}_{i=1}^N$ with the cumulative sum and the lead-lag embedding (as demonstrated in \eqref{eq:cumsumLeadLagSigTerms}), a bit of algebra brings us to:
%
\begin{eqnarray}
Mean(X)\;&=&\;\frac{1}{N}S^{(1)}\\
Var(X)\;&=&\;-\frac{N+1}{N^2}S^{(1,2)} + \frac{N-1}{N^2}S^{(2,1)},\nonumber
\end{eqnarray}
%
\ilya{Apparently the variance is wrong, according to Simone? It should be $Var(X)= \frac{N-1}{N^2} * S^{(1,2)}-\frac{N+1}{N^2} * S^{(2,1)}$}
where $N$ is the total number of data points in the sample. The possible caveat here is the degeneracy in the terms of the signature, causing this representation not to be unique and introducing a problem of colinearity of the signature terms. One of the standard approaches to resolve this problem is the shrinkage techniques, such as the LASSO \cite{tibshirani1996regression}, ridge or their hybrid combination known as the elastic net regularization \cite{zou2005regularization}.



% but for the {\it feature selection} procedure this does not matter, since a penalisation scheme (for example LASSO) will choose the best linear combination. This example demonstrates how the usual statistical moments are given by linear combinations of the terms of the signature.
%, and, as previously mentioned, higher order statistical moments are obtained in a similar way (as linear combinations of the signature terms) from the truncated signature at higher levels.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Working with the terms of the signature represents a more general way of looking at the usual statistical moments. The signature terms
%, also known as signature {\it coordinates} or {\it projections}
serve as descriptive statistics of data embedded into a path. As we have seen above, different functions applied to the signature terms $S^I(X)$ can result in familiar quantities (like $mean$ and $variance$), whilst other non-linear combinations of these terms may unveil more information hidden in the data. This process can be roughly presented in Fig.~\ref{fig:statSigComparison}:
%
\begin{figure}[H]
\centering
\includegraphics[width=\linewidth]{sigStat}
\caption{Conceptual comparison between the statistical approach to data and the signature approach. The signature transformation generates terms $S^I(X)$ which can be more flexible for data description.}
\label{fig:statSigComparison}
\end{figure}
\noindent
\end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%{\bf STILL UNCLEAR HOW TO RELATE SUM OF SQUARED ELEMENTS TO VARIANCE OR MOMENT}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
\subsubsection{Reconstruction of data from its signature}

For the rectilinear embedding of data points it is possible to get back the original data from the signature terms. We first briefly explain the theoretical background of the method \cite{lyons2011inversion,lyons2014inverting} and then demonstrate an application of this method to time-series. Consider a path embedded from some data points by a rectilinear interpolation. Such paths are also known as {\it axis} paths, since each movement along the path is parallel to the Euclidean coordinate axis. Consider first a path obtained from a single data point. Denoting the direction of axis by $\{e_1,e_2,\dots,e_d\}$ and the increment along each axis by $\{r_1,r_2,\dots,r_d\}$ in $d$-dimension, the endpoint of the path can be written as:
%
\begin{eqnarray}
X\;=\;r_1e_1 + r_2e_2 +\dots + r_de_d
\end{eqnarray}
%
then by multiplicativity, its full signature is given by:
%
\begin{eqnarray}
S(X)\;=\;e^{r_1 e_1}e^{r_2 e_2}\dots e^{r_d e_d}.
\end{eqnarray}
%
One can readily see that the signature term with the multi-index $I_k=\{e_1 e_2\dots e^2_k \dots e_d\}$ is given by:
%
\begin{eqnarray}
S^{I_k}\;=\;\frac{1}{2}r_1 r_2 \dots r_k^2\dots r_d,
\end{eqnarray}
%
from which it follows that:
%
\begin{eqnarray}
r_k\;=\;\frac{2 S^{I_k}(X)}{S^{I_0}(X)},
\end{eqnarray}
%
where $I_0 = \{e_1 e_2 e_3 \dots e_d\}$, thus recovering the length of each straight line component. Next we briefly review the example from \cite{levin2015learning} [cf. Section 4.1.1] where this method is presented in full detail. 

Suppose that $0<m<n\le N$, $m,n\in \mathbb{N}$, then the signature of a time-series $\{t_i,X_i\}_{i=m}^n$ uniquely determines the time-series $\{t_,X_i\}_{i=m}^n$ itself. More precisely, given a rectilinear path consisting of $N$ points, the truncated signature at level $N+1$ can reconstruct the original path. Consider time-series presented in Fig.~\ref{fig:bRectilinear} and given by \eqref{eq:twoOneDimSeq_2}-\eqref{eq:twoOneDimSeq_3}, then:
%
\begin{eqnarray}
\Delta X = T^{-1} S,
\end{eqnarray}
%
where 
%
\begin{eqnarray}
\Delta X = \left(\begin{matrix}
X_1\\
X_2 - X_1\\
X_3 - X_2\\
X_4 - X_3\\
\end{matrix}\right)\;;\;\;
T = \left(\begin{matrix}
1 & 1 & 1 & 1\\
t_1 & t_2 & t_3 & t_4\\
t_1^2 & t_2^2 & t_3^2 & t_4^2\\
t_1^3 & t_2^3 & t_3^3 & t_4^3
\end{matrix}\right)\;;\;\;
S = \left(\begin{matrix}
0!S^{2}(X)\\
1!S^{(1,2)}(X)\\
2!S^{1,1,2}(X)\\
3!S^{1,1,1,2}(X)
\end{matrix}\right).
\end{eqnarray}
%
One can see that the rectilinear embedding allows us to simplify computation of signature terms. Given a multi-index $I = \{1,1,...1,2\}$ with $k-1$ copies of $1$, results in:
%
\begin{eqnarray}
S^I\;=\; \frac{1}{k!}t_1^k X_1 + \sum_{i=1}^{n-1}\frac{1}{k!}t_i^k\left(X_{i+1} - X_i\right)
\end{eqnarray}
%
This result also means that time-series $\{X_i\}_{i=1}^n$ can be represented as a linear functional on its signature of the embedded path $\{t_i,X_i\}_{i=1}^n$.



\end{comment}

\begin{comment}
    >>>We start with the embedded path presented in Fig.~\ref{fig:embedding2DAnd3D}(a), for which the total increment and the signed area are depicted in Fig.~\ref{fig:signedArea1}.
%
\begin{figure}[ht]
\centering
\includegraphics[scale=0.4]{artwork/signed_area_1}
\caption{Example of signed area enclosed by the piece-wise linear path (blue) and the chord (red dashed line). The light blue area is negative and pink area is positive.}
\label{fig:signedArea1}
\end{figure}
\noindent

Computing the signature and the log signature of this path up to level $L=2$ gives:
%
\begin{eqnarray}
S(X) &=& (1, 7, 5, 24.5, 19, 16, 12.5) = (1,S^{(1)},S^{(2)},S^{(1,1)},S^{(1,2)},S^{(2,1)},S^{(2,2)})
\end{eqnarray}
%
and
\begin{eqnarray}
\log S(X) &=& (7, 5, 1.5) = (S^{(1)}, S^{(2)}, S^{[1,2]}),\nonumber
\end{eqnarray}
%
where the last term in $\log S(X)$ is given by $\frac{1}{2}(S^{(1,2)}-S^{(2,1)})$ and corresponds to the total area between the endpoints. The fact that it is positive means that the {\it pink} area is larger than the {\it light blue} one. The geometric interpretation of the second order terms $S^{(1,2)}$ and $S^{(2,1)}$ are presented in \fig{fig:areasS12andS21}.

\begin{figure}[htb]
\begin{minipage}{.45\linewidth}
\centering
\includegraphics[scale=.3]{artwork/area_S21_n}
\subcaption{Area given by the term $S^{(1,2)}$ = 19.\label{fig:areasS12andS21a}}
\end{minipage}%
\begin{minipage}{.45\linewidth}
\centering
\includegraphics[scale=.3]{artwork/area_S12_n}
\subcaption{Area given by the term $S^{(2,1)}$ = 16.}
\end{minipage}
\centering
\caption{The geometric meaning of the terms $S^{(1,2)}$ and $S^{(2,1)}$. The left panel (a) represents the area enclosed by the path and two perpendicular dashed lines passing through the endpoints of the path, while the right panel (b) shows another possibility for the area to be enclosed by the path and two perpendicular dashed lines passing through the endpoints.}
\label{fig:areasS12andS21}
\end{figure}
\noindent

Switching the order of integration over the path in the terms $S^{(1,2)}$ and $S^{(2,1)}$ gives rise to two areas which complete each other and add up to the total area of a rectangular with side lengths $X^1$ and $X^2$. This simple geometrical meaning is nothing but the shuffle product relation:
%
\begin{eqnarray}
S^{(1)}\cdot S^{(2)}  &=& S^{(1,2)} + S^{(2,1)}\nonumber\\
5\cdot 7 &=& 19+16.
\end{eqnarray}
%
The geometric interpretation of the higher order terms is less intuitive and we omit this discussion.

\end{comment}

%The geometric interpretation of the higher order terms is less intuitive, but one can think in terms of dimensional analysis: the first terms (which have a single index) correspond to a single integral, which has dimension of length to the power 1 (or \emph{length}): $S^{1},S^{2}\propto l^1$, second order terms contain two-fold iterated integrals, corresponding to length squared (or \emph{area}): $S^{i,j}\propto l^{2}$, third order terms correspond to three-fold integrals (or \emph{volume}): $S^{i,j,k}\propto l^3$. Continuing with this logic, one can view the signature transformation as an infinite expansion of hyper-volume objects: length, area, volume, etc. We leave further development of this intuition to the reader.


%
%
%\begin{eqnarray}
%logS(X) \propto (l^0,l^1,l^2,l_1^3,l_2^3,l_1^4,l_2^4,l_3^4,\dots)
%\end{eqnarray}
%
%but we leave further development of this intuition to the reader.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> section_files_tex/2_2.tex <==
\subsection{Machine learning with signature features}

The signature of a path is a collection of iterated integrals that succinctly captures the path's geometric properties and encodes its essential information. This makes it particularly well-suited for machine learning applications for sequential data and time-series analysis. The workflow is simple and is summarised in the following algorithm:
%
$$ \text{{\it data}} \rightarrow \text{{\it path}} \rightarrow \text{{\it signature of path}} \rightarrow \text{{\it features of data}}\rightarrow \text{{\it learning algorithms}} $$
%The main idea of using the signature transformation for machine learning problems is motivated by its ability to extract characteristic features from data. As already discussed, embedding data into a path and computing its signature provides us with important information about the original data.
This algorithm is general and works for any type of sequential data which can be embedded into a continuous path. The extracted features might be used for various types of machine learning applications, including both supervised and unsupervised learning. For example, one can classify time-series or distinguish clusters of data. One of the advantages of feature extraction with the signature method is that the signature is sensitive to the geometric shape of a path.
%For example, if two data sets possess identical statistical moments, signature will generate distinct features.
Sensitivity to the geometric shape of the input data has lead to a successful application of the signature method to Chinese character recognition problem \cite{graham2013sparse}. One of the most known and natural applications of the signature method is in quantitative finance, namely analysis of time-series data \cite{gyurko2014extracting,levin2015learning}. Time-series represent ordered sequential data which is a natural candidate for creating a path, followed by computing the signature and applying machine learning algorithms for further analysis.
%Any type of time-ordered sequential data naturally fits into the signature framework.
Moreover, if the input data come from several parallel sources, this will result in a multi-dimensional path. An example for such a type of data is {\it panel} data (in Econometrics) or {\it longitudinal} data (in Medicine, Psychology, Biostatistics etc.) which involve repeated observations of the same quantity over periods of time.

Concluding this brief introduction to applications of the signature method, we emphasise that this method introduces a new concept of dealing with data: thinking of data as geometric paths and using the path signature method to analyse this data.
%{\it ``Our mathematical study of these objects does not encourage us to think
%broadly about the truly enormous range of "paths" that occur. Although
%most mathematicians would agree on a definition of a path, most have a
%rather stereotyped and limited imagination about the variety of paths that
%are "in the wild"." --- Terry Lyons}
In the rest of this subsections, we demonstrate how to apply the signature transformation to problems in statistical machine learning with streamed data, focusing on the common analytical task of classification.  However, other machine learning and inferential statistical tasks with streamed data can also be performed using the signature formalism, including regression, clustering, and kernel learning, some of which we review in Section \ref{subsec:overview_applications}.


\subsubsection{Classification of hand-written digits: an example}

In this section, we demonstrate the application of the path signature method to a machine learning pen-based recognition of handwritten digits classification task. The data set is available from the University of California, Irvine, Machine Learning Repository \cite{misc_pen-based_recognition_of_handwritten_digits_81}. The data set comprises 250 hand-written integer numbers in the range from 0 to 9, generated by 44 writers using a tablet with a stylus. The data represent a collection of consecutive data points represented by $(x, y)$ coordinates. The raw data that were captured from the tablet consisted of integer values and were normalised to lie in the range between 0 and 100. The consecutive data points were resampled and represented as a sequence of coordinate pairs $(x_i, y_i), i=1,\dots,8$, regularly spaced on the trajectory. An example of ten random digits in the tabular format are shown in Tab. \ref{tab:digits} and first four rows are displayed in Fig. \ref{fig:digits}.
%
\begin{table}[htp!]
    \centering
    \begin{adjustbox}{width=\textwidth}
    \begin{tabular}{rrrrrrrrrrrrrrrrr}
     x\_1 &  y\_1 &  x\_2 &  y\_2 &  x\_3 &  y\_3 &  x\_4 &  y\_4 &  x\_5 &  y\_5 &  x\_6 &  y\_6 &  x\_7 &  y\_7 &  x\_8 &  y\_8 &  Label \\
    \hline
      12 &   87 &    0 &   44 &   20 &    4 &   66 &    0 &  100 &   30 &   89 &   75 &   49 &  100 &   13 &   77 &      0 \\
      23 &   76 &   52 &  100 &  100 &   98 &   79 &   71 &   63 &   50 &   82 &   19 &   49 &    0 &    0 &    7 &      3 \\
       0 &   40 &   32 &   59 &   71 &   82 &  100 &  100 &   85 &   75 &   71 &   50 &   64 &   25 &   75 &    0 &      1 \\
       0 &  100 &   53 &   95 &   80 &   66 &   69 &   30 &   66 &    0 &  100 &   30 &   61 &   36 &    7 &   39 &      7 \\
       0 &   67 &   43 &   74 &   78 &   91 &  100 &  100 &   95 &   74 &   87 &   49 &   84 &   23 &   96 &    0 &      1 \\
      10 &   97 &    2 &   47 &   24 &    1 &   74 &    0 &  100 &   43 &   82 &   90 &   33 &  100 &    0 &   65 &      0 \\
       0 &   48 &   30 &   67 &   65 &   85 &  100 &  100 &   84 &   75 &   65 &   51 &   47 &   25 &   34 &    0 &      1 \\
      55 &   70 &   73 &  100 &   62 &   66 &   49 &   26 &   30 &    0 &    0 &    2 &   50 &    3 &  100 &    6 &      1 \\
     100 &  100 &   66 &   88 &   32 &   66 &    7 &   39 &    0 &   10 &   44 &    0 &   62 &   18 &   14 &   22 &      6 \\
      85 &  100 &   43 &   76 &   11 &   48 &    0 &   17 &   44 &    0 &  100 &   10 &   59 &   20 &    1 &   10 &      6 \\
    \hline
    \end{tabular}
    \end{adjustbox}
    \caption{An example of ten random samples of hand-written digits in a tabular format from the Pen-based Recognition of Handwritten Digits data set \cite{misc_pen-based_recognition_of_handwritten_digits_81}. Columns denoted by $x_i$, and $y_i$ $(i=1,\dots,8)$ correspond to coordinates (features) and the last column designates the class label of digits.}
    \label{tab:digits}
\end{table}
%
\begin{figure}[htp!]
    \centering
    \includegraphics[width=\linewidth]{artwork/fig_22_digits.pdf}
    \caption{Pictorial representation of the first four rows from the Table \ref{tab:digits}. From left to right: `0', `3', `1' and `7'. The solid red dot represents the starting point $(x_1, y_1)$.}
    \label{fig:digits}
\end{figure}
%
Each data sample is represented by a two dimensional coordinate sequence $(x_i, y_i) \in \mcX$, that can be seen as a path in $\mathbb{R}^2$. For the sake of simplicity, we apply the signature transformation without composite augmentations. Following the steps outlined in Section \ref{sec:signature_of_a_path}, the signature will be the feature map:
%
\begin{equation}
    S:\mcX \rightarrow \Sigma,
\end{equation}
where $S^{I}\in\Sigma$ are the elements of the infinite signature series \eqref{eq:definSig} and $I$ being a multi-index defined in \eqref{eq:words_def}. For example, applying the level-2 truncated signature transformation on the first four rows:
%
\begin{eqnarray}
    X^{zero} = \{(x_i, y_i)\}_{i=1}^{N=8} &=& \{(12, 87), (0, 44), (20, 4), (66, 0)\\
     &=& (100, 30), (89, 75), (49, 100), (13, 77)\}\nonumber\\
    X^{three} &=& \{(23, 76), (52, 100), (100, 98), (79, 71)\nonumber\\
     &=& (63, 50), (82, 19), (49, 0), (0, 7)\}\nonumber\\
    X^{one} &=& \{(0, 40), (32, 59), (71, 82), (100, 100)\nonumber\\
     &=& (85, 75), (71, 50), (64, 25), (75, 0)\}\nonumber\\
    X^{seven} &=& \{(0, 100), (53, 95), (80, 66), (69, 30)\nonumber\\
     &=& (66, 0), (100, 30), (61, 36), (7, 39)\}\nonumber     
\end{eqnarray}
will yield:
\begin{eqnarray}
    S(X^{zero}) &=& (1, 1, -10, 0.5, 7044.5, -7054.5, 50)\\
    S(X^{three}) &=& (1, -23, -69, 264.5, -4893, 6480, 2380.5)\nonumber\\
    S(X^{one}) &=& (1, 75, -40, 2812.5, -4660, 1660, 800)\nonumber\\
    S(X^{seven}) &=& (1, 7, -61, 24.5, -3693, 3266, 1860.5)\nonumber
\end{eqnarray}
%
Applying the signature transformation on each row of the data matrix in Tab.~\ref{tab:digits} will generate the \textit{signature feature matrix}:

\begin{table}[htp!]
    \centering
    \begin{tabular}{rrrrrrrr}
     1 &   $S^{(1)}$ &   $S^{(2)}$ &     $S^{(1,1)}$ &       $S^{(1,2)}$ &      $S^{(2,1)}$ &      $S^{(2,2)}$ &  Label \\
    \hline
     1 &   1 & -10 &    0.5 &  7044.5 & -7054.5 &   50 &      0 \\
     1 & -23 & -69 &  264.5 & -4893 &  6480 & 2380.5 &      3 \\
     1 &  75 & -40 & 2812.5 & -4660 &  1660 &  800 &      1 \\
     1 &   7 & -61 &   24.5 & -3693 &  3266 & 1860.5 &      7 \\
     1 &  96 & -67 & 4608 & -7123 &   691 & 2244.5 &      1 \\
     1 & -10 & -32 &   50 &  7388.5 & -7068.5 &  512 &      0 \\
     1 &  34 & -48 &  578 & -4179 &  2547 & 1152 &      1 \\
     1 &  45 & -64 & 1012.5 &   178 & -3058 & 2048 &      1 \\
     1 & -86 & -78 & 3698 &  5984 &   724 & 3042 &      6 \\
     1 & -84 & -90 & 3528 &  6028.5 &  1531.5 & 4050 &      6 \\
    \hline
    \end{tabular}
    \caption{The signature feature matrix from the original data presented in Tab. \ref{tab:digits} and the corresponding labels.}
\end{table}
%
Now, one can use the signature feature matrix as input to statistical hypothesis tests for downstream analytical tasks or machine learning algorithms to predict the class labels. 

Another interesting observation is that the higher order signature terms can capture more nuanced patterns of paths. Consider only samples of hand-written `zero' and `eight' digits, such as shown in Fig.~\ref{fig:digits_8_0}.
\begin{figure}[htp!]
    \centering
    \includegraphics[width=\linewidth]{artwork/fig_22_digits_0_8.pdf}
    \caption{Examples of hand-written zeros and eights. From left to right: `8', `0', `0', `8'. The solid red dot represents the starting point $(x_1, y_1)$.}
    \label{fig:digits_8_0}
\end{figure}
Both `zero' and `eight' shapes share a similar geometric pattern: the starting and then end points usually coincide. However, the \textit{areas} enclosed by both shapes will be different due to their orientations as discussed in Section \ref{sec:signed_area}. The clear differences between the distributions of the first $S^{(1)}, S^{(2)}$ and second order $S^{(1,2)}, S^{(2,1)}$ signature terms are shown in Fig.~\ref{fig:sig_s1_s2_vs_s12_s21} and can improve the performance of machine learning or statistical approaches.
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{artwork/fig_22_digits_0_8_area.pdf}
    \caption{The distribution of the first (left panel) and second (right panel) signature terms describing `zero' and `eight' digits. The second order signature terms, that are proportional to a signed enclosed area, demonstrate good separability between two classes.}
    \label{fig:sig_s1_s2_vs_s12_s21}
\end{figure}


Furthermore, the signature feature matrix can also be used for unsupervised learning tasks, including dimensionality reduction for clustering approaches. For example, applying the Uniform Manifold Approximation and Projection (UMAP) for Dimension Reduction method \cite{mcinnes2018umap} on the signature feature matrix, one can find clusters of points belonging to the same class label, see Fig.~\ref{fig:UMAP}.
%
\begin{figure}
    \centering
    \includegraphics[width=0.7\linewidth]{artwork/fig_22_digits_umap.pdf}
    \caption{Projection of the signature feature space from $\mathbb{R}^7$ onto $\mathbb{R}^2$ using UMAP. The right column designates class labels $0, \dots, 9$.}
    \label{fig:UMAP}
\end{figure}



%\subsubsection{Learning with multivariate time-series}



\begin{comment}


\subsubsection{Linear Regression}

% The main goal of this approach is to identify the specific feature set of the observed data and linearise the functional relationships between them (features).
In~\cite{levin2015learning}, Levin, Lyons, and Ni addressed an application of the signature method to time-series analysis and develop a new regression method based on the expected signature of paths. This method of linear regression on the signature of data streams is general and allows explicit computations and predictions. The {\it the expected signature model} as a linear mapping: $L: X\mapsto Y$
%
\begin{eqnarray}
Y = L(X) + \epsilon,
\end{eqnarray}
%
with $E[\epsilon]=0$ and $X\in T((\R^d)),\; Y\in T((\R^e))$, where 
\begin{eqnarray}
T((\R^d)) = \prod_{n=0}^{\infty} (\R^d)^{\otimes n}
\end{eqnarray}
%
is the algebra of tensor series over $\R^d$. We briefly outline the main idea of this model. Consider the univariate time-series ({\it returns}) denoted by $\{r_i\}_{i=1}^N$ and some fixed $k\in \mathbb{N}$, such that $1 < k < N$. Define the {\it p-past} returns up to time $t_k$ by $F_k = \{r_i\}_{i=k-p}^k$ and the {\it q-future} returns (from time $t_{k+1}$) by $G_{k+1} = \{r_i\}_{i=k+1}^{k+q}$. The signatures of $F_k$ and $G_{k+1}$ are respectively: 
%
\begin{eqnarray}\label{eq:pastFutureSig}
X_k &=& S\left(\{t_i,r_i\}_{i=k-p}^k\right)\\
Y_k &=& S\left(\{t_i,r_i\}_{i=k+1}^{k+q}\right).\nonumber
\end{eqnarray}
%
The definition of the Expected Signature model $ES(p,q,n,m)$ states that the stationary time-series $\{r_i\}_{i=1}^N$ satisfies the assumptions of the $ES$ model with parameters $p,q,n,m$ if there exists a linear functional $f:T^n\left(\mathbb{R}^2\right) \mapsto T^n\left(\mathbb{R}^2\right)$ such that:
%
\begin{eqnarray}
\rho_m\left(S(\{r_{t+i}\}_{i=1}^q)\right) = f\left(\rho_m\left(S(\{r_{t-i}\}_{i=0}^p)\right)\right) + a_t,
\end{eqnarray}
%
where $N \geq p+q$ is a positive integer, $m$ is the depth of truncation of signature, and the residual term $a_t$ satisfies $E[a_t|F_t] = 0$. Let $\mu_k$ be the expectation of $S(\{t_i,r_i\}_{i=k+1}^{k+q})$
%
\begin{eqnarray}\label{eq:meanEq}
\mu_k = E[S(\{t_i,r_i\}_{i=k+1}^{k+q})|F_k].
\end{eqnarray}
%
It thus follows from the ES model that
%
\begin{eqnarray}
\mu_k = f(X_k),
\end{eqnarray}
%
where $X_k$ is defined in \eqref{eq:pastFutureSig} with both $\mu_k$ and $a_k$ in $T((\R^2))$. Next, the conditional covariance of the signature of the future return conditioned on $F_k$ is defined as
%
\begin{eqnarray}\label{eq:volatilEq}
\Sigma_k^2(I,J) = Cov\left(S^I(Y_k),S^J(Y_k)|F_k\right),
\end{eqnarray}
%
where $I,J$ are two multi-indexes as defined previously in the text. In time-series analysis, \eqref{eq:meanEq} corresponds to the mean equation for $Y_k$, and \eqref{eq:volatilEq} is the volatility equation for $Y_k$. The fundamental assumption of the ES model is the stationarity of the time-series $\{r_i\}$, which is common in time-series analysis.

It has been shown that many standard autoregressive models (AR, ARCH, GARCH, etc.) are special cases of the ES model. For example, given the time-series $\{t_i,r_i\}$ the mean equation and volatility are written as:
%
\begin{center}
\begin{tabular}{r l l}

 & AR & ES \\ 

$m_k :$ & $E[r_{k+1}|F_k]$ & $S^{(2)}(\mu_k)$ \\ 

$\sigma^2_k :$ & $Var[r_{k+1}|F_k]$ & $2S^{(2,2)}(\mu_k) - \left(S^{(2)}(\mu_k)\right)^2$. \\ 

\end{tabular} 
\end{center}
%
Several important properties linking the autoregressive models and ES model are proven in~\cite{levin2015learning}. One of them states that if a time-series $\{r_k\}$ satisfies the assumptions of ARCH(q) model and its mean equation is given by
%
\begin{eqnarray}
\mu_k = \beta_0 + \sum_{i=1}^Q\beta_i r_{k-i},
\end{eqnarray}
%
then there exists a sufficiently large integer $n$ such that the time-series $\{r_k\}$ satisfies the assumption of $ES(q+Q,1,n,2)$. Also, the model $ES(p,1,n,2)$ is considered as a classical time-series, where the signature of the past returns as an explanatory variable.

The work in~\cite{levin2015learning} provides explicit numerical benchmarks between various autoregressive models and the expected signature model for various set-ups and configurations of the models.

========================================================






In this section we demonstrate an explicit example of an application of the signature method to classification of time-series. This method is moreover easily applied to analysis of sequential data of any type. In the next section we overview some of the recent applications of the signature method to various problem in machine learning.


We aim at learning a classifier which discriminates between two types of univariate time-series, synthetically simulated using the $ARMA(p,q)$ model. The difference between time-series is encoded in different value of the model parameters. Consider a collection of observations of time-series $\{Y_{i,j}\}$ labeled by two indices $i,j$, where the first index $i$ denotes each distinct time-series and the second index $j$ accounts for the measurement at time $t_j$. %It is convenient to organize this type of data set into a two-dimensional matrix of size $N\times P$, with $i = 1,...,N $ and $j = 1,...,P$. To demonstrate a toy-model example of time-series classification, we consider a general $ARMA$ model, where the difference between two models is characterized by different value of variables $(p,q)$. 

The $ARMA(p,q)$ model is {\bf A}uto{\bf R}egressive {\bf M}oving {\bf A}verage model with parameters $p$ (the order of the autoregressive model) and $q$ (the order of the moving-average model). This is a superposition of the autoregressive $AR(p)$ and the moving-average $MA(q)$ models:
%
\begin{eqnarray}
\textit{AR(p)}\;&:& Y_t = \phi_0 + \phi_1 Y_{t-1} + \phi_2 Y_{t_2} + \dots + \phi_p Y_{t-p} + \epsilon_t \\
\textit{MA(q)}\;&:& Y_t = \mu + \epsilon_t + \theta_1\epsilon_{t-1} + \theta_2\epsilon_{t-2} + \dots + \theta_q \epsilon_{t-q}, \nonumber
%\textit{I(d)}\;&:&\;L^d Y_t = Y_{t-d}\nonumber
\end{eqnarray}
%
where $\mu$ is the mean of the series, $\theta_i$ with $\phi_i$ are the parameters of the models and $\epsilon_{t-i}$ is the white noise error term. We are not diving into the mathematical foundation of the model, but rather focus on its application. To demonstrate how the feature extraction method works in this case, we create a binary classification problem using the ARMA model. We generate 1000 distinct time-series (500 time-series of each class) of length 100. In this particular, the case two classes correspond to the following models:
%
\begin{eqnarray}\label{eq:arma101}
\textit{class ``0"}\;: Y_t - 0.4Y_{t-1}\;=\;0.5 + \epsilon_t + 0.5\epsilon_{t-1}\\
\textit{class ``1"}\;: Y_t - 0.8Y_{t-1}\;=\;0.5 + \epsilon_t + 0.7\epsilon_{t-1}\nonumber  
\end{eqnarray}
%
where $\epsilon_t$ is normally distributed with zero mean and unit variance. An example of a time-series from each class is depicted in Fig.~\ref{fig:arimaTimeSeries}.
%
\begin{figure}[htb]
\centering
\includegraphics[width=0.5\linewidth]{artwork/arma_011}
\centering
\caption{Example of time-series $Y_{i}$ from two distinct classes generated from ARMA(1,1) model specified by \eqref{eq:arma101}.}
\label{fig:arimaTimeSeries}
\end{figure}
\noindent
%
To give a simple intuitive picture, the resulting two-classes time-series data $\{Y_i\}$ and their class labels are organised in a matrix form:

\begin{center}
\begin{tabular}{cccccc|c}
$t_{1}$ & $t_{2}$ & $t_{3}$ & $t_{4}$ & $\dots$ & $t_{100}$ & Class \\ 
\hline 
$Y_{1,1}$ & $Y_{1,2}$ & $Y_{1,3}$ & $Y_{1,4}$ & $\dots$ & $Y_{1,100}$ & 0 \\ 
$Y_{2,1}$ & $Y_{2,2}$ & $Y_{2,3}$ & $Y_{2,4}$ & $\dots$ & $Y_{2,100}$ & 0 \\ 
$Y_{3,1}$ & $Y_{3,2}$ & $Y_{3,3}$ & $Y_{3,4}$ & $\dots$ & $Y_{3,100}$ & 0 \\  
$\vdots$ & $\vdots$ & $\vdots$ & $\vdots$ & $\vdots$ & $\vdots$ & $\vdots$ \\
$Y_{500,1}$ & $Y_{500,2}$ & $Y_{500,3}$ & $Y_{500,4}$ & $\dots$ & $Y_{500,100}$ & 0 \\ 
$Y_{1,1}$ & $Y_{1,2}$ & $Y_{1,3}$ & $Y_{1,4}$ & $\dots$ & $Y_{1,100}$ & 1 \\ 
$Y_{2,1}$ & $Y_{2,2}$ & $Y_{2,3}$ & $Y_{2,4}$ & $\dots$ & $Y_{2,100}$ & 1 \\ 
$Y_{3,1}$ & $Y_{3,2}$ & $Y_{3,3}$ & $Y_{3,4}$ & $\dots$ & $Y_{3,100}$ & 1 \\  
$\vdots$ & $\vdots$ & $\vdots$ & $\vdots$ & $\vdots$ & $\vdots$ & $\vdots$ \\
$Y_{500,1}$ & $Y_{500,2}$ & $Y_{500,3}$ & $Y_{500,4}$ & $\dots$ & $Y_{500,100}$ & 1 \\   
\end{tabular} 
\end{center}
%
We outline the essential steps of the procedure.
\begin{itemize}
\item	create a continuous path $X_i$ from each time-series $\{Y_i\}$ (row-wise)
\item	if needed, make use of the lead-lag transform to account for the variability in data
\item	compute the truncated signature $S(X_i)|_L$ of the path $X_i$ up to level $L$
\item	use the terms of signature $\{S_i^I\}$ as features 
\end{itemize}
%
\ilya{Simone wrote: In Chapter 2.2.1 when applying the data to a problem from time series, I don't quite understand how you have approached the subject. On p.30 it says, that a 'continuous' path $X_i$ was created and then again on the bottom, it says that $X_i$ contains the lead and lag transform of the original data as a cumulative sum.}
Following the aforementioned steps, each observation $\{Y_i\}$ is converted into a two-dimensional path. We also used a cumulative sum transformation \eqref{eq:zerocumSum}:
\begin{eqnarray}
X_i = \left\{\left(\tilde{Y}^{lead}_i,\tilde{Y}^{lag}_i\right)\right\},
\end{eqnarray}
%
and then the signature terms are computed:
\begin{eqnarray}
S(X_i)\;=\;\left(1, S_i^{(1)}, S_i^{(2)}, S_i^{(1,1)}, S_i^{(1,2)},\dots, S_i^{I},\dots\right).\end{eqnarray}
The resulting feature matrix has the form:
\begin{center}
\begin{tabular}{cccccc|c}
\multicolumn{6}{c}{Feature Set} & Class\\
%&  &  & & Feature  & Set & Class \\ 
\hline 
$\hat{S}_1^{(1)}$ & $\hat{S}_1^{(2)}$ & $\hat{S}_1^{(1,1)}$ & $\hat{S}_1^{(1,2)}$ & $\dots$ & $\hat{S}_1^{I}$ & 0 \\ 
$\hat{S}_2^{(1)}$ & $\hat{S}_2^{(2)}$ & $\hat{S}_2^{(1,1)}$ & $\hat{S}_2^{(1,2)}$ & $\dots$ & $\hat{S}_2^{I}$ & 0 \\
$\hat{S}_3^{(1)}$ & $\hat{S}_3^{(2)}$ & $\hat{S}_3^{(1,1)}$ & $\hat{S}_3^{(1,2)}$ & $\dots$ & $\hat{S}_3^{I}$ & 0 \\
$\vdots$ & $\vdots$ & $\vdots$ & $\vdots$ & $\vdots$ & $\vdots$ & $\vdots$ \\
$\hat{S}_{500}^{(1)}$ & $\hat{S}_{500}^{(2)}$ & $\hat{S}_{500}^{(1,1)}$ & $\hat{S}_{500}^{(1,2)}$ & $\dots$ & $\hat{S}_{500}^{I}$ & 0 \\
$\hat{S}_1^{(1)}$ & $\hat{S}_1^{(2)}$ & $\hat{S}_1^{(1,1)}$ & $\hat{S}_1^{(1,2)}$ & $\dots$ & $\hat{S}_1^{I}$ & 1 \\ 
$\hat{S}_2^{(1)}$ & $\hat{S}_2^{(2)}$ & $\hat{S}_2^{(1,1)}$ & $\hat{S}_2^{(1,2)}$ & $\dots$ & $\hat{S}_2^{I}$ & 1 \\
$\hat{S}_3^{(1)}$ & $\hat{S}_3^{(2)}$ & $\hat{S}_3^{(1,1)}$ & $\hat{S}_3^{(1,2)}$ & $\dots$ & $\hat{S}_3^{I}$ & 1 \\
$\vdots$ & $\vdots$ & $\vdots$ & $\vdots$ & $\vdots$ & $\vdots$ & $\vdots$ \\
$\hat{S}_{500}^{(1)}$ & $\hat{S}_{500}^{(2)}$ & $\hat{S}_{500}^{(1,1)}$ & $\hat{S}_{500}^{(1,2)}$ & $\dots$ & $\hat{S}_{500}^{I}$ & 1 \\   
\end{tabular} 
\end{center}
%
%where the element $S_i^I$ corresponds to $I$-th signature term of $i$-th times series observation. 
It is usual practice to standardise the signatures column-wise, where the {\it hat} corresponds to standardised values, computed by subtracting from each value $S_i^I$ the column mean and dividing by the column standard deviation.

For sake of simplicity, we compute the truncated signature up to level $L=2$, remove the first constant term and thus produce a 6-dimensional feature space. The example of the signature and the log-signature terms projected on the two dimensional plane are presented in Fig.~\ref{fig:exampleOfSignature}.


\begin{figure}[H]
\centering
	\subcaptionbox{\label{fig:sigfets}}%Mean and standard deviation as feature space for two classes.}%
	  [.47\linewidth]{\includegraphics[width=0.5\linewidth]{artwork/sigFeat_56_1}}
\centering	  
	\subcaptionbox{\label{fig:logsigfets}}%Terms of log signature of path embedded from the data.}%
	  [.47\linewidth]{\includegraphics[width=0.5\linewidth]{artwork/logSigFeat_56}}
\caption{Feature extraction from ARMA(1,1) time-series. The left panel (a) represents two signature terms $S^{(1,2)}$ and $S^{(2,1)}$, while the right panel (b) shows the first and the third terms of log-signature $\log S^{1}$,$\log S^{[1,2]}$.}
\label{fig:exampleOfSignature}
\end{figure}
\noindent
%
Since we are not aiming to compare different classification algorithms, but rather to demonstrate the signature method at work, we arbitrarily choose a standard logistic regression algorithm with LASSO \cite{tibshirani1996regression} penalization scheme. The relevant features which are selected by LASSO are: $$\left\{S^{(1)}, S^{(2)}, S^{(1,2)}, S^{(2,1)}\right\}.$$ The classification results are summarised in Table~\ref{tab:tab2}.

\begin{table}[htb]
\centering
	\subcaptionbox{Training data set (70$\%$)\\ with accuracy 0.92\label{tab:tabA}}
	  [.48\linewidth]
	  {
	  	\begin{tabular}{|c|c|c|}
		\hline 
		\diagbox[width=8em]{True}{Predicted} & 0 & 1  \\ 
		\hline 
			0 & 326 & 20  \\ 
		\hline 
			1 & 35 & 319  \\ 
		\hline 
		\end{tabular} 
	  }
\centering	  
	\subcaptionbox{Testing data set (30$\%$)\\ with accuracy 0.90 \label{tab:tabB}}
	  [.47\linewidth]
	  {
	  	\begin{tabular}{|c|c|c|}
		\hline
		\diagbox[width=8em]{True}{Predicted} & 0 & 1  \\ 
		\hline 
		0 & 139 & 15  \\ 
		\hline 
		1 & 14 & 132  \\ 
		\hline 
		\end{tabular} 
	  }
\caption{Confusion matrix of the classification showing both the training and the testing data sets results.}
\label{tab:tab2}
\end{table}
\noindent


Using the full signature for feature extraction is conceptually similar to working with basis functions. Having obtained the signature terms as representing features of data, one can continue further with standard methods in machine learning to solve problems.
\end{comment}



\begin{comment}
\subsubsection{Dealing with missing data in time-series}

\ilya{Could also mention unevenly sampled data.}

Sometimes sequential observations are not complete and some values might be missing due to various reasons. For example in medical follow up studies patients may not provide response data at required times due to personal reasons or clinical conditions. There are many ways to deal with missing data, for example imputing, various sophisticated interpolation methods, Gaussian smoothing kernels, and many more techniques are thoroughly studied and described in the literature. These methods might perform well and even result in robust analysis and predictions, but conceptually, imputing missing values may change the underlying information about initial data and thus create biased analysis which masks the original message. 

One of the methods to treat missing values is to introduce a new binary variable: {\it indicator} matrix $R_{ij}$ along with observations $Y_{ij}$, where $i$ corresponds to individual time-series and $j$ denotes a time instance as explained in  \cite{diggle2002analysis}. The elements of the indicator matrix are defined by:
%
\begin{eqnarray}
R_{ij}\;=\;
\left\{
	\begin{array}{ll}
		0  & \;\;\mbox{if } Y_{ij}\;\; \mbox{observed}, \\
		1  & \;\;\mbox{if } Y_{ij}\;\; \mbox{is missing}.
	\end{array}
\right.
\end{eqnarray}
%

The data might be of three major types:
%
\begin{itemize}
\item MCAR - missing completely at random: missingness does not depend on data at all $P(M|Y, \theta) = P(M|\theta)$
\item MAR - missing at random: missingness does not depend on the unobserved data,
but does depend on the observed values $P(M|Y, \theta) = P(M|Y_{obs}, \theta)$
\item NMAR - not missing at random: missingness depends on the unobserved data $P(M|Y, \theta) = P(M|Y_{miss}, \theta)$
\end{itemize}

A common approach to treat missing vales is to base inference on the likelihood function for the incomplete data by treating the indicator matrix $R_{ij}$ as a random variable. Specifying the joint distribution of $R_{ij}$ and $Y_{ij}$ together with the Expectation-Maximisation algorithm is usually the method of choice.

The signature framework naturally allows us to embed the indicator vector (a single row of the indicator matrix $R_{ij}$) into the path by lifting the path in to higher dimension. For example, consider a time-series with several missing values and its corresponding indicator vector (here the index $i$ is fixed):
%
\begin{eqnarray}%\label{eq:missing_data}
Y_j\;&=&\;\{1,3,\star,5,3,\star,\star,9,3,5\}\\
R_j\;&=&\;\{0,0,1,0,0,1,1,0,0,0\},\nonumber
\end{eqnarray}
%
where the symbol ``$\star$" denotes a missing value at the expected time point. The idea is to create a two dimensional path from this data. The evolution of the path is from the starting point towards the end and can be seen as propagation in three dimensional space; the first two dimensions are ``observed data" and ``missing data", while the third direction corresponds to time. At every time point where we have a missing point, we jump from the ``observed" to the ``missing" dimension and fill in the missing place with the same value as seen before (a.k.a {\it feed forward} method). The intuition is simple: unless we have any new information about the data, we continue walking along a ``missing" axis direction, which is in another dimension than the ``observed" data. The resulting path is given by \eqref{eq:missing_data}
%
\begin{eqnarray}\label{eq:missing_data}
\tilde{Y}_{j} = \{(0,1,0),(1,3,0),(2,{\bf 3},1),(3,5,1),(4,3,1),(5,{\bf 3},2),(6,{\bf 3},3),(7,9,3),(8,3,3),(9,5,3)\}.\nonumber\\
\end{eqnarray}
%
Here we introduce an auxiliary time parametrisation vector $t\;=\;\{0,1,2,\dots,9\}$ to account for the time propagation and create a path in three-dimensional space as depicted in Fig.~\ref{fig:missingData}. Red points represent the missing data. The path propagates from $t=0$ to $t=9$, and the observed points lie in the plane $\{t,Y\}$, while in the presence of a missing value, the path jumps along the increasing direction of $R$ axis.

\begin{figure}[htb]
\centering
\includegraphics[width=0.8\linewidth]{artwork/missVal_1}
\centering
\caption{Example of embedding of data with missing values into a single path. The red dots represent unobserved data.}
\label{fig:missingData}
\end{figure}
\noindent

This approach allows us to treat data streams with unobserved data at the same footing as complete data streams, which demonstrates another conceptual advantage of the signature framework.


\subsection{Kernelization}
\label{subsec:kernel}

An important aspect of the signature which has recently gained attention is the ability to efficiently \textit{kernelize} the signature transformation.
To describe this, we introduce a \textit{truncated inner product}
on the space of signatures.
For an integer $k\geq 0$ and two signatures, $S(X)_{a,b}$ and $S(Y)_{a,b}$, we define
\begin{align}
\langle S(X)_{a,b},S(Y)_{a,b}\rangle_k
&= \sum_{|I|=k} S(X)_{a,b}^I S(Y)_{a,b}^I, \label{eq:inner_prod_level}
\\
\langle S(X)_{a,b},S(Y)_{a,b}\rangle_{\leq k}
&= \sum_{n = 0}^k \langle S(X)_{a,b},S(Y)_{a,b}\rangle_n,\label{eq:inner_prod_full}
\end{align}
where in~\eqref{eq:inner_prod_level} the sum is over all multi-indexes $I=(i_1,\ldots, i_k)$ of length $k$.
%This inner product is the natural extension of the Euclidean inner product on $\R^d$ to the space on formal power series introduced in Section~\ref{subsubsec:Chen}.
%Though not entirely trivial, the sum above converges as $K\to\infty$ thanks to the factorial decay of the signature $|S^I(X)_{a,b}| \leq \frac{L^k}{k!}$,
%where $L=\int_a^b\|X'_t\|dt$ is the length of $X$ and $I$ is any multi-index of length $k$.

Given a data set, a number of machine learning algorithms,
such as support vector machines, only need as input
the inner products (or more generally kernels) between the data points; this is known as the \textit{kernel trick}.
Fortunately, there is a way to compute
$\langle S(X),S(Y)\rangle_{\leq k}$ using a Horner-type scheme
\textit{without} the need to compute $S(X)$ and $S(Y)$ to level $k$, which was first introduced in~\cite{KO19}.
To see how this is done, recall the recursive definition
\begin{equation}
    S(X)^{i_1,\ldots,i_k}_{a,t}=\int_{a}^t S(X)^{i_1,\ldots,i_{k-1}}_{a,v}dX^{i_k}_v
    \;.
\end{equation}
Hence, for any $(s,t)\in[a,b]^2$
\begin{align}
\langle S(X)_{a,s},S(Y)_{a,t}\rangle_k
&= \sum_{i=1}^d\sum_{|J|=k-1} \int_a^s S(X)_{a,u}^J dX^i_u \int_a^t S(Y)_{a,v}^J dY_v^i
\\
&=\int_{a < u < s}\int_{a<v<t} \langle S(X)_{a,u},S(Y)_{a,v}\rangle_{k-1} d\langle X_u, Y_v \rangle,
\end{align}
where we used Fubini's theorem in the second equality,
and where, in the final integral, $d\langle X_u, Y_v \rangle$ is shorthand for $\langle \dot X_u,\dot Y_v\rangle du dv = (\sum_{i=1}^d \dot X^i_u Y^i_v) du dv$.

We therefore see that, in order to compute $\langle S(X)_{a,s},S(Y)_{a,t}\rangle_k$,
we need to retain from level $k-1$ only the function
$\langle S(X)_{a,u},S(Y)_{a,v}\rangle_{k-1}$ for $(u,v)\in[a,s]\times[a,t]$.
%and integrate it over $[a,s]\times[a,t]$ against $\langle \dot X_u,\dot Y_v\rangle$.

In the case that $X$ and $Y$ are piecewise linear paths with $P$ and $Q$ time steps respectively, $\langle \dot X_s,\dot Y_t\rangle$ is constant over $PQ$ regions of $[a,b]^2$.
Therefore, provided that we stored $\langle S(X)_{a,s},S(Y)_{a,t}\rangle_{k-1}$ for all $(s,t)\in [a,b]^2$ in memory, which is of size $O(PQ)$,
we can compute $\langle S(X)_{a,s},S(Y)_{a,t}\rangle_{k}$ for all $(s,t)\in [a,b]^2$
using $O(PQ)$ time.

In particular, we can compute the array of real numbers
\begin{equation}\label{eq:signatures_kernel}
\langle S(X)_{a,b},S(Y)_{a,b}\rangle_0, \; \langle S(X)_{a,b},S(Y)_{a,b}\rangle_1, \;
\ldots,\;
\langle S(X)_{a,b},S(Y)_{a,b}\rangle_k,
\end{equation}
and therefore also $\langle S(X)_{a,b}, S(Y)_{a,b}\rangle_{\leq k}$,
in $O(PQ(k + d))$ time and using $O(MN)$ memory
(the $O(PQd)$ factor comes from computing once at the start $\langle \dot X_s,\dot Y_t\rangle= (\sum_{i=1}^d \dot X^i_s Y^i_t)$ for $(s,t)\in[a,b]^2$).

One should compare this to the naive method of computing first $S(X)_{a,b}^I$ and $S(Y)_{a,b}^I$ for all $|I|\leq k$, and then computing $\langle S(X)_{a,b}, S(Y)_{a,b}\rangle_{\leq k}$ using~\eqref{eq:inner_prod_full}:
the array $\{S(X)_{a,b}^I : |I|\leq k\}$
contains $1+d+\ldots + d^k = O(d^{k})$ numbers,
so this naive method has at least exponential dependence on the dimension.
If we wish to work with high dimensional paths, we see that the first method provides a very fast kernelization algorithm.
This method has been applied in~\cite{KO19} to hand movement classification problem \cite{sapsanis2013emg}
and to hand written digit recognition 
from the UCI repository.

\begin{remark}
One case where the naive method 
provides better performance is if $K$ and $d$ are small, but $P$ and $Q$ are large.
This is because the naive method has linear dependence on $P, Q$ while the method above has quadratic dependence.
\end{remark}

\begin{remark}
Due  to the factorial decay property~\eqref{eq:factorial decay}, 
the \emph{untruncated} signature kernel $\langle S(X)_{a,b},S(Y)_{a,b}\rangle
= \sum_{n = 0}^\infty \langle S(X)_{a,b},S(Y)_{a,b}\rangle_n$ is well-defined.
It was observed in~\cite{SCFLY_21} that this untruncated kernel is the solution of a Goursat PDE, which allows for an efficient computation of $\langle S(X)_{a,b},S(Y)_{a,b}\rangle$.
\end{remark}

\subsubsection{Lifts of paths to reproducing kernel Hilbert spaces}

One of the biggest advantages of the kernel method is its applicable to paths with values in \textit{infinite dimensional spaces}, where direct computation of signature features is impossible.

Consider a set $\mcX$ and a function $k\colon \mcX\times\mcX\to\R$ which is symmetric (i.e. $k(x,y)=k(y,x)$) and positive definite (i.e. the $n\times n$ matrix $\{k(x_i,x_j)\}_{i,j=1}^n$ is positive definite for all $n\geq 1$ and $x_1,\ldots,x_n\in\mcX$). The typical example to keep in mind is $\mcX=\R^d$ and $k$ is a standard kernel, e.g.  $k$ is the standard inner product $k(x,y)=\langle x,y\rangle$ or the Gauss (RBF) kernel $k(x,y)=\exp(-\|x-y\|^2/{2\sigma^2})$ for parameter $\sigma>0$.

With these objects, we can form an inner product space: the vector space $H$ is the subspace of all $\R$-valued functions on $\mcX$ spanned by the set $\{k_x \,:\,x\in\mcX\}$, where $k_x(y):=k(x,y)$ for all $y\in\mcX$.
The inner product between $k_x,k_y\in H$ given defined to be $\scal{k_x,k_y}_H := k(x,y)$,
and this is extended by linearity to all of $H$:
\begin{equation}\label{eq:inner_prod_def}
    \scal{\sum_i a_i k_{x_i}, \sum_j b_j k_{y_j}} = \sum_{i,j}a_ib_j \scal{k_{x_i},k_{y_j}}
\end{equation}
(we leave it as an exercise to verify that~\eqref{eq:inner_prod_def}
is well-defined on $H$ i.e.~\eqref{eq:inner_prod_def} only depends on $\sum_i a_i k_{x_i}$ and $\sum_j b_j k_{y_j}$ as functions on $\mcX$,
and that symmetry and positive-definiteness of $k$ implies that $\scal{\cdot,\cdot}_H$ is an inner product on $H$).
The (completion of the) inner product space $(H,\scal{\cdot,\cdot}_H)$
is known as the \textit{reproducing kernel Hilbert space} of $k$.
This construction is attributed to Moore--Aronszajn~\cite{Aronszajn50}.

Consider now a path $X\colon [a,b]\to H\mcX$.
We can ``lift'' $X$ to an $H$-valued path $k_X\colon[a,b]\to H$ by $k_X(t) = k_{X_t}$.
(One can equally arrive at an $H$-valued path $X$ by starting with a $\mcX$-valued sequence $\{X_i\}_{i=1}^N$, which lifts to an $H$-valued sequence $\{k_{X_i}\}_{i=1}^N$, and then taking $X$ as the piecewise linear interpolation of the latter.)
Since $H$ is infinite-dimensional in general,
computing the signature of $k_X$ is often infeasible.\footnote{In this review we have only detailed the definition of the signature of paths taking values in finite-dimensional spaces. The reader can rest assured that the signature is well-defined for paths taking values in many infinite-dimensional spaces
which include Hilbert spaces.}
Remarkably, however, using the Horner-type scheme described in this section,
%given two paths $X,Y\colon [0,T] \to \mcX$ (or sequences),
one can efficiently compute  inner products $\langle S(k_X),S(k_Y)\rangle_{\leq n}$ provided that the kernel  $k$ is cheap to evaluate.

Even if $\mcX=\R^d$, it is often advantageous to use a non-Euclidean kernels $k$ and apply learning algorithms to the ``lifted'' path $k_X$.
For example, the Gauss kernel on $\R^d$ was used to achieve state-of-the-art results in supervised classification tasks in~\cite{KO19,CNO20}.



\subsubsection{Normalized signature moments to characterize laws of stochastic processes}

In~\cite{CO18}, the signature was applied to the following problem:
given two independent stochastic processes $X,Y$, i.e., random paths from $[a,b]$ to $\R^d$,
how can we determine if they have the same law?

A theoretical answer was already provided in~\cite{CL16}
by solving the moment problem, or more generally by using the Fourier transform as described in Section~\ref{subsubsec:moments}.
However, this approach has the same drawbacks in many applications as classical moments: from a theoretical perspective, moments need decay conditions to characterize probability measures,
while from a practical perspective, moments are not \textit{robust} in the sense that they are sensitive to outliers;
see~\cite{Hampel_robust, huber} for more on robust statistics.
On the other hand, the Fourier transform defined in~\cite{CL16}, which needs no decay assumptions and is robust, is not an easily computable quantity in practice.

To address these issues,~\cite{CO18} introduced \textit{normalized signature moments},
which have the advantage of being robust, computable (up an explicit error), and not requiring decay assumptions to characterize  probability measures.

For a signature $S(X)_{a,b}$ and a positive real number $\lambda>0$, define the ``normalized signature'' by $\Phi(X)^I = \lambda^k S(X)_{a,b}^I$,
where $k$ ranges over all $k\geq 0$
and $I$ ranges over all multi-indexes $I=(i_1,\ldots, i_k)$.
Note that $\Phi(X)$ is simply a rescaling of $S(X)$ at every level, and if $\lambda>0$ is known, we can recover $S(X)$ from $\Phi(X)$.

The main theoretical result of~\cite{CO18}
is that, if $X$ is a random path, then
we can choose $\lambda>0$ as a function of $S(X)$ in such a way that the following properties hold.
\begin{itemize}
    \item \textbf{$\Phi(X)$ characterizes the law of $X$:} the collection of numbers $\mathbb{E}[\Phi(X)^I]$, where $I$ ranges over all multi-indexes, uniquely determines the law of $S(X)$ (and therefore of $X$ if, for example, $X$ is of the form $X_t=(t,\bar X_t)$ with a fixed starting point as in Proposition~\ref{prop:signature_unique}.)
    
    \item \textbf{$\Phi(X)$ is bounded and robust:}
    define the ``inner product''
    \begin{equation}
        \langle\Phi(X),\Phi(Y)\rangle = \sum_{I} \Phi(X)^I\Phi(Y)^I
    \end{equation}
    where the sum is over all multi-indexes $I$.
    Then there there exists $A>0$ such that $|\langle\Phi(X),\Phi(Y)\rangle|\leq A$ for all paths $X$ and $Y$.
    Furthermore, $\langle\Phi(X),\Phi(Y)\rangle$
    is continuous in $(X,Y)$ under an appropriate metric.
    
    \item \textbf{Computable:} there exists a level-$k$ approximation $\langle\Phi(X),\Phi(Y)\rangle_{\leq k}^+$ such that
    \begin{equation}
    \lim_{k\to\infty}\langle\Phi(X),\Phi(Y)\rangle_{\leq k}^+ = \langle\Phi(X),\Phi(Y)\rangle
    \end{equation}
    with an explicit convergence rate and such that $\langle\Phi(X),\Phi(Y)\rangle_{\leq k}^+$ can be computed in (almost) the same time and memory as $\langle S(X),S(Y)\rangle_{\leq k}$, which is linear in $k$ -- see the discussion following~\eqref{eq:signatures_kernel}.
    
    
    \item \textbf{Maximum mean discrepancy (MMD):}
    consider two stochastic processes $X,Y$.
    The quantity
    \begin{equation}\label{eq:MMD}
    \|\mathbb{E}[\Phi(X)] - \mathbb E[\Phi(Y)]\|^2 := \sum_I |\mathbb E[\Phi(X)^I]-\mathbb E[\Phi(Y)^I]|^2,
    \end{equation}
    where the sum is over all multi-indexes $I$,
    defines a \textit{maximum mean discrepancy} (MMD), which is a metric on the laws of stochastic processes.
    Moreover,
    \begin{equation}\label{eq:MMD_compute}
        \|\mathbb{E}[\Phi(X)] - \mathbb E[\Phi(Y)]\|^2
        = \mathbb E[\langle \Phi(X),\Phi(X')\rangle]
        -2 \mathbb E[\langle \Phi(X),\Phi(Y)\rangle]
        + \mathbb E[\langle \Phi(Y),\Phi(Y')\rangle]|
    \end{equation}
    where $X,X'$ have the same law, $Y,Y'$ have the same, and all four are mutually independent.
    Expression~\eqref{eq:MMD_compute} shows that $\|\mathbb{E}[\Phi(X)] - \mathbb E[\Phi(Y)]\|^2$ is computable from i.i.d. samples from the laws of $X$ and $Y$. 
\end{itemize}

The normalized signature MMD~\eqref{eq:MMD} was used in~\cite{CO18} for a non-parametric two-sample hypothesis test.
The goal of the test is
to determine if two probability measures on paths are equal using a finite number of samples from each measure.


\end{comment}


==> section_files_tex/2_3.tex <==
\subsection{Overview of signature-based machine learning applications}
\label{subsec:overview_applications}

%\ilya{Here would be a good place to add the topological data analysis stuff in~\cite{CNO20}, and also the recent progress with Terry's group (deep signature transforms, etc.). Some references we might want to include: recognition of handwriting~\cite{char2} and gestures~\cite{gesture1}, analysis of financial data \cite{finance2}, financial models~\cite{sig_sdes}, psychiatric data~\cite{psych1}, neural networks~\cite{DeepSigs}, and GANs~\cite{sig_gans}.}


Over the past two decades, the rough path signature method has been the subject of extensive research and applications across various scientific domains.
%, drawing the attention of scholars worldwide.
The method has found success in diverse areas such as finance, healthcare, natural language processing, wearable devices and computer vision, demonstrating its versatility and the powerful expressiveness inherent in its approach. This adaptability has established the signature method as a critical asset in the ongoing research of modern machine learning techniques for streamed data.

The signature method's application to sequential data representation has evolved substantially, extending far beyond its original scope and undergoing considerable refinement. In this section, we aim to provide a concise overview of some notable examples where the signature method has been employed to tackle diverse challenges in machine learning and data analysis. Through these examples, we hope to showcase the wide-ranging implications and potential of this innovative approach in further advancing the field of machine learning. 

Already in 2005, Lyons and Sidorova worked on the application of rough path theory to the problem of sound compression \cite{lyons2005sound}. They presented a new approach which turned out to be more effective than the traditional Fourier and wavelet transforms. The main difference between these methods is in the linearity of the Fourier approach, while the signature method accounts for non-linear dependencies. 

The path signature transformation was extensively used in financial applications. Field {\it et al.}~\cite{gyurko2014extracting} have applied the signature transformation to multidimensional financial data streams to identify atypical market behaviour and recognise patterns of trading algorithms. In~\cite{levin2015learning}, Levin, Lyons, and Ni proposed a new non-parametric regression method based on the expected signature of paths. Truncating the signature results in an efficient local description and offers a provable efficiency gain over linear path segment descriptions with the same number of features. This approach can potentially achieve significant dimension reduction in highly oscillatory data streams. In numerical examples, their method achieves similar accuracy to the Gaussian Process approach but with lower computational cost, especially for large sample sizes. The truncated signature-based regression and classification models have further led to numerous applications in finance, such as the obtaining approximate solutions to the problem of optimal execution \cite{kalsi2020optimal}, non-parametric pricing and hedging of exotic derivatives \cite{lyons2020non} and many others \cite{perez2020signatures}.

The ability of path signature to handle complex data streams, reduce dimensionality of the feature space, and enhance prediction accuracy makes it a valuable asset in healthcare and medicine. As wearable technology becomes more common, the amount of data generated from these devices is enormous. By analysing data from connected devices, e.g., heart rate monitors, fitness trackers, sleep monitors, gait and other modalities, researchers can gain insights into patients' health conditions, such as to identify early patients with neurological disorders that have a higher risk of falls \cite{rehman2020gait}. Electronic Health Records (EHRs) contain vast amounts of data, including patient demographics, medical history, medications, and lab results. Applying the path signature method to EHRs can help identify patterns and trends, enabling better disease management, early detection of potential health issues, such as an early onset of sepsis \cite{morrill2020utilization}, to predict a diagnosis of Alzheimer's disease using brain image-derived biomarkers (e.g., the hippocampus, ventricles and whole brain volumes) \cite{moore2019using}. The path signature method was applied to analyse data from self-reporting tools and mobile applications, to detect longitudinal patterns \cite{kormilitzin2017detecting} in clinical trials \cite{geddes2015comparative}, predict mood changes and episodes \cite{kormilitzin2016application}, derive clinically meaningful information from daily self-reported mood ratings to classify patients’ diagnosis and to predict mood scores \cite{perez2018signature} and efficiently capture the chronological information in medical texts \cite{kormilitzin2020efficient}.

The path signature approach has been applied to computer vision tasks, such as human-pose estimation \cite{yang2022developing} and recognition of hand-writing in various languages \cite{wilson2018path,xie2017learning}. The signature approach was extended to the area of deep learning \cite{kidger2019deep} and neural controlled differential equations \cite{kidger2020neural}, and applied in topological data analysis \cite{CNO20}. Signatures were furthermore combined with kernel methods applicable to problems in classification and hypothesis testing \cite{CO18,KO19}.

Further examples of applications of rough paths, signatures and neural controlled differential equations can be found at \url{https://www.datasig.ac.uk/papers}.


\begin{comment}
    

Paths as geometric objects are legitimate candidates for applications to image recognition tasks. For example, hand written digits can be seen as continuous paths, and then the signature method becomes a natural approach to classification problems. The signature method has been successfully applied to the challenging problem of Chinese character recognition by B. Graham \cite{graham2013sparse}, and later by J. Lianwen \cite{yang2015deepwriterid}
\ilya{Is this reference correct? Lianwen does not seem to be an author.}
to a more general problem of hand written character recognition. Graham and Lianwen have shown (separately) that using signature terms as features of the image, for use in a convolutional neural network (CNN), significantly improved accuracy of online character recognition. This approach, which combines the signature and CNN methods, has won the ICDAR2013 Online Isolated Chinese Character recognition competition receiving $0.95530$ accuracy\footnote{http://tinyurl.com/nfvbdlk}. The group of J. Lianwen has developed the application\footnote{http://www.deephcr.net/en.html} with graphical user interface for character recognition. This application is based on the signature method for feature extraction from elements of images.

These successful results indicate that applications of the signature method combined with deep neural networks represent a new and efficient way to tackle challenges in the field of image recognition.



%The authors presented an efficient algorithm for reconstruction of the original sound signal $X$ from its signature terms. Consider a problem of digital compression of a continuous multi-dimensional signal $X$. Assuming that the signal is measured on a fine time scale, the signal can be seen as a continuous piece-wise linear path. Computing the signature of the resulting path, will produce signature terms $S^I(X)$ which represent the coefficients of compression of the original signal. The authors of~\cite{lyons2005sound} presented an efficient algorithm for reconstruction of the original signal $X$ from its signature terms.



%We would like to devote this section to an overview of the applications of the signature method to various problems in machine learning and data analysis which have appeared in the literature. The application areas are quite wide, including financial data, sound compression, time-series analysis, medical data, and image recognition tasks.

\subsubsection{Extracting information from the signature of a financial data stream}

Field {\it et al.}~\cite{gyurko2014extracting} have applied the signature transformation to financial data streams to find hidden patterns in trading strategies. The authors presented several examples of learning from data and further classification of unseen streams. The advantage of using the signature method is its ability to represent data using a small set of features which captures the most important properties of data in a non-parametric way without traditional statistical modelling. In their first experiment, the authors looked for atypical market behaviour across standard 30-minute time buckets obtained from the WTI crude oil future market. In the second experiment, they aimed to distinguish between orders generated by two different trade execution algorithms. We will overview their methodology and results.

As we have already seen, the basics steps within the signature approach is to convert data into paths and then compute the iterated integrals of the resulting paths. In~\cite{gyurko2014extracting}, the authors considered the following data streams:
%
\begin{itemize}
\item $P^a$ : best ask price
\item $P^b$ : best bid price
\item $V^a$ : number of orders at best ask price
\item $V^b$ : number of orders at best bid price
\item $C$\; :  cumulative traded volume
\end{itemize}
%
The final path was constructed from an embedding of normalisations of these streams. The normalisation was introduced in order to standardise the data and remove any spurious patterns. The ask and bid prices were transformed into the {\it mid price} $p_{t}$ and the {\it spread} $s_t$. Also, they included normalised time as $u_t$ and imbalance $d_t$. The details of the normalisation and transformation are described in~\cite{gyurko2014extracting}. The path is then:
%
\begin{eqnarray}
X\;=\; \left\{\left(u_{t_i},p_{t_i},s_{t_i},d_{t_i},c_{t_i}\right)_{i=0}^N\right\}
\end{eqnarray}
%
In order to capture the quadratic variation of the price, the path is extended by means of a lead-lag transform:
%
\begin{eqnarray}\label{eq:6dim-path}
Z\;=\; \left\{\left(u_{t_i}^{lead},p_{t_i}^{lead},s_{t_i}^{lead},d_{t_i}^{lead},c_{t_i}^{lead},p_{t_i}^{lag}\right)_{i=0}^N\right\}
\end{eqnarray}
%
Notice, if one is interested in the quadratic variation of any other variables, then the ``lag" transformations of these variables should be included in the resulting path.

The aim is to learn a discriminant function which can classify new streams based on features extracted from signature of paths embedded from the data. The classification method was chosen as linear regression combined with LASSO shrinkage in order to select relevant terms in the signature. To measure the significance of separation, the authors used the non-parametric Kolmogorov-Smirnov test, and the receiver operating characteristic (ROC) curve and the area under the curve.

The objectives of the first experiment in~\cite{gyurko2014extracting} are WTI crude oil futures, sampled by minutes from standard 30-minutes interval between 09:30-10:00, 10:30-11.00, and 14:00-14:30. Considering the 6-dimensional input path \eqref{eq:6dim-path} and its truncated signature at level $L=4$, there are 1555 signature terms in total, but successful application of the LASSO algorithm allowed to select four terms which are the most informative. The results are illustrated in Fig~\ref{fig:GregsPics}. The upper panels show a visible separation between two groups plotted on the feature planes $S^{(1,5,1,5,)},S^{(5,1,5,1)}$ (\ref{fig:greg_1a}) and $S^{(5,1,5,1)},S^{(1,5,5,1)}$ (\ref{fig:greg_1b}) respectively.  The bottom panels demonstrate estimated densities of regressed values with KS distance 0.9 (training) and 0.91 (out-of-sample) and 95$\%$ accuracy \ref{fig:greg_1c}. The ROC curve of the classifier with AUC = 0.986 (out-of-sample AUC 0.984) is presented in \ref{fig:greg_1d}.
%
\begin{figure}[H]
\centering
	\subcaptionbox{\label{fig:greg_1a}}%
	  [.48\linewidth]{\includegraphics[width = 0.4\linewidth]{artwork/G_1}}
	\subcaptionbox{\label{fig:greg_1b}}%
	  [.48\linewidth]{\includegraphics[width = 0.4\linewidth]{artwork/G_2}}
	\subcaptionbox{\label{fig:greg_1c}}%
	  [.48\linewidth]{\includegraphics[scale=0.265]{artwork/G_10}}
	\subcaptionbox{\label{fig:greg_1d}}%
	  [.48\linewidth]{\includegraphics[scale=0.355]{artwork/G_20}}
\caption{Visible separation between two groups projected onto $S^{(i,j,k,l)}$ feature plane (upper panels) and accuracy of separation (bottom panels). Courtesy of Field {\it et al.}~\cite{gyurko2014extracting}.}
\label{fig:GregsPics}
\end{figure}
\noindent
%
The results from the second experiment of classification of trading algorithms are presented in Fig.~\ref{fig:GregsPics2}. The aim is to classify the traces of trade execution algorithm. The data streams are sampled from the FTSE 100 index future market (NYSE Liffe) with the same transformation as described earlier. The beginning and the end of the streams are defined by the start and the end of parent orders generated by two different trade algorithms which are denoted by $A$ and $B$. Left panel \ref{fig:greg_2a} shows the estimated densities of regressed values with KS distance of 0.66 (0.518) with accuracy 82$\%$ (74.3$\%$) for training (out-of-sample) data sets. The right panel shows the ROC curve of the classifier with the AUC 0.892 (0.777) for training (out-of-sample) sets respectively.
%
\begin{figure}[H]
\centering
	\subcaptionbox{\label{fig:greg_2a}}%
	  [.48\linewidth]{\includegraphics[scale=0.265]{artwork/G_ab_1}}
	\subcaptionbox{\label{fig:greg_2b}}%
	  [.48\linewidth]{\includegraphics[scale=0.355]{artwork/G_ab_2}}
\caption{Result of classification of two trading algorithms. Courtesy of Field {\it et al.}~\cite{gyurko2014extracting}.}
\label{fig:GregsPics2}
\end{figure}
\noindent
%
The conclusions and numerical results of this work demonstrate a great potential for applications of the signature method to various problems in financial data.

\subsubsection{Sound compression - the rough paths approach}

This research project dates back to 2005, when T. Lyons and N. Sidorova worked on the application of rough paths theory to the problem of sound compression \cite{lyons2005sound}. They presented a new approach which turned out to be more effective than the traditional Fourier and wavelet transforms. The main difference between these methods is in the linearity of the Fourier approach, while the signature method accounts for non-linear dependencies. Consider a problem of digital compression of a continuous multi-dimensional signal $X$. Assuming that the signal is measured on a fine time scale, the signal can be seen as a continuous piece-wise linear path. Computing the signature of the resulting path, will produce signature terms $S^I(X)$ which represent the coefficients of compression of the original signal. The authors of~\cite{lyons2005sound} presented an efficient algorithm for reconstruction of the original signal $X$ from its signature terms.


\subsubsection{Character recognition}

Paths as geometric objects are legitimate candidates for applications to image recognition tasks. For example, hand written digits can be seen as continuous paths, and then the signature method becomes a natural approach to classification problems. The signature method has been successfully applied to the challenging problem of Chinese character recognition by B. Graham \cite{graham2013sparse}, and later by J. Lianwen \cite{yang2015deepwriterid}
\ilya{Is this reference correct? Lianwen does not seem to be an author.}
to a more general problem of hand written character recognition. Graham and Lianwen have shown (separately) that using signature terms as features of the image, for use in a convolutional neural network (CNN), significantly improved accuracy of online character recognition. This approach, which combines the signature and CNN methods, has won the ICDAR2013 Online Isolated Chinese Character recognition competition receiving $0.95530$ accuracy\footnote{http://tinyurl.com/nfvbdlk}. The group of J. Lianwen has developed the application\footnote{http://www.deephcr.net/en.html} with graphical user interface for character recognition. This application is based on the signature method for feature extraction from elements of images.

These successful results indicate that applications of the signature method combined with deep neural networks represent a new and efficient way to tackle challenges in the field of image recognition.


\subsubsection{Learning from the past, predicting the statistics for the future, learning an evolving system}

In~\cite{levin2015learning}, Levin, Lyons, and Ni address an application of the signature method to time-series analysis and develop a new regression method based on the expected signature of paths. This method of linear regression on the signature of data streams is general and allows explicit computations and predictions. The main goal of this approach is to identify the specific feature set of the observed data and linearise the functional relationships between them (features). The authors introduced {\it the expected signature model} as a linear mapping: $L: X\mapsto Y$
%
\begin{eqnarray}
Y = L(X) + \epsilon,
\end{eqnarray}
%
with $E[\epsilon]=0$ and $X\in T((\R^d)),\; Y\in T((\R^e))$, where 
\begin{eqnarray}
T((\R^d)) = \prod_{n=0}^{\infty} (\R^d)^{\otimes n}
\end{eqnarray}
%
is the algebra of tensor series over $\R^d$. We briefly outline the main idea of this model. Consider the univariate time-series ({\it returns}) denoted by $\{r_i\}_{i=1}^N$ and some fixed $k\in \mathbb{N}$, such that $1 < k < N$. Define the {\it p-past} returns up to time $t_k$ by $F_k = \{r_i\}_{i=k-p}^k$ and the {\it q-future} returns (from time $t_{k+1}$) by $G_{k+1} = \{r_i\}_{i=k+1}^{k+q}$. The signatures of $F_k$ and $G_{k+1}$ are respectively: 
%
\begin{eqnarray}\label{eq:pastFutureSig}
X_k &=& S\left(\{t_i,r_i\}_{i=k-p}^k\right)\\
Y_k &=& S\left(\{t_i,r_i\}_{i=k+1}^{k+q}\right).\nonumber
\end{eqnarray}
%
The definition of the Expected Signature model $ES(p,q,n,m)$ states that the stationary time-series $\{r_i\}_{i=1}^N$ satisfies the assumptions of the $ES$ model with parameters $p,q,n,m$ if there exists a linear functional $f:T^n\left(\mathbb{R}^2\right) \mapsto T^n\left(\mathbb{R}^2\right)$ such that:
%
\begin{eqnarray}
\rho_m\left(S(\{r_{t+i}\}_{i=1}^q)\right) = f\left(\rho_m\left(S(\{r_{t-i}\}_{i=0}^p)\right)\right) + a_t,
\end{eqnarray}
%
where $N \geq p+q$ is a positive integer, $m$ is the depth of truncation of signature, and the residual term $a_t$ satisfies $E[a_t|F_t] = 0$. Let $\mu_k$ be the expectation of $S(\{t_i,r_i\}_{i=k+1}^{k+q})$
%
\begin{eqnarray}\label{eq:meanEq}
\mu_k = E[S(\{t_i,r_i\}_{i=k+1}^{k+q})|F_k].
\end{eqnarray}
%
It thus follows from the ES model that
%
\begin{eqnarray}
\mu_k = f(X_k),
\end{eqnarray}
%
where $X_k$ is defined in \eqref{eq:pastFutureSig} with both $\mu_k$ and $a_k$ in $T((\R^2))$. Next, the conditional covariance of the signature of the future return conditioned on $F_k$ is defined as
%
\begin{eqnarray}\label{eq:volatilEq}
\Sigma_k^2(I,J) = Cov\left(S^I(Y_k),S^J(Y_k)|F_k\right),
\end{eqnarray}
%
where $I,J$ are two multi-indexes as defined previously in the text. In time-series analysis, \eqref{eq:meanEq} corresponds to the mean equation for $Y_k$, and \eqref{eq:volatilEq} is the volatility equation for $Y_k$. The fundamental assumption of the ES model is the stationarity of the time-series $\{r_i\}$, which is common in time-series analysis.

It has been shown that many standard autoregressive models (AR, ARCH, GARCH, etc.) are special cases of the ES model. For example, given the time-series $\{t_i,r_i\}$ the mean equation and volatility are written as:
%
\begin{center}
\begin{tabular}{r l l}

 & AR & ES \\ 

$m_k :$ & $E[r_{k+1}|F_k]$ & $S^{(2)}(\mu_k)$ \\ 

$\sigma^2_k :$ & $Var[r_{k+1}|F_k]$ & $2S^{(2,2)}(\mu_k) - \left(S^{(2)}(\mu_k)\right)^2$. \\ 

\end{tabular} 
\end{center}
%
Several important properties linking the autoregressive models and ES model are proven in~\cite{levin2015learning}. One of them states that if a time-series $\{r_k\}$ satisfies the assumptions of ARCH(q) model and its mean equation is given by
%
\begin{eqnarray}
\mu_k = \beta_0 + \sum_{i=1}^Q\beta_i r_{k-i},
\end{eqnarray}
%
then there exists a sufficiently large integer $n$ such that the time-series $\{r_k\}$ satisfies the assumption of $ES(q+Q,1,n,2)$. Also, the model $ES(p,1,n,2)$ is considered as a classical time-series, where the signature of the past returns as an explanatory variable.

The work in~\cite{levin2015learning} provides explicit numerical benchmarks between various autoregressive models and the expected signature model for various set-ups and configurations of the models.

\subsubsection{Identifying patterns in MEG scans}

The project of Gyurko {\it et al.}~\cite{megConbrio}
\ilya{something doesn't look right about this reference - I can't find it online anywhere}
is devoted to an application of the signature method to pattern recognition in medical studies and neuroimaging ({\bf M}agneto{\bf E}ncephalo{\bf G}raphy). The patients are asked to press a button whenever they like, and their electromagnetic brain activity is constantly monitored during this trial. The data streams of the electric signal are shown in Fig.~\ref{fig:negCONBRIO} in the first two upper panels. For the sake of simplicity, Gyurko {\it et al.} considered only two channels from the MEG scanner as sources for the streaming data. The main goal was to identify a pattern in these two data streams which is able to predict the pressing of a button. The button-pressing instance was presented by a vector with binary outcome: ``1"  and ``0" stand for the button being pressed and not being pressed respectively (Fig.~\ref{fig:negCONBRIO}, bottom panel). They used a rolling window analysis of time-series and regressed the button-pressing instances on signature of the data streams inside the rolling window.

\begin{figure}[H]
\centering
\includegraphics[width=\linewidth]{artwork/meg_1}
\caption{Finding patterns in two-dimensional data stream (two upper panels). The bottom panel shows the binary vector of the button-state (pressed or not pressed). The horizontal axis is in time units. }
\label{fig:negCONBRIO}
\end{figure}
\noindent
%
The detection and prediction results were good: AUC of ROC: 0.92 (learning set) and AUC of ROC (out-of-sample) 0.93, which indicates good separability between the two states (1 and 0). This example shows that applications of the signature approach are fairly general and are not constrained to particular cases.


\subsubsection{Learning the effect of treatment on behavioural patterns of patients with bipolar disorder.}

This is another example of an application of the signature method to analysis of medical data. Our main goal of this project is to learn the behavioural patterns of patients suffering from bipolar disorder. The data are follow-up self-reported assessment scale collected by the True Colours\footnote{https://oxfordhealth.truecolours.nhs.uk/www/en/} web platform which is developed by the Department of Psychiatry at the University of Oxford and is used for the CONBRIO programme\footnote{http://conbrio.psych.ox.ac.uk/home}.
\ilya{This link doesn't seem to work.}
Patients are encouraged to submit via this platform their answers to the self-assessment questionnaires. These questionnaires are standard clinical tools for assessment of the severity of depression (QIDS-SR$_{16}$)~\cite{rush200316} and mania (AMSR)~\cite{altman1997altman} symptoms. These questionnaires contain 16 and 5 questions and scales are ranged [0 27] and [0 25] for QIDS-SR$_{16}$ and AMSR respectively. In Fig.~\ref{fig:qidsScore}, an example of the QIDS score for 50 weeks follow-up observations is displayed.
%
\begin{figure}[H]
\centering
\includegraphics[width=0.9\linewidth]{artwork/qids_1}
\caption{A typical example of the follow-up observations of the QIDS score.}
\label{fig:qidsScore}
\end{figure}
\noindent
%
As a part of our research programme, we analysed data from the CEQUEL clinical trial \cite{geddes2015comparative}. The primary objective is to compare the combination therapy of quetiapine plus lamotrigine with quetiapine monotherapy for treatment of bipolar depression. Among other interesting research questions, we focused on the behavioural pattern of patients in two different treatment groups: placebo and lamotrigine. Patients are asked to submit their self-assessment scores to the True Colours platform on a weekly basis. The system sends a scheduled prompt text every week and patients should reply within one week interval. If no response is received within a week, the system flags this week as a missing observation and sends a new prompt at the beginning of the next week. We analysed the delays - the time intervals between the prompt text and the patient's reply measured in integer units of days. The delays are presented schematically in the Fig.~\ref{fig:delays_old}. 
%
\begin{figure}[H]
\centering
\includegraphics[width=0.7\linewidth]{artwork/delays_old}
\caption{Definition of the delays $d_i$. The time line is divided by the dashed lines into weekly intervals. The delay is defined as the time difference between the beginning of the week (dashed line) and the time when the response is received (red dot). This particular configuration of delays corresponds to: $\{d_i\} = \{4,2,5,0,5,0\}$.}
\label{fig:delays_old}
\end{figure}
\noindent
%
The delays of the QIDS data from the Fig.~\ref{fig:qidsScore} are shown in the Fig.~\ref{fig:delaysAll}. 

\begin{figure}[H]
\centering
\includegraphics[width=\linewidth]{artwork/delays_1}
\caption{Example of the delays $d_i$ of the QIDS scores presented in the Fig.~\ref{fig:qidsScore}. Submissions are denoted by the red dots.}
\label{fig:delaysAll}
\end{figure}
\noindent

We were interested in the question, whether the distribution of delays $\{d_i\}$ is different between the two different treatment groups, namely placebo and lamotrigine. To answer this question, we applied the signature method to time-series constructed from the delay data $\{d_{i}\}$ and used regularised logistic regression to discriminate between the two groups. The sample sizes of the two groups are: 18 and 11 patients in the placebo and the lamotrigine group respectively. We constructed continuous paths from the sequence of integer delays $\{d_i\}$ by means of two types of embeddings: the first is the three dimensional simple lead-lag transformation of the raw data $\{d_i\}$ with time stamps:
%
\begin{eqnarray}
X\;=\;\left\{\left(t^{lead}_i,d^{lead}_i,d^{lag}_i\right)_i\right\},
\end{eqnarray}
%
and the second embedding corresponds to the lead-lag transformation of the cumulative sum (partial sums) of the delays:
%
\begin{eqnarray}
S\;=\;\left\{\left(s^{lead}_i,s^{lag}_i\right)_i\right\}.
\end{eqnarray}
%
We computed signature terms from these two embeddings separately up to level $L$ and combined these terms in a single design matrix, which we used as the feature matrix for the logistic regression. The design matrix exhibited some degree of multicollinearity, thus we applied the elastic net regularisation scheme \cite{zou2005regularization} to the logistic regression. The elastic net allows a smooth regularisation, which benefits from both L$_1$ and L$_2$ norm shrinkage schemes, groups the correlated covariates, and removes the less relevant features. The choice of the $\alpha$ parameter of the elastic net is performed by the cross validated grid search, and estimated as $\alpha = 0.55$ giving the smallest deviance error as shown in Fig.~\ref{fig:kor3}. 
%
\begin{figure}[H]
\centering
%	\subcaptionbox{\label{fig:greg_2a}}%
%	  [.48\linewidth]
{\includegraphics[width=0.45\linewidth, height=5.3cm]{artwork/CVlassoPlot}}
%	\subcaptionbox{\label{fig:greg_2b}}%
%	  [.48\linewidth]
\hfill
{\includegraphics[width=0.45\linewidth]{artwork/CVlassoPlotPaths}}
\caption{Statistical results of cross validated elastic net regularisation scheme.}
\label{fig:kor3}
\end{figure}
\noindent
%
The final classification model is chosen by the ``one-standard-error'' rule, denoted by the position of the blue dashed line, given the fact that the initial 10-dimensional feature set was shrunk to a 6-dimensional subset. Some of the features of this subset are displayed in the Fig.~\ref{fig:kor4}.
%
\begin{figure}[htb]
\centering
\includegraphics[width=\linewidth]{artwork/classif_3}
\centering
\caption{Examples of relevant features selected by the penalised logistic regression. These two groups denoted by ``0" and ``1" correspond to the placebo and the lamotrigine groups respectively.}
\label{fig:kor4}
\end{figure}
\noindent
%

The results of this project demonstrated the ability of the signature method to extract characteristic features from the data in a systematic way without introducing any {\it ad hoc} methods. The signature feature extraction method serves as an initial step in the machine learning pipeline. Once we transformed the raw data into a set of signature terms, we naturally proceed further with standard machine learning techniques and methodologies using these features as inputs.


\subsubsection{Barcodes and topological data analysis}
\label{subsubsec:TDA}

\ilya{We should probably scrap this section}

In~\cite{CNO20}, the path signature was used in persistent homology, one of the main tools of topological data analysis,
to give a novel way to extract features for statistical learning.
The typical object one studies in
persistent homology is a \textit{barcode}, or \textit{persistence diagram}.
Barcodes record the birth and death of homological features of point cloud under various changes of scale; for every homological dimension studied, one obtains a barcode.
For our purposes, a barcode is a finite multiset $B=\{[b_i,d_i)\}_{i=1}^m$
of subintervals $[b_i,d_i)\subset [0,T]$ for some $T>0$,
which we treat as a feature of our data.

\begin{example}
A common example is the \textit{Vietoris–Rips filtration}.
Loosely speaking, given a finite set of points $Z\subset \R^d$ with diameter at most $T$, one defines a simplicial complex for every $t\in[0,T]$ by adding a subset $\{z_1,\ldots, z_n\}\subset Z$ into the complex if and only if $|z_i-z_j|\leq t$ for all $1\leq i,j\leq, n$.
The corresponding barcodes record the change in homology of the resulting simplex as $t$ increases from $0$ to $T$.
See Figure~\ref{fig:bars}.
\begin{figure}[h!]
\includegraphics[scale = 0.3]{artwork/barpic.png}
\caption{Example of barcodes.
Blue lines are the bars from the $0$-th homological dimension (counting the number of connected components in the complex),
and red lines are the bars from the $1$-st homological dimension (counting the number of ``holes'' in the complex).}\label{fig:bars}
\end{figure}
\end{example}

The space of barcodes is a non-linear (metric) space, making the application of many machine learning algorithms to persistent homology highly non-trivial and an active area of research, see~\cite{adams2017persistence} and there references therein.
So-called \textit{persistence paths} were introduced in~\cite{CNO20} to tackle this problem by embedding the space of barcodes into the space of paths, after which signature methods can applied.
\begin{remark}
In contrast to the previous examples, where there is an \textit{intrinsic} path (time-ordering) in the data,
the paths introduced in~\cite{CNO20} are \textit{extrinsic} in the sense that they are artificially produced in order to facilitate
statistical learning.
This application in particular highlights that the signature method can be applied to problems where paths are not immediately present.
\end{remark}
We describe three examples of such persistence path embeddings.
\begin{example}[Naive embedding.]
As the name suggests, this is likely the first method which comes to mind.
Consider the bars $[b_1,d_1),\dots, [b_m,d_m)$ of a barcode in an arbitrary order (say, decreasing in length or in birth time $b_i$).
Consider the path $X\colon[0,T]\to \R^m$ defined by $\dot X^i(t) = 1$ if $t\in [b_i,d_i)$ and $\dot X^i(t) = 0$ if $t\notin [b_i,d_i)$.
In words, the path $X$ increases in the $i$-th coordinate at unit speed if the $i$-th bar is active.
\end{example}

\begin{example}[Betti and Euler embeddings.]
The $i$-th Betti number of a simplicial complex is the rank of the $i$-th dimensional homology group.
In terms of barcodes, the $i$-th Betti number at scale $t\in[0,T]$, denoted $\beta_t^i$, is the number of bars in the barcode of $i$-th homological dimension present at $t\in[0,T]$.
To construct a path from this data,
let $t_1< t_2<\ldots <t_N$ be the ordered set of all endpoints of intervals in $B$ (i.e. all birth and death times) with the convention that $t_1=0$ and $t_N=T$.
The \textit{Betti embedding} is the path $X\colon[0,T]\to \R^n$ defined by $X_{t_j} = (\beta_0^{t_j},\ldots \beta_{n-1}^{t_j})\in\R^n$ for all
$j=0,\ldots,N$
and with piecewise linear interpolation in between these points.
The \textit{Euler embedding} is the path $Y\colon[0,T]$ derived from $X$ by taking the alternating sum $Y_t = \sum_{i=0}^{n-1} (-1)^iX^i_t$.
\end{example}

\begin{example}[Envelope embedding.]
This embedding is different in flavor from the previous two since the role of time is no longer played by the scale parameter $t$.
One arranges the bars $[b_1,d_1),\ldots,[b_m,d_m)$ in decreasing length and stacks and stacks these above the positive integers. 
One then creates an upper and lower envelope by connecting in a piecewise linear fashion the death and birth times respectively
resulting in a two-dimensional path $X\colon[0,N]\to\R^2$,
see Figure~\ref{fig:env}.
\begin{figure}[h!]
\includegraphics[scale=.4]{artwork/envemb.png}
\caption{Example of envelope embedding.}\label{fig:env}
\end{figure}
\end{example}

These embeddings, combined with the signature method, were applied to the three classification tasks in~\cite{CNO20}.
Betti and Euler embeddings (and their kernelized versions) in general performed the best, followed closely by the envelope embedding.
Notably, these methods performed on par with state-of-the-art methods in topological data analysis, outperforming benchmark methods from~\cite{adams2017persistence, sliced_wasserstein} in two out of three tasks.

\begin{remark}
An additional embedding was introduced in~\cite{CNO20}, called the \textit{integrated landscape embedding}, which uses the
persistence landscapes of Bubenik~\cite{Bubenik15}.
This embedding possesses very attractive theoretical stability and discriminatory properties.
However, the resulting paths were high-dimensional and piecewise parabolic (i.e. piecewise linear \textit{derivatives}),
so due to computation difficulties
this embedding was not implemented in the experiments.
The high-dimensionality of the resulting path could theoretically be tackled with kernel methods (see Section~\ref{subsubsec:kernel}),
but how to efficiently implement these methods for non-piecewise linear paths remains an interesting research problem.
\end{remark}
\end{comment}

==> section_files_tex/2_4.tex <==
\section{Outlook}

%So far, we have presented a theoretical background and practical applications of this method, but nothing has been mentioned about exact numerical computations of the signature and iterated integrals of paths. As it has been defined in \eqref{eq:definSig}, the terms of the signature are iterated integrals of a path, while the path is normally constructed by an interpolation of data points. One can compute such iterated integrals using several computational algorithms(cubature methods) which are generally straightforward to implement. %The research group in the University of Oxford works with a particular implementation of such algorithms written in C++ ({\it CoRoPa} project) \footnote{http://coropa.sourceforge.net/} with Python wrapper package {\it sigtools}. Research groups from other universities have successfully implemented computations of iterated integrals with Matlab\texttrademark. 
%Recently, a new software `ESig' package has been developed. It is implementated in C++ ({\it CoRoPa} project) \footnote{http://coropa.sourceforge.net/} with a Python wrapper. 


